X-ray and IR Point Source Identification and Characteristics in the Embedded, Massive Star-Forming Region RCW 108

We report on the results of an approximately 90 ks Chandra observation of a complex region that hosts multiple sites of recent and active star formation in ARA OB1a. The field is centered on the embedded cluster RCW 108-IR and includes and a large portion of the open cluster NGC 6193. We detect over 420 X-ray sources in the field and combined these data with deep near-IR, Spitzer/IRAC and MSX mid-IR data. We find about 360 of the X-ray sources have near--IR counterparts. We divide the region into 5 parts based on the X-ray point source characteristics and extended 8 micron emission. The most clearly defined regions are the central region - identified by embedded sources with high luminosities in the both the near-IR and X-ray as well as high X-ray temperatures (about 3 keV) and the eastern region - identified by low extinction and 1 keV X-ray temperatures. Other regions, identified by their directional relationship to RCW 108-IR are less uniform - representing combinations of the first two regions, independent star formation epochs, or both. Over 18% percent of the cluster members with over 100 counts exhibit flares. Overall about 50% of the stars appear to have optically thick disks when IRAC data are employed. The largest fraction of X-ray sources are best described as possessing some disk material via a more detailed extinction fitting. We estimate that the total number of pre--main sequence stars in the field is about 1600. Approximately 800 are confined to (1.1 pc) central region.

==> table_1.tex <==
\begin{deluxetable}{llllrrrc}
%\tabletypesize{\normal}
\tablecaption{Faint X-ray sources detected in the RCW 108 Field \label{XSources}}
\tablewidth{0pt}
\tablehead{
\colhead{SRC \#} &\colhead{CXOWSB~J} &\colhead{RA}  &\colhead{DEC}   & \colhead{Offaxis}   &
 \colhead{Counts} &\colhead{Counts}  & \colhead {BB95}\\
\colhead{} &\colhead{} &\colhead{(J2000.0)}  &\colhead{(J2000.0)}   & \colhead{[arcsec.]}   &
\colhead{[Raw]} &   \colhead{[Net]} & \colhead{}}
\startdata
  1&164036.6-485217.3&16:40:36.64&-48:52:17.37&375.2&130&112.7&1   \\
  2&164035.8-485106.7&16:40:35.82&-48:51:06.76&369.5&187&169.8&1   \\
  3&164034.9-485049.5&16:40:34.90&-48:50:49.52&363.2&95&79.3&1	   \\
  4&164033.3-485023.6&16:40:33.32&-48:50:23.67&353.6&666&661.5&4   \\
  5&164032.1-485323.0&16:40:32.14&-48:53:23.02&341.8&23&17.5&1	   \\
  6&164031.9-484913.0&16:40:31.90&-48:49:13.06&365.2&59&43&1	   \\
  7&164031.8-485312.4&16:40:31.89&-48:53:12.42&336.7&138&133.2&1   \\
  8&164031.4-485311.9&16:40:31.44&-48:53:11.95&332.3&152&147.1&2   \\
  9&164031.2-485211.5&16:40:31.23&-48:52:11.56&321.6&59&51.8&1	   \\
 10&164031.0-485249.6&16:40:31.07&-48:52:49.68&324.2&61&55.7&1	   \\
 11&164030.9-484938.0&16:40:30.92&-48:49:38.04&346.1&33&27.9&1	   \\
 12&164030.6-485215.6&16:40:30.67&-48:52:15.61&316.3&738&730.8&6   \\
 13&164030.6-485026.4&16:40:30.66&-48:50:26.41&327.5&37&31.3&1	   \\
 14&164030.2-485108.3&16:40:30.20&-48:51:08.36&314.4&43&38.3&2	   \\
 15&164030.1-484957.8&16:40:30.12&-48:49:57.82&331.4&18&12.7&2	   \\
 16&164029.3-485246.2&16:40:29.37&-48:52:46.28&307.2&205&199.3&1   \\
 17&164028.5-485237.8&16:40:28.59&-48:52:37.87&298.2&57&51.5&1	   \\
 18&164028.1-485352.5&16:40:28.10&-48:53:52.52&313.4&44&38.2&1	   \\
 19&164027.6-485028.0&16:40:27.61&-48:50:28.01&298.2&40&34.6&1	   \\
 20&164027.0-485221.7&16:40:27.08&-48:52:21.77&281.5&52&46.8&1	   \\
 21&164026.8-485118.3&16:40:26.84&-48:51:18.38&280.1&72&66.3&1	   \\
 22&164026.7-485200.4&16:40:26.74&-48:52:00.48&276.9&54&49.1&1	   \\
 23&164026.5-485105.4&16:40:26.54&-48:51:05.41&279.1&72&66.3&1	   \\
 24&164024.7-485200.5&16:40:24.72&-48:52:00.52&256.9&70&64.9&1	   \\
 25&164024.3-485334.0&16:40:24.31&-48:53:34.04&271.8&94&88.3&1	   \\
 26&164024.0-485333.5&16:40:24.01&-48:53:33.55&268.8&102&95.9&1	   \\
 27&164023.9-485053.0&16:40:23.90&-48:50:53.03&256.2&58&50.6&1	   \\
 28&164023.2-485115.3&16:40:23.21&-48:51:15.35&245&78&72.2&1	   \\
 29&164022.9-485307.6&16:40:22.93&-48:53:07.63&250.2&113&107.7&1   \\
 30&164021.9-484838.9&16:40:21.96&-48:48:38.98&301.4&202&196.7&3   \\
 31&164021.9-485532.1&16:40:21.95&-48:55:32.14&316.4&31&25.9&1	   \\
 32&164021.4-485244.3&16:40:21.45&-48:52:44.33&230.1&78&76.1&1	   \\
 33&164021.0-485219.0&16:40:21.08&-48:52:19.06&222.3&20&18.5&1	   \\
 34&164020.3-485013.0&16:40:20.36&-48:50:13.08&236.6&36&34&1	   \\
 35&164020.3-485246.2&16:40:20.35&-48:52:46.24&219.9&31&28.8&1	   \\
 36&164020.0-485103.4&16:40:20.08&-48:51:03.48&217.1&34&32.4&1	   \\
 37&164020.1-485020.0&16:40:20.12&-48:50:20.02&231.5&302&300.4&1   \\
 38&164019.8-484939.7&16:40:19.85&-48:49:39.74&248.4&38&32.5&1	   \\
 39&164019.5-485249.9&16:40:19.52&-48:52:49.96&213&59&57.2&1	   \\
 40&164019.1-485011.4&16:40:19.11&-48:50:11.47&226.2&149&147.4&1   \\
 41&164019.0-485242.7&16:40:19.03&-48:52:42.77&206.5&18&16.6&1	   \\
 42&164018.8-484940.5&16:40:18.80&-48:49:40.54&239.3&21&19.6&1	   \\
 43&164018.2-485637.9&16:40:18.23&-48:56:37.90&343&88&81.4&1	   \\
 44&164018.0-484910.7&16:40:18.00&-48:49:10.72&51.1&32&27&1	   \\
 45&164016.4-485528.2&16:40:16.49&-48:55:28.25&276.8&32&25.9&1	   \\
 46&164016.1-484709.2&16:40:16.13&-48:47:09.21&333&95&91.1&1	   \\
 47&164015.8-485333.2&16:40:15.81&-48:53:33.20&195.8&29&27.8&1	   \\
 48&164015.4-485417.5&16:40:15.44&-48:54:17.55&218.8&19&18&1	   \\
 49&164015.4-485503.9&16:40:15.44&-48:55:03.94&251.6&102&97.1&1	   \\
 50&164014.3-485253.8&16:40:14.31&-48:52:53.83&165.2&33&31.4&1	   \\
 51&164014.2-485016.1&16:40:14.29&-48:50:16.10&182.5&22&20.6&1	   \\
 52&164014.2-485102.8&16:40:14.28&-48:51:02.81&162.2&19&17.6&1	   \\
 53&164014.2-485540.8&16:40:14.23&-48:55:40.81&273.6&189&184.6&1   \\
 54&164013.9-485706.3&16:40:13.97&-48:57:06.39&346.7&55&48.8&1	   \\
 55&164013.4-485614.2&16:40:13.46&-48:56:14.24&298.1&73&67.8&1	   \\
 56&164013.1-485305.0&16:40:13.17&-48:53:05.07&159.4&48&46.4&3	   \\
 57&164012.8-485113.8&16:40:12.80&-48:51:13.82&144.9&13&11.9&1	   \\
 58&164012.5-485233.7&16:40:12.59&-48:52:33.74&142.7&21&19.6&1	   \\
 59&164012.3-484637.7&16:40:12.36&-48:46:37.75&344&44&40.8&1	   \\
 60&164012.0-484831.9&16:40:12.08&-48:48:31.97&241.6&30&23.8&1	   \\
 61&164011.9-484817.0&16:40:11.96&-48:48:17.09&253.6&1096&1090.6&3 \\
 62&164011.9-484859.2&16:40:11.92&-48:48:59.23&218.3&46&44.2&1	   \\
 63&164011.6-485134.1&16:40:11.60&-48:51:34.15&129&12&10.1&1	   \\
 64&164011.0-485451.9&16:40:11.07&-48:54:51.97&215.7&255&252.9&2   \\
 65&164010.7-485232.3&16:40:10.76&-48:52:32.34&125.1&20&18.3&1	   \\
 66&164010.7-485049.3&16:40:10.78&-48:50:49.38&135.7&22&20.1&1	   \\
 67&164010.6-485426.1&16:40:10.68&-48:54:26.19&192.6&44&42.5&3	   \\
 68&164010.6-485239.1&16:40:10.63&-48:52:39.11&126&31&29.5&3	   \\
 69&164010.6-485303.2&16:40:10.61&-48:53:03.29&136.4&21&19.7&1	   \\
 70&164010.5-485124.5&16:40:10.53&-48:51:24.54&120.5&390&387.4&4   \\
 71&164010.5-485340.0&16:40:10.51&-48:53:40.05&157.5&15&13.8&1	   \\
 72&164010.3-485010.6&16:40:10.36&-48:50:10.67&154.9&75&73.4&1	   \\
 73&164010.3-485250.1&16:40:10.37&-48:52:50.15&128.1&19&17.5&1	   \\
 74&164010.0-485425.5&16:40:10.05&-48:54:25.51&188.3&26&24.3&1	   \\
 75&164009.3-485538.5&16:40:09.30&-48:55:38.54&247.6&63&57&1	   \\
 76&164008.8-485147.3&16:40:08.85&-48:51:47.36&100.5&14&12.6&1	   \\
 77&164008.8-485404.2&16:40:08.82&-48:54:04.21&164&18&16.6&1	   \\
 78&164008.7-485108.4&16:40:08.70&-48:51:08.40&108.8&29&27.1&1	   \\
 79&164008.6-485629.9&16:40:08.62&-48:56:29.99&292.7&53&48.9&1	   \\
 80&164008.3-485127.6&16:40:08.32&-48:51:27.63&98.7&15&13.6&1	   \\
 81&164007.8-485035.3&16:40:07.82&-48:50:35.39&119.7&18&16.4&1	   \\
 82&164007.5-485057.5&16:40:07.53&-48:50:57.50&104&33&31.7&1	   \\
 83&164007.4-485104.2&16:40:07.45&-48:51:04.24&99.8&12&10.4&1	   \\
 84&164007.4-485024.1&16:40:07.49&-48:50:24.15&125.1&380&378.5&4   \\
 85&164007.1-485054.9&16:40:07.14&-48:50:54.98&102.3&24&22.6&1	   \\
 86&164007.1-485038.2&16:40:07.12&-48:50:38.24&112.6&43&42&1	   \\
 87&164006.7-485034.1&16:40:06.75&-48:50:34.16&112.8&15&13.3&1	   \\
 88&164006.5-485703.1&16:40:06.51&-48:57:03.19&318.5&50&46.1&3	   \\
 89&164006.4-485043.4&16:40:06.44&-48:50:43.47&104.1&27&25.5&1	   \\
 90&164006.3-485431.5&16:40:06.33&-48:54:31.55&174.5&40&38.7&1	   \\
 91&164006.3-485140.6&16:40:06.37&-48:51:40.67&77&18&16.5&1	   \\
 92&164006.2-485111.9&16:40:06.28&-48:51:11.92&86&174&172.8&2	   \\
 93&164006.0-485143.9&16:40:06.03&-48:51:43.92&73.1&61&59.2&1	   \\
 94&164005.9-485629.4&16:40:05.96&-48:56:29.48&284.5&80&75.5&1	   \\
 95&164005.9-485111.4&16:40:05.93&-48:51:11.45&83.2&18&16.8&1	   \\
 96&164005.7-485213.7&16:40:05.70&-48:52:13.72&71.9&27&25.1&1	   \\
 97&164005.6-485538.1&16:40:05.60&-48:55:38.18&234.1&21&19.7&1	   \\
 98&164005.4-485349.5&16:40:05.42&-48:53:49.59&133.2&27&25.7&1	   \\
 99&164004.7-485152.3&16:40:04.78&-48:51:52.30&60.2&14&12.1&1	   \\
100&164004.4-485145.3&16:40:04.48&-48:51:45.36&57.8&65&63.1&1	   \\
101&164003.8-485254.8&16:40:03.88&-48:52:54.85&79.4&15&14.2&1	   \\
102&164003.5-485009.7&16:40:03.55&-48:50:09.77&114.9&40&38.8&1	   \\
103&164003.3-485125.3&16:40:03.39&-48:51:25.31&54.7&35&33.7&1	   \\
104&164002.4-485634.7&16:40:02.45&-48:56:34.79&283.1&153&148.3&1   \\
105&164001.9-485153.5&16:40:01.93&-48:51:53.52&32&40&37.7&1	   \\
106&164001.9-485445.5&16:40:01.91&-48:54:45.50&174.3&24&22.7&2	   \\
107&164001.8-485137.2&16:40:01.84&-48:51:37.27&35.4&90&88.2&1	   \\
108&164001.7-485235.1&16:40:01.74&-48:52:35.12&50.8&29&27.9&1	   \\
109&164001.6-485153.3&16:40:01.66&-48:51:53.32&29.4&79&76.3&1	   \\
110&164001.6-485042.9&16:40:01.61&-48:50:42.97&76.8&40&38.3&1	   \\
111&164001.2-485145.5&16:40:01.28&-48:51:45.50&26.9&65&63.4&1	   \\
112&164001.1-485152.2&16:40:01.17&-48:51:52.21&24.5&13&11.1&1	   \\
113&164001.0-485051.5&16:40:01.03&-48:50:51.55&66.7&124&122.1&1	   \\
114&164000.8-485138.5&16:40:00.82&-48:51:38.52&26.2&78&75&1	   \\
115&164000.6-484609.5&16:40:00.67&-48:46:09.55&345.2&17&12.1&2	   \\
116&164000.3-485143.1&16:40:00.34&-48:51:43.16&19.7&328&323.6&1	   \\
117&164000.3-485107.7&16:40:00.33&-48:51:07.72&49.2&35&32.4&1	   \\
118&164000.1-485139.9&16:40:00.15&-48:51:39.93&20.3&1383&1379&3	   \\
119&164000.1-485124.4&16:40:00.16&-48:51:24.44&33.1&84&81.5&2	   \\
120&164000.0-485142.6&16:40:00.01&-48:51:42.60&17.4&349&345.6&3	   \\
121&163959.9-485153.0&16:39:59.92&-48:51:53.05&12.2&87&84.5&1	   \\
122&163959.9-485107.1&16:39:59.93&-48:51:07.19&48.5&60&57.7&1	   \\
123&163959.7-485441.7&16:39:59.74&-48:54:41.79&167.9&10&8.9&1	   \\
124&163959.7-485159.7&16:39:59.76&-48:51:59.74&11.9&123&121.6&1	   \\
125&163959.5-485137.2&16:39:59.50&-48:51:37.29&18.7&99&94.1&1	   \\
126&163959.4-485059.8&16:39:59.44&-48:50:59.86&54.8&58&56.7&1	   \\
127&163959.3-485127.8&16:39:59.34&-48:51:27.87&27.1&16&14.5&1	   \\
128&163958.9-485049.3&16:39:58.99&-48:50:49.34&64.9&47&46.5&2	   \\
129&163958.7-485137.7&16:39:58.73&-48:51:37.72&16.4&23&20.4&1	   \\
130&163958.5-485236.9&16:39:58.50&-48:52:36.94&42.8&11&8.5&1	   \\
131&163958.5-485204.9&16:39:58.53&-48:52:04.90&10.9&499&498.1&4	   \\
132&163958.5-485153.8&16:39:58.52&-48:51:53.87&1.7&24&20.4&2	   \\
133&163958.3-484653.4&16:39:58.36&-48:46:53.41&300.8&36&31&1	   \\
134&163957.6-484556.8&16:39:57.65&-48:45:56.83&357.5&149&144.5&3   \\
135&163957.2-485213.9&16:39:57.25&-48:52:13.95&24.4&12&10.9&1	   \\
136&163956.0-485148.3&16:39:56.01&-48:51:48.39&27.1&261&259.6&1	   \\
137&163954.5-485321.0&16:39:54.58&-48:53:21.08&95.9&12&10.6&1	   \\
138&163954.4-485201.9&16:39:54.49&-48:52:01.97&42.2&24&23.1&1	   \\
139&163954.2-485514.1&16:39:54.26&-48:55:14.15&204.7&20&19.2&1	   \\
140&163953.7-485145.6&16:39:53.72&-48:51:45.68&49.7&31&30.5&1	   \\
141&163953.7-485136.9&16:39:53.74&-48:51:36.93&51.8&12&11.3&1	   \\
142&163953.3-485148.4&16:39:53.32&-48:51:48.47&53.3&21&20.5&1	   \\
143&163953.2-485239.8&16:39:53.22&-48:52:39.81&70.7&19&17.6&1	   \\
144&163953.0-485130.0&16:39:53.02&-48:51:30.08&60.9&13&12.3&1	   \\
145&163951.8-485141.6&16:39:51.83&-48:51:41.65&68.9&22&21.4&1	   \\
146&163951.3-484645.5&16:39:51.33&-48:46:45.56&317.1&122&117.8&1   \\
147&163949.6-485023.8&16:39:49.68&-48:50:23.86&126.7&12&10.4&2	   \\
148&163949.4-485225.2&16:39:49.42&-48:52:25.28&96.6&79&77.8&2	   \\
149&163948.4-484900.4&16:39:48.46&-48:49:00.48&200.9&11&9.6&1	   \\
150&163946.8-485146.6&16:39:46.82&-48:51:46.67&117.3&29&27.5&1	   \\
151&163946.3-485634.9&16:39:46.38&-48:56:34.91&305.8&840&834.8&7   \\
152&163945.4-485135.5&16:39:45.45&-48:51:35.54&132&22&20.7&1	   \\
153&163945.4-485101.7&16:39:45.42&-48:51:01.77&141.1&27&25.7&1	   \\
154&163944.2-485204.3&16:39:44.21&-48:52:04.30&143.2&12&10.1&1	   \\
155&163941.1-485004.8&16:39:41.10&-48:50:04.89&205.1&43&42.2&1	   \\
156&163939.5-485456.0&16:39:39.58&-48:54:56.01&261.9&25&21.3&1	   \\
157&163939.6-485348.7&16:39:39.60&-48:53:48.74&220.4&103&102.1&1   \\
158&163939.5-484730.9&16:39:39.58&-48:47:30.98&323.9&108&102.9&1   \\
159&163939.3-485356.5&16:39:39.30&-48:53:56.50&227&12&10.5&1	   \\
160&163939.2-485320.1&16:39:39.20&-48:53:20.14&210.7&58&56.3&1	   \\
161&163939.1-485225.9&16:39:39.12&-48:52:25.93&195.7&26&24.5&1	   \\
162&163938.9-484619.5&16:39:38.92&-48:46:19.57&387.4&34&18.6&1	   \\
163&163938.7-485348.4&16:39:38.77&-48:53:48.44&227.3&19&17.6&1	   \\
164&163938.6-485454.7&16:39:38.68&-48:54:54.73&267.5&155&150.7&1   \\
165&163938.2-485656.2&16:39:38.21&-48:56:56.22&363.3&287&273.8&3   \\
166&163938.2-484658.0&16:39:38.22&-48:46:58.02&358.6&87&82.2&3	   \\
167&163937.1-485643.5&16:39:37.11&-48:56:43.55&359.2&447&443.2&3   \\
168&163937.2-484651.6&16:39:37.22&-48:46:51.64&369.4&124&109.7&1   \\
169&163936.9-485200.1&16:39:36.95&-48:52:00.16&214.6&17&15.3&1	   \\
170&163935.1-485404.6&16:39:35.17&-48:54:04.62&266.1&182&178&3	   \\
171&163934.4-485332.1&16:39:34.49&-48:53:32.14&258&38&33.7&1	   \\
172&163934.3-485506.8&16:39:34.33&-48:55:06.89&308&145&141.4&2	   \\
173&163933.5-485459.0&16:39:33.54&-48:54:59.03&309.4&134&130.5&1   \\
174&163930.6-485102.7&16:39:30.69&-48:51:02.75&281.1&155&150.2&2   \\
175&163930.6-485031.0&16:39:30.68&-48:50:31.09&288.7&43&38.3&1	   \\
176&163928.8-485019.8&16:39:28.80&-48:50:19.80&309.8&37&32.4&3	   \\
177&164036.1-485353.4&16:40:36.17&-48:53:53.44&388.5&69&54.2&2	   \\
178&164035.5-485327.0&16:40:35.55&-48:53:27.04&375.3&42&26.6&1	   \\
179&164033.6-485433.3&16:40:33.66&-48:54:33.38&379.9&60&44.1&1	   \\
180&164033.3-485041.8&16:40:33.39&-48:50:41.88&350&34&29&1	   \\
181&164033.0-485001.4&16:40:33.06&-48:50:01.47&357.5&21&16.5&1	   \\
182&164032.8-485437.1&16:40:32.85&-48:54:37.10&374.3&40&23.2&2	   \\
183&164032.7-485110.9&16:40:32.74&-48:51:10.99&338.7&31&25.8&1	   \\
184&164030.4-485441.4&16:40:30.46&-48:54:41.45&355.2&19&12.5&1	   \\
185&164029.2-485224.9&16:40:29.20&-48:52:24.92&302.6&23&16.2&1	   \\
186&164028.3-484937.9&16:40:28.32&-48:49:37.92&322.7&20&14.6&1	   \\
187&164027.0-485437.3&16:40:27.02&-48:54:37.37&323.6&19&13.2&1	   \\
188&164025.7-484837.5&16:40:25.74&-48:48:37.54&331.6&50&45&1	   \\
189&164024.9-485101.1&16:40:24.99&-48:51:01.11&264.9&31&25.4&2	   \\
190&164024.4-485141.6&16:40:24.48&-48:51:41.60&254.8&22&16.1&1	   \\
191&164024.1-485443.3&16:40:24.17&-48:54:43.35&303&21&16.9&1	   \\
192&164023.9-484715.1&16:40:23.93&-48:47:15.15&374.1&72&53.3&1	   \\
193&164023.9-484952.4&16:40:23.90&-48:49:52.48&277&25&19.7&1	   \\
194&164023.7-484724.4&16:40:23.77&-48:47:24.46&366.2&56&38.1&1	   \\
195&164022.7-485110.6&16:40:22.78&-48:51:10.67&241.7&26&20.7&1	   \\
196&164022.7-485658.6&16:40:22.70&-48:56:58.69&385.7&47&29&2	   \\
197&164020.7-485417.1&16:40:20.70&-48:54:17.15&259.9&24&20.3&1	   \\
198&164020.5-484756.1&16:40:20.51&-48:47:56.12&321&16&10.8&1	   \\
199&164019.4-485636.2&16:40:19.43&-48:56:36.28&348.4&19&13.9&1	   \\
200&164018.5-485615.5&16:40:18.52&-48:56:15.52&326.4&24&19.3&1	   \\
201&164017.6-484659.6&16:40:17.63&-48:46:59.65&348.9&56&50.6&1	   \\
202&164016.3-484810.9&16:40:16.34&-48:48:10.96&283.2&20&15.7&1	   \\
203&164016.2-485627.3&16:40:16.20&-48:56:27.35&323.2&15&8.8&1	   \\
204&164015.4-484830.1&16:40:15.48&-48:48:30.11&262.9&14&8.5&1	   \\
205&164015.3-485611.9&16:40:15.30&-48:56:11.93&305.4&18&11.2&1	   \\
206&164014.6-484620.8&16:40:14.64&-48:46:20.88&368.6&85&73.1&1	   \\
207&163959.4-485642.8&16:39:59.44&-48:56:42.84&288.8&18&13.7&1	   \\
208&163957.4-485656.4&16:39:57.46&-48:56:56.41&302.5&23&17.9&1	   \\
209&163957.2-485153.6&16:39:57.25&-48:51:53.67&14.2&12&10&1	   \\
210&163951.1-485153.1&16:39:51.13&-48:51:53.16&74.6&16&14.6&1	   \\
211&163950.9-484702.1&16:39:50.96&-48:47:02.14&301.8&21&16.7&2	   \\
212&163949.1-485655.7&16:39:49.19&-48:56:55.76&315.8&23&18.4&1	   \\
213&163947.7-485659.3&16:39:47.77&-48:56:59.31&323.6&22&17.3&1	   \\
214&163944.6-485417.6&16:39:44.66&-48:54:17.69&199.4&9&8.1&2	   \\
215&163936.3-484755.3&16:39:36.39&-48:47:55.36&324.8&43&38.2&1	   \\
216&163934.8-485530.7&16:39:34.86&-48:55:30.79&319.6&22&18&1	   \\
217&163926.1-485147.4&16:39:26.12&-48:51:47.46&321.5&25&20.6&1	   \\
218&163925.4-485007.1&16:39:25.47&-48:50:07.12&344.9&22&18.1&1	   \\
219&163923.2-484958.9&16:39:23.28&-48:49:58.93&368.1&42&26.4&1	   \\
220&163922.9-485302.2&16:39:22.95&-48:53:02.20&359.1&56&51.7&1	   \\
221&164014.3-484928.3&16:40:14.34&-48:49:28.38&212.4&11&9.9&1	   \\
222&164010.4-485738.8&16:40:10.45&-48:57:38.89&363.7&51&34.7&1	   \\
223&163952.8-485755.5&16:39:52.80&-48:57:55.58&366.1&29&14.4&1	   \\
224&163930.7-484724.2&16:39:30.78&-48:47:24.22&385.8&28&12.4&1	   \\
225&163920.5-485142.1&16:39:20.51&-48:51:42.14&376.9&29&15.6&1	   \\
226&164058.2-484935.5&16:40:58.26&-48:49:35.55&604.1&177&146.1&1   \\
227&164055.6-485048.5&16:40:55.66&-48:50:48.52&566&122&85.3&1	   \\
228&164054.4-485144.2&16:40:54.42&-48:51:44.27&550&118&98.9&2	   \\
229&164052.4-485248.1&16:40:52.45&-48:52:48.11&533.1&70&61.6&1	   \\
230&164051.9-484958.9&16:40:51.95&-48:49:58.90&538.2&367&330.1&3   \\
231&164051.5-485008.5&16:40:51.56&-48:50:08.56&532.4&362&324&3	   \\
232&164049.8-485149.1&16:40:49.84&-48:51:49.14&504.8&102&60.5&1	   \\
233&164049.7-485009.9&16:40:49.74&-48:50:09.99&514.5&208&169.2&2   \\
234&164049.4-484828.8&16:40:49.47&-48:48:28.85&541.8&149&124.1&1   \\
235&164048.4-485242.4&16:40:48.47&-48:52:42.47&493.5&104&67.9&1	   \\
236&164046.4-484940.2&16:40:46.49&-48:49:40.23&490.5&184&144.2&3   \\
237&164044.9-485034.9&16:40:44.97&-48:50:34.97&463.5&83&65.9&1	   \\
238&164044.6-485300.6&16:40:44.67&-48:53:00.63&458.5&149&132.3&3   \\
239&164044.4-485226.4&16:40:44.47&-48:52:26.44&452.8&67&50.1&1	   \\
240&164044.3-485101.8&16:40:44.37&-48:51:01.82&453.9&221&203.7&1   \\
241&164043.9-484724.9&16:40:43.91&-48:47:24.96&521.4&178&160.1&1   \\
242&164043.8-484936.7&16:40:43.80&-48:49:36.70&466.1&37&20.8&1	   \\
243&164043.6-484851.6&16:40:43.61&-48:48:51.64&479.5&133&117.1&1   \\
244&164042.3-485404.9&16:40:42.31&-48:54:04.98&449.7&54&38.2&1	   \\
245&164041.0-485112.2&16:40:41.01&-48:51:12.28&419.8&1633&1615.9&5 \\
246&164040.9-484932.8&16:40:40.98&-48:49:32.86&440.7&111&96&1	   \\
247&164040.3-485016.9&16:40:40.36&-48:50:16.98&422.6&193&175.6&1   \\
248&164039.7-485016.2&16:40:39.75&-48:50:16.20&416.9&213&195.9&1   \\
249&164038.2-485423.0&16:40:38.23&-48:54:23.06&417.5&41&22.6&1	   \\
250&164037.4-484845.1&16:40:37.40&-48:48:45.14&426.4&86&69.8&1	   \\
251&164032.3-484706.7&16:40:32.35&-48:47:06.72&439.4&48&33.3&1	   \\
252&164027.4-485716.1&16:40:27.43&-48:57:16.17&428.9&111&95.3&1	   \\
253&164026.9-484623.7&16:40:26.97&-48:46:23.73&432.7&133&117.8&1   \\
254&164026.7-484612.6&16:40:26.72&-48:46:12.65&439.6&142&126.5&1   \\
255&164026.4-484636.7&16:40:26.40&-48:46:36.73&419.1&474&457.8&2   \\
256&164026.3-485703.7&16:40:26.36&-48:57:03.79&412.7&63&46.2&3	   \\
257&164021.9-484558.3&16:40:21.91&-48:45:58.37&423.3&543&527.4&4   \\
258&164016.3-484546.2&16:40:16.34&-48:45:46.25&407.1&77&64.6&1	   \\
259&164016.0-485816.3&16:40:16.07&-48:58:16.32&418.8&31&15.2&1	   \\
260&164013.5-490001.0&16:40:13.50&-49:00:01.04&508.3&198&160&1	   \\
261&164013.0-484356.4&16:40:13.09&-48:43:56.46&498.4&115&97&1	   \\
262&164010.4-484353.6&16:40:10.44&-48:43:53.62&494.4&345&320&1	   \\
263&164009.3-485854.5&16:40:09.32&-48:58:54.57&433.3&89&73.7&1	   \\
264&164007.9-485906.1&16:40:07.98&-48:59:06.19&441.6&59&43.5&1	   \\
265&164007.7-485852.7&16:40:07.74&-48:58:52.73&428&40&26.1&2	   \\
266&164007.2-484436.2&16:40:07.22&-48:44:36.23&446&124&109.9&1	   \\
267&164005.9-485908.6&16:40:05.90&-48:59:08.62&440.2&118&105.7&1   \\
268&164004.9-484518.1&16:40:04.94&-48:45:18.11&400.8&106&92.1&1	   \\
269&164003.9-490024.3&16:40:03.95&-49:00:24.33&512.8&306&272.2&1   \\
270&164000.7-484259.5&16:40:00.79&-48:42:59.57&535&79&57.4&1	   \\
271&163954.7-484456.9&16:39:54.71&-48:44:56.91&419.1&88&73.2&1	   \\
272&163950.6-485903.9&16:39:50.66&-48:59:03.93&437&42&26.6&1	   \\
273&163950.2-484348.7&16:39:50.22&-48:43:48.71&492.6&41&5.1&1	   \\
274&163949.1-490059.0&16:39:49.17&-49:00:59.08&552.9&211&194.6&2   \\
275&163948.9-485825.3&16:39:48.95&-48:58:25.38&402.8&66&51.6&2	   \\
276&163945.8-484450.4&16:39:45.84&-48:44:50.45&442.3&47&33.9&1	   \\
277&163944.6-484430.2&16:39:44.63&-48:44:30.24&465.1&76&61.4&1	   \\
278&163944.6-484044.6&16:39:44.63&-48:40:44.63&683.8&184&156.8&2   \\
279&163942.0-484333.1&16:39:42.01&-48:43:33.15&527.4&89&56.9&1	   \\
280&163939.3-484513.6&16:39:39.33&-48:45:13.66&443.8&175&159.8&1   \\
281&163939.3-484221.6&16:39:39.36&-48:42:21.63&603.6&200&148.5&1   \\
282&163937.6-484446.6&16:39:37.67&-48:44:46.61&475.3&130&117.1&1   \\
283&163930.9-484642.5&16:39:30.95&-48:46:42.57&414.9&62&47.5&2	   \\
284&163929.5-484618.2&16:39:29.51&-48:46:18.27&442.6&159&144.9&1   \\
285&163926.7-484612.0&16:39:26.76&-48:46:12.05&465.3&92&74.9&1	   \\
286&163925.8-484531.4&16:39:25.82&-48:45:31.45&501.9&130&97&1	   \\
287&163923.8-484639.4&16:39:23.87&-48:46:39.40&466.2&118&98.9&3	   \\
288&163922.7-485730.1&16:39:22.79&-48:57:30.12&488&127&96.8&1	   \\
289&163918.1-485046.7&16:39:18.10&-48:50:46.75&406.2&65&49.5&1	   \\
290&163917.7-485500.2&16:39:17.70&-48:55:00.25&445.1&101&86.4&1	   \\
291&163917.0-485356.0&16:39:17.04&-48:53:56.08&428.5&27&13.2&1	   \\
292&163916.3-485454.1&16:39:16.32&-48:54:54.00&454.9&48&34.6&1	   \\
293&163916.3-485230.5&16:39:16.32&-48:52:30.58&419.7&132&118.3&1   \\
294&163912.4-484945.9&16:39:12.40&-48:49:45.90&474.6&141&126.3&1   \\
295&163911.5-485103.4&16:39:11.58&-48:51:03.44&467.7&69&53.6&1	   \\
296&163908.7-485230.3&16:39:08.79&-48:52:30.33&493.7&68&34.5&1	   \\
297&163903.1-484939.6&16:39:03.13&-48:49:39.63&564.7&196&180&1	   \\
298&164103.0-485000.6&16:41:03.06&-48:50:00.68&645.4&127&125.6&4   \\
300&164058.6-485100.6&16:40:58.69&-48:51:00.62&594.5&72&71&1	   \\
301&164056.2-485153.0&16:40:56.28&-48:51:53.00&568.3&67.0&66.3&3   \\
303&164049.8-485219.5&16:40:49.84&-48:52:19.53&505.3&56&9.2&2	   \\
304&164044.2-484834.2&16:40:44.23&-48:48:34.28&492&64&31.3&1	   \\
305&164043.3-484802.4&16:40:43.30&-48:48:02.47&497.7&68&37&1	   \\
306&164039.0-484843.8&16:40:39.01&-48:48:43.85&441.2&36&22.1&1	   \\
307&164037.2-485548.4&16:40:37.20&-48:55:48.44&446.2&31&17.9&1	   \\
308&164033.9-484758.0&16:40:33.96&-48:47:58.03&420.7&44&26.7&1	   \\
309&164018.6-485857.7&16:40:18.67&-48:58:57.71&467.1&29&14&1	   \\
310&164010.7-490051.3&16:40:10.78&-49:00:51.31&550.2&97&63.8&1	   \\
311&164007.4-485829.4&16:40:07.40&-48:58:29.42&404.5&41&24.1&1	   \\
312&164001.6-484355.7&16:40:01.67&-48:43:55.79&479.3&26&14&1	   \\
313&164001.2-484430.5&16:40:01.22&-48:44:30.52&444.3&50&37.8&1	   \\
314&163959.6-490023.8&16:39:59.69&-49:00:23.82&509.8&56&29.3&1	   \\
315&163958.5-490112.4&16:39:58.56&-49:01:12.42&558.3&60&31.8&1	   \\
316&163957.8-484301.1&16:39:57.87&-48:43:01.10&533.1&50&22.2&1	   \\
317&163956.5-484511.7&16:39:56.52&-48:45:11.77&403&25&12.1&1	   \\
318&163953.4-485940.0&16:39:53.46&-48:59:40.08&468.8&27&14.1&1	   \\
319&163950.0-484400.8&16:39:50.06&-48:44:00.84&480.9&57&21.6&1	   \\
320&163937.0-484347.4&16:39:37.05&-48:43:47.46&531.6&76&43.1&1	   \\
321&163934.5-484425.7&16:39:34.52&-48:44:25.71&508.1&66&32.3&1	   \\
322&163925.2-485711.5&16:39:25.25&-48:57:11.52&457.6&65&49.7&4	   \\
323&163924.4-484727.7&16:39:24.42&-48:47:27.76&430.7&58&42&1	   \\
324&163923.8-484741.7&16:39:23.88&-48:47:41.77&426.5&46&32.2&1	   \\
325&163921.7-485753.5&16:39:21.74&-48:57:53.58&511.7&50&36.7&1	   \\
326&163921.5-485732.4&16:39:21.50&-48:57:32.49&498.9&96&69.2&1	   \\
327&163911.2-485524.2&16:39:11.24&-48:55:24.22&512.9&56&24.6&1	   \\
328&163909.7-485335.1&16:39:09.75&-48:53:35.10&493.2&67&34.6&1	   \\
329&163909.3-484831.6&16:39:09.35&-48:48:31.66&527.6&67&41.6&1	   \\
330&163908.1-485023.9&16:39:08.10&-48:50:23.98&507.4&54&20.5&1	   \\
331&163906.6-485636.8&16:39:06.60&-48:56:36.89&586.3&78&67.2&1	   \\
332&163905.6-485136.3&16:39:05.69&-48:51:36.32&523.3&56&24.3&1	   \\
333&163905.4-485557.6&16:39:05.43&-48:55:57.65&578.8&96&75.8&2	   \\
334&163905.6-484852.8&16:39:05.61&-48:48:52.80&554.5&122&109.1&1   \\
337&164021.9-484443.9&16:40:21.92&-48:44:43.91&487.6&45&27.5&1	   \\
338&163957.9-490217.7&16:39:57.90&-49:02:17.72&623.6&52&25.6&1	   \\
339&163953.6-484233.9&16:39:53.60&-48:42:33.96&562.5&56&24.6&1	   \\
340&163907.3-485145.0&16:39:07.39&-48:51:45.09&506.3&80&46.4&1	   \\
341&163846.6-485347.3&16:38:46.62&-48:53:47.31&719.9&142&118.9&1   \\
\enddata
\tablenotetext{a}{BB95 = The number of Bayesian Blocks of greater than
  95\% confidence required to describe the lightcurve.  Any number
  $> 1$ indicates variability at 95\% confidence.}
\end{deluxetable}






























































































































































































































































































































































==> table_10.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrr}
%begin{deluxetable}{123456789012345}
\tabletypesize{\tiny}
\tablecolumns{15}
\tablewidth{0pc}
\tablecaption{Near--IR Observations of X-Ray Sources
\label{nir} }
\tablewidth{0pt}
\tablehead{ \colhead{SRC\#} & \colhead{IR R.A.} & \colhead{IR Dec.} & 
\colhead{offset} & \colhead{off-axis} & \colhead{J} &  \colhead{Jerr}
& \colhead{H} & \colhead{Herr} & \colhead{K} &  \colhead{Kerr}  & \colhead{$Q$} &
\colhead{A$_V$} &  \colhead{model}  & \colhead{flags}}
\startdata
East &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  1 & 16:40:36.70 & -48:52:16.0 & 1.504 & 375.2 & 12.52 & 0.01 & 11.58 & 0.006 & 11.08 & 0.007 & 0.07 & 3.46 & M star & NTT       \\
  2 & 16:40:35.80 & -48:51:06.0 & 0.777 & 369.5 & 13.43 & 0.016 & 12.45 & 0.01 & 11.90 & 0.010 & 0.04 & 1.85 & Disk & NTT 	 \\
  3 & 16:40:34.90 & -48:50:48.0 & 1.524 & 363.2 & 13.64 & 0.018 & 12.84 & 0.012 & 12.62 & 0.014 & 0.44 & 2.24 & Disk & NTT	 \\
  4 & 16:40:33.40 & -48:50:23.0 & 1.015 & 353.6 & 13.52 & 0.017 & 12.74 & 0.011 & 12.50 & 0.014 & 0.35 & 1.49 & Disk & NTT	 \\
  5 & 16:40:32.20 & -48:53:23.0 & 0.614 & 341.8 & 15.38 & 0.04 & 14.56 & 0.029 & 14.23 & 0.032 & 0.25 & 3.65 & HMS & NTT	 \\
  6 & 16:40:32.00 & -48:49:12.0 & 1.439 & 365.2 & 13.58 & 0.017 & 12.73 & 0.011 & 12.30 & 0.012 & 0.13 & 1.2 & Disk & NTT	 \\
  7 & 16:40:31.90 & -48:53:12.0 & 0.426 & 336.7 & 14.20 & 0.023 & 13.37 & 0.016 & 13.12 & 0.019 & 0.41 & 2.31 & -- & NTT	 \\
  8 & 16:40:31.50 & -48:53:12.0 & 0.616 & 332.3 & 13.63 & 0.018 & 12.74 & 0.011 & 12.21 & 0.012 & -0.02 & 0.86 & Disk & NTT	 \\
  9 & 16:40:31.40 & -48:52:12.0 & 1.719 & 321.6 & 16.45 & 0.095 & 14.94 & 0.048 & 14.62 & 0.059 & 0.95 & 10.98 & Disk & NTT	 \\
 10 & 16:40:31.10 & -48:52:49.0 & 0.745 & 324.2 & 14.29 & 0.024 & 13.45 & 0.016 & 13.21 & 0.019 & 0.43 & 2.43 & -- & NTT	 \\
 11 & 16:40:31.00 & -48:49:38.0 & 0.797 & 346.1 & 14.92 & 0.033 & 13.96 & 0.021 & 13.39 & 0.022 & -0.01 & 1.55 & -- & NTT	 \\
 12 & 16:40:30.70 & -48:52:15.0 & 0.682 & 316.3 & 14.09 & 0.022 & 12.60 & 0.011 & 11.36 & 0.008 & -0.63 & 3.45 & Disk & NTT	 \\
 13 & 16:40:30.70 & -48:50:26.0 & 0.573 & 327.5 & 15.17 & 0.037 & 14.35 & 0.026 & 14.00 & 0.030 & 0.22 & 4.1 & HMS & NTT	 \\
 14 & 16:40:30.20 & -48:51:09.0 & 0.632 & 314.4 & 14.65 & 0.029 & 13.61 & 0.018 & 13.21 & 0.019 & 0.36 & 3.97 & -- & NTT	 \\
 15 & 16:40:30.20 & -48:49:59.0 & 1.424 & 331.4 & 17.51 & 0.117 & 16.81 & 0.106 & 16.53 & 0.129 & 0.23 & 0.28 & -- & NTT	 \\
 16 & 16:40:29.40 & -48:52:46.0 & 0.399 & 307.2 & 12.74 & 0.011 & 11.95 & 0.008 & 11.70 & 0.009 & 0.36 & 1.67 & Disk & NTT	 \\
 17 & 16:40:28.60 & -48:52:37.0 & 0.886 & 298.2 & 14.45 & 0.026 & 13.63 & 0.018 & 13.33 & 0.020 & 0.31 & 1.74 & Disk & NTT	 \\
 18 & 16:40:28.20 & -48:53:52.0 & 1.099 & 313.4 & 14.31 & 0.024 & 13.39 & 0.015 & 13.07 & 0.018 & 0.39 & 3.05 & Disk & NTT	 \\
 19 & 16:40:27.60 & -48:50:27.0 & 1.019 & 298.2 & 13.75 & 0.019 & 12.92 & 0.012 & 12.67 & 0.014 & 0.41 & 2.34 & Disk & NTT	 \\
 20 & 16:40:27.10 & -48:52:21.0 & 0.790 & 281.5 & 13.47 & 0.016 & 12.88 & 0.012 & 12.69 & 0.015 & 0.26 & 1.42 & -- & NTT	 \\
 21 & 16:40:26.90 & -48:51:18.0 & 0.687 & 280.1 & 13.82 & 0.02 & 12.98 & 0.013 & 12.74 & 0.016 & 0.43 & 2.54 & Disk & NTT	 \\
 22 & 16:40:26.80 & -48:52:00.0 & 0.752 & 276.9 & 13.97 & 0.021 & 13.23 & 0.014 & 12.99 & 0.017 & 0.34 & 1.5 & HMS & NTT	 \\
 23 & 16:40:26.60 & -48:51:05.0 & 0.740 & 279.1 & 14.56 & 0.027 & 13.68 & 0.018 & 13.43 & 0.021 & 0.46 & 2.98 & -- & NTT	 \\
 24 & 16:40:24.80 & -48:52:00.0 & 0.951 & 256.9 & 14.16 & 0.023 & 13.24 & 0.014 & 12.97 & 0.017 & 0.44 & 3.23 & Disk & NTT	 \\
 25 & 16:40:24.40 & -48:53:33.0 & 1.380 & 271.8 & 14.80 & 0.031 & 13.91 & 0.02 & 13.61 & 0.023 & 0.40 & 2.87 & Disk & NTT	 \\
 26 & 16:40:24.10 & -48:53:33.0 & 1.057 & 268.8 & 15.48 & 0.042 & 14.45 & 0.026 & 14.25 & 0.032 & 0.68 & 5.41 & Disk & NTT	 \\
 27 & 16:40:23.90 & -48:50:52.0 & 1.030 & 256.2 & 14.97 & 0.034 & 14.07 & 0.024 & 13.65 & 0.027 & 0.17 & 1.74 & -- & NTT	 \\
 28 & 16:40:23.20 & -48:51:15.0 & 0.373 & 245 & 13.74 & 0.018 & 12.85 & 0.012 & 12.54 & 0.013 & 0.36 & 2.66 & -- & NTT	 \\
 29 & 16:40:22.90 & -48:53:08.0 & 0.470 & 250.2 & 11.59 & 0.007 & 10.14 & 0.003 & 9.48 & 0.003 & 0.33 & 7.53 & Disk & NTT	 \\
 30 & 16:40:22.00 & -48:48:38.0 & 1.040 & 301.4 & 11.83 & 0.007 & 11.52 & 0.006 & 11.37 & 0.008 & 0.04 & -- & -- & NTT		 \\
 31 & 16:40:22.00 & -48:55:32.0 & 0.489 & 316.4 & 15.02 & 0.034 & 14.16 & 0.022 & 13.87 & 0.026 & 0.37 & 2.38 & -- & NTT	 \\
 32 & 16:40:21.50 & -48:52:44.0 & 0.604 & 230.1 & 12.80 & 0.012 & 11.82 & 0.007 & 11.16 & 0.007 & -0.13 & 1.18 & -- & NTT	 \\
 33 & 16:40:21.10 & -48:52:19.0 & 0.224 & 222.3 & 14.53 & 0.027 & 13.65 & 0.018 & 13.26 & 0.019 & 0.21 & 4.77 & HMS & NTT	 \\
 34 & 16:40:20.40 & -48:50:12.0 & 1.143 & 236.6 & 14.41 & 0.026 & 13.63 & 0.018 & 13.34 & 0.021 & 0.28 & 1.25 & -- & NTT	 \\
 35 & 16:40:20.40 & -48:52:46.0 & 0.557 & 219.9 & 14.90 & 0.032 & 13.98 & 0.021 & 13.58 & 0.022 & 0.25 & 2.41 & Disk & NTT	 \\
 36 & 16:40:20.10 & -48:51:03.0 & 0.527 & 217.1 & 13.65 & 0.018 & 12.80 & 0.012 & 12.36 & 0.012 & 0.12 & 1.16 & -- & NTT	 \\
 37 & 16:40:20.20 & -48:50:19.0 & 1.291 & 231.5 & 12.25 & 0.009 & 11.38 & 0.006 & 10.88 & 0.006 & 0.02 & 3.02 & M star & NTT	 \\
 38 & 16:40:19.90 & -48:49:39.0 & 0.898 & 248.4 & 14.59 & 0.028 & 13.57 & 0.017 & 12.96 & 0.017 & 0.00 & 4.52 & M star & NTT	 \\
 39 & 16:40:19.60 & -48:52:50.0 & 0.796 & 213 & 12.52 & 0.01 & 12.06 & 0.008 & 11.76 & 0.009 & -0.05 & -- & Disk & NTT		 \\
 40 & 16:40:19.10 & -48:50:11.0 & 0.472 & 226.2 & 12.46 & 0.01 & 11.17 & 0.005 & 10.22 & 0.004 & -0.32 & 3.11 & Disk & NTT	 \\
 41 & 16:40:19.10 & -48:52:42.0 & 1.055 & 206.5 & 15.19 & 0.037 & 13.96 & 0.02 & 13.35 & 0.020 & 0.21 & 8.07 & HMS & NTT	 \\
177 & 16:40:36.20 & -48:53:53.0 & 0.526 & 388.5 & 14.98 & 0.033 & 14.07 & 0.022 & 13.63 & 0.024 & 0.18 & 5.64 & HMS & NTT	 \\
178 & 16:40:35.60 & -48:53:27.0 & 0.471 & 375.3 & 15.05 & 0.034 & 14.09 & 0.022 & 13.62 & 0.023 & 0.17 & 2.39 & -- & NTT	 \\
179 & 16:40:33.80 & -48:54:31.0 & 2.774 & 379.9 & 15.68 & 0.046 & 15.04 & 0.037 & 14.74 & 0.043 & 0.12 & 4.15 & HMS & NTT	 \\
180 & 16:40:33.50 & -48:50:42.0 & 1.09 & 350 & 14.43 & 0.026 & 13.57 & 0.017 & 13.33 & 0.020 & 0.44 & 2.7 & Disk & NTT		 \\
181 & 16:40:33.10 & -48:50:01.0 & 0.613 & 357.5 & 15.01 & 0.034 & 14.38 & 0.026 & 14.12 & 0.032 & 0.18 & 3.01 & HMS & NTT	 \\
182 & 16:40:32.90 & -48:54:37.0 & 0.517 & 374.3 & 16.13 & 0.057 & 15.11 & 0.039 & 14.80 & 0.044 & 0.49 & 4.42 & -- & NTT	 \\
183 & 16:40:32.80 & -48:51:10.0 & 1.164 & 338.7 & 15.40 & 0.041 & 14.17 & 0.023 & 13.53 & 0.023 & 0.13 & 4.61 & -- & NTT	 \\
184 & 16:40:30.50 & -48:54:43.0 & 1.602 & 355.2 & 15.13 & 0.036 & 14.28 & 0.026 & 13.90 & 0.029 & 0.21 & 2.36 & M star & NTT	 \\
185 & 16:40:29.20 & -48:52:24.0 & 0.92 & 302.6 & 11.56 & 0.006 & 11.25 & 0.005 & 11.06 & 0.007 & 0.00 & -- & -- & NTT		 \\
186 & 16:40:28.50 & -48:49:40.0 & 2.738 & 322.7 & 13.26 & 0.015 & 12.61 & 0.011 & 12.33 & 0.012 & 0.17 & 3.4 & HMS & NTT	 \\
187 & 16:40:27.20 & -48:54:37.0 & 1.807 & 323.6 & 14.92 & 0.032 & 14.02 & 0.021 & 13.73 & 0.024 & 0.40 & 2.88 & Disk & NTT	 \\
188 & 16:40:25.80 & -48:48:37.0 & 0.798 & 331.6 & 13.68 & 0.018 & 12.77 & 0.011 & 12.48 & 0.013 & 0.42 & 3.09 & -- & NTT	 \\
189 & 16:40:25.00 & -48:50:59.0 & 2.118 & 264.9 & 13.73 & 0.018 & 12.78 & 0.012 & 12.29 & 0.012 & 0.13 & 2.13 & -- & NTT	 \\
190 & 16:40:24.50 & -48:51:41.0 & 0.618 & 254.8 & 17.66 & 0.128 & 17.13 & 0.132 & 16.49 & 0.115 & -0.57 & -- & -- & NTT	 \\
191 & 16:40:24.20 & -48:54:43.0 & 0.459 & 303 & 14.09 & 0.022 & 13.07 & 0.013 & 12.38 & 0.013 & -0.15 & 4.88 & M star & NTT	 \\
192 & 16:40:23.90 & -48:47:14.0 & 1.189 & 374.1 & 15.61 & 0.045 & 14.82 & 0.03 & 14.31 & 0.032 & -0.08 & 2.55 & M star & NTT	 \\
193 & 16:40:24.00 & -48:49:52.0 & 1.115 & 277 & 15.77 & 0.048 & 14.97 & 0.033 & 14.71 & 0.039 & 0.35 & 1.72 & Disk & NTT	 \\
194 & 16:40:23.80 & -48:47:24.0 & 0.538 & 366.2 & 13.84 & 0.019 & 12.86 & 0.012 & 12.24 & 0.012 & -0.07 & 1.44 & -- & NTT	 \\
195 & 16:40:22.80 & -48:51:10.0 & 0.707 & 241.7 & 14.09 & 0.022 & 13.10 & 0.013 & 12.53 & 0.014 & 0.02 & 1.93 & -- & NTT	 \\
196 & 16:40:22.80 & -48:56:57.0 & 1.95 & 385.7 & 14.70 & 0.029 & 13.76 & 0.019 & 13.45 & 0.022 & 0.41 & 3.32 & -- & NTT	 \\
197 & 16:40:20.70 & -48:54:18.0 & 0.851 & 259.9 & 14.26 & 0.024 & 13.54 & 0.017 & 13.26 & 0.019 & 0.23 & 3.06 & HMS & NTT	 \\
198 & 16:40:20.50 & -48:47:55.0 & 1.131 & 321 & 12.68 & 0.011 & 11.76 & 0.007 & 11.29 & 0.007 & 0.12 & 1.75 & -- & NTT	 \\
199 & 16:40:19.40 & -48:56:37.0 & 0.784 & 348.4 & 15.83 & 0.05 & 14.89 & 0.033 & 14.58 & 0.038 & 0.41 & 3.28 & -- & NTT	 \\
226 & 16:40:58.26 & -48:49:35.6 & 0.274 & 604.1 & 14.47 & 0.0733 & 13.62 & 0.101 & 13.27 & 0.077 & 0.27 & 1.88 & -- & AAA	 \\
228 & 16:40:54.42 & -48:51:44.3 & 1.227 & 550 & 15.16 & 0.0503 & 14.31 & 0.0527 & 13.95 & 0.050 & 0.24 & 1.73 & -- & AAA	 \\
229 & 16:40:52.45 & -48:52:48.1 & 0.692 & 533.1 & 13.94 & 0.0609 & 12.95 & 0.0666 & 12.46 & 0.046 & 0.15 & 2.47 & -- & AAA \\
230 & 16:40:51.95 & -48:49:58.9 & 0.287 & 538.2 & 13.62 & 0.0319 & 12.88 & 0.0352 & 12.62 & 0.030 & 0.30 & 1.03 & -- & AAA \\
231 & 16:40:51.56 & -48:50:08.6 & 0.610 & 532.4 & 13.67 & 0.0272 & 12.82 & 0.0318 & 12.52 & 0.024 & 0.32 & 2.06 & -- & AAA \\
232 & 16:40:49.84 & -48:51:49.1 & 0.785 & 504.8 & 15.59 & 0.096 & 14.72 & 0.1064 & 14.40 & 0.100 & 0.32 & 2.25 & Disk & AAA	 \\
233 & 16:40:49.74 & -48:50:10.0 & 0.942 & 514.5 & 12.75 & 0.0272 & 11.93 & 0.0241 & 11.74 & 0.027 & 0.49 & 2.61 & -- & AAA \\
234 & 16:40:49.47 & -48:48:28.9 & 0.309 & 541.8 & 13.63 & 0.0272 & 12.83 & 0.0415 & 12.37 & 0.034 & 0.04 & 0.33 & -- & AAA \\
235 & 16:40:48.47 & -48:52:42.5 & 1.159 & 493.5 & 14.03 & 0.0348 & 13.13 & 0.0335 & 12.86 & 0.038 & 0.43 & 3.05 & -- & AAA	 \\
236 & 16:40:46.49 & -48:49:40.2 & 0.879 & 490.5 & 14.51 & 0.0654 & 13.65 & 0.1108 & 13.31 & 0.083 & 0.29 & 2.05 & -- & ABA \\
237 & 16:40:44.97 & -48:50:35.0 & 1.223 & 463.5 & 14.28 & 0.0666 & 13.49 & 0.091 & 13.24 & 0.072 & 0.38 & 1.83 & -- & AAA	 \\
238 & 16:40:44.67 & -48:53:00.6 & 0.427 & 458.5 & 14.70 & 0.0289 & 13.81 & 0.03 & 13.58 & 0.037 & 0.50 & 3.32 & Disk & AAA	 \\
239 & 16:40:44.47 & -48:52:26.4 & 0.610 & 452.8 & 14.27 & 0.0319 & 13.48 & 0.0335 & 13.17 & 0.026 & 0.27 & 1.28 & -- & AAA \\
240 & 16:40:44.37 & -48:51:01.8 & 0.758 & 453.9 & 13.68 & 0.0319 & 12.86 & 0.0472 & 12.52 & 0.040 & 0.24 & 1.4 & -- & AAA	 \\
241 & 16:40:43.91 & -48:47:25.0 & 0.623 & 521.4 & 12.77 & -- & 12.03 & -- & 11.81 & 0.031 & 0.36 & -- & -- & UUA	 \\
242 & 16:40:43.80 & -48:49:36.7 & 0.068 & 466.1 & 15.30 & 0.1274 & 13.50 & -- & 13.22 & -- & 1.32 & -- & -- & BUU \\
243 & 16:40:43.61 & -48:48:51.6 & 0.087 & 479.5 & 8.98 & 0.027 & 8.85 & 0.0218 & 8.76 & 0.021 & -0.02 & -- & Disk & AAA	 \\
244 & 16:40:42.31 & -48:54:05.0 & 0.678 & 449.7 & 15.04 & 0.0677 & 14.04 & 0.0785 & 13.40 & 0.057 & -0.09 & 4.5 & M star & AAA	 \\
245 & 16:40:41.01 & -48:51:12.3 & 0.468 & 419.8 & 10.15 & 0.0239 & 9.74 & 0.0241 & 9.54 & 0.023 & 0.06 & -- & Disk & AAA	 \\
246 & 16:40:40.98 & -48:49:32.9 & 1.015 & 440.7 & 11.46 & 0.0334 & 11.04 & 0.0486 & 10.96 & 0.038 & 0.28 & -- & Disk & AAA	 \\
247 & 16:40:40.36 & -48:50:17.0 & 0.279 & 422.6 & 13.23 & 0.0466 & 12.18 & 0.043 & 11.45 & 0.029 & -0.18 & 1.6 & -- & AAA	 \\
248 & 16:40:39.75 & -48:50:16.2 & 0.406 & 416.9 & 12.02 & 0.0402 & 11.56 & 0.0617 & 11.40 & 0.058 & 0.18 & -- & -- & AAA	 \\
249 & 16:40:38.40 & -48:54:24.0 & 1.944 & 417.5 & 17.70 & 0.125 & 16.53 & 0.092 & 16.58 & 0.159 & 1.25 & 9.37 & Disk & NTT	 \\
250 & 16:40:37.40 & -48:48:44.0 & 1.140 & 426.4 & 14.61 & 0.028 & 13.76 & 0.019 & 13.50 & 0.022 & 0.42 & 2.57 & Disk & NTT	 \\
251 & 16:40:32.30 & -48:47:07.0 & 0.583 & 439.4 & 14.71 & 0.03 & 13.70 & 0.02 & 13.22 & 0.021 & 0.18 & 2.79 & Disk & NTT	 \\
252 & 16:40:27.50 & -48:57:17.0 & 1.082 & 428.9 & 14.57 & 0.027 & 13.68 & 0.019 & 13.43 & 0.022 & 0.48 & 3.2 & Disk & NTT	 \\
253 & 16:40:27.00 & -48:46:24.0 & 0.399 & 432.7 & 13.43 & 0.016 & 12.57 & 0.011 & 12.10 & 0.011 & 0.06 & 2.82 & M star & NTT	 \\
254 & 16:40:26.70 & -48:46:12.0 & 0.670 & 439.6 & 13.30 & 0.015 & 12.49 & 0.01 & 12.16 & 0.012 & 0.25 & 1.9 & M star & NTT	 \\
255 & 16:40:26.40 & -48:46:37.0 & 0.261 & 419.1 & 12.64 & 0.011 & 11.91 & 0.008 & 11.57 & 0.009 & 0.15 & 0.19 & -- & NTT	 \\
256 & 16:40:26.30 & -48:57:05.0 & 1.339 & 412.7 & 14.46 & 0.026 & 13.27 & 0.015 & 12.84 & 0.016 & 0.45 & 5.72 & Disk & NTT	 \\
257 & 16:40:21.90 & -48:45:58.0 & 0.386 & 423.3 & 12.30 & 0.009 & 11.54 & 0.006 & 11.05 & 0.007 & -0.06 & -- & Disk & NTT	 \\
298 & 16:41:03.06 & -48:50:00.7 & 3.246 & 645.4 & 13.70 & -- & 13.09 & 0.043 & 12.89 & 0.047 & 0.26 & -- & -- & UAA	 \\
300 & 16:40:58.69 & -48:51:00.6 & 0.668 & 594.5 & 14.37 & 0.055 & 13.07 & 0.0513 & 12.57 & 0.037 & 0.44 & 6.71 & Disk & AAA	 \\
303 & 16:40:49.84 & -48:52:19.5 & 1.667 & 505.3 & 14.60 & -- & 14.49 & 0.1021 & 14.28 & 0.126 & -0.25 & -- & -- & UAB	 \\
304 & 16:40:44.23 & -48:48:34.3 & 0.637 & 492 & 14.83 & 0.0906 & 13.95 & 0.083 & 13.77 & 0.064 & 0.57 & 3.49 & -- & AAA	 \\
305 & 16:40:43.30 & -48:48:02.5 & 1.044 & 497.7 & 13.73 & 0.0503 & 12.99 & 0.0553 & 12.66 & 0.046 & 0.17 & 4.2 & HMS & AAA	 \\
306 & 16:40:39.01 & -48:48:43.9 & 0.785 & 441.2 & 11.18 & 0.0256 & 10.95 & 0.0281 & 10.83 & 0.021 & 0.01 & -- & Disk & AAA	 \\
307 & 16:40:37.20 & -48:55:46.0 & 2.431 & 446.2 & 14.78 & 0.03 & 14.05 & 0.022 & 13.85 & 0.027 & 0.39 & 1.32 & Disk & NTT	 \\
308 & 16:40:33.90 & -48:47:56.0 & 2.113 & 420.7 & 14.89 & 0.037 & 14.30 & 0.034 & 14.01 & 0.037 & 0.08 & 4.27 & HMS & NTT	 \\
337 & 16:40:21.92 & -48:44:43.9 & 2.506 & 487.6 & 13.98 & 0.0453 & 13.02 & 0.0433 & 12.59 & 0.042 & 0.21 & 5.42 & HMS & AAA	 \\
342 & 16:40:56.99 & -48:59:02.9 & 3.141 & 716.9 & 15.76 & 0.0744 & 14.66 & 0.0678 & 14.16 & 0.059 & 0.25 & 4.00 & Disk & AAA	 \\
401 & 16:40:28.3 &  -48:49:56.6 & 1.966 & 313.3 & 14.15 & 0.03 & 13.48& 0.04 & 13.37 & 0.0366 &  0.48 & 1.20 & -- &AAA\\
402 & 16:40:27.5 &  -48:50:40.0 & 0.227 & 293.4 & 19.16 & 0.33 & --  &--& -- & -- &   -- & -- &--& NTT\\
403 & 16:40:27.4 &  -48:51:17.0 & 0.624 & 285.0 & 17.50 & 0.21 & -- & -- & 16.09 & 0.218 &  -- & -- &--& NTT\\
406 & 16:40:22.5 &  -48:52:31.0 & 0.812 & 237.0 & 17.01 & 0.09 & 16.56 & 0.08 & 16.28 & 0.099 & -0.03 & 0.00 & --&NTT\\
409 & 16:40:21.1 &  -48:52:01.0 & 1.223 & 220.8 & 16.90 & 0.09 & 15.82 & 0.06 & 15.31 & 0.058 & 0.21 & 3.66 &--& NTT\\
410 & 16:40:19.9 &  -48:49:46.0 & 0.941 & 246.6 & 16.07 & 0.06 & 14.83 & 0.03 & 14.38 & 0.034 & 0.48 & 6.35 & --& NTT\\
411 & 16:40:19.7 &  -48:53:14.0 & 0.684 & 221.4 & 16.18 & 0.06 & 15.20 & 0.04 & 14.76 & 0.04 & 0.23 & 2.84 & --& NTT\\
474 & 16:40:39.2 &  -48:48:01.9 & 0.539 & 462.6 & 13.48 & 0.04 & 12.61 & 0.04 & 12.26 & 0.03 & -0.52 & 7.11 & -- & EAA\\
475 & 16:40:26.5 &  -48:57:44.8 & 2.133 & 444.6 & 17.39 & 0.11 & 16.29 & 0.09 & 15.94 & 0.12  & -- & -- &--& NTT\\
476 & 16:40:26.8 &  -48:58:57.2 & 1.374 & 423.1 & 15.68 & 0.07 & 13.57 & 0.02 & 12.62 & 0.0199 & 0.50 & 14.38 & --& AAA\\
481 & 16:40:21.7 &  -48:46:38.0 & 3.056 & 504.0 & 14.58 & 0.05 & 13.98 & 0.05 & 13.60 & 0.0462 & -0.05 & 0.00 & --& AAA\\
482 & 16:40:38.6 &  -48:59:48.7 & 3.394 & 480.2 & 13.91 & 0.04 & 13.05 & 0.03 & 12.75 & 0.0315 & 0.35 & 2.30 & --&  AAA\\
486 & 16:40:33.2 &  -48:56:11.0 & 0.748 & 425.4 & 15.18 & 0.04 & 14.04 & 0.02 & 13.64 & 0.025 & 0.46 & 5.37 & --& NTT\\
\tableline
North &  &  &  &  &  &  &  &  &  &  &  &  &  &                                                                            \\
 46 & 16:40:16.20 & -48:47:09.0 & 0.722 & 333 & 14.03 & 0.022 & 13.23 & 0.015 & 12.94 & 0.017 & 0.33 & 1.68 & -- & NTT	  \\
 59 & 16:40:12.30 & -48:46:37.0 & 0.952 & 344 & 14.72 & 0.029 & 13.64 & 0.018 & 13.21 & 0.019 & 0.34 & 4.27 & -- & NTT	  \\
 60 & 16:40:12.10 & -48:48:31.0 & 0.992 & 241.6 & 16.42 & 0.066 & 13.78 & 0.019 & 11.57 & 0.009 & -1.13 & 11.51 & Disk & NTT	  \\
 61 & 16:40:12.00 & -48:48:16.0 & 1.156 & 253.6 & 12.56 & 0.01 & 11.23 & 0.005 & 10.48 & 0.005 & 0.06 & 5.18 & Disk & NTT	  \\
133 & 16:39:58.40 & -48:46:52.0 & 1.456 & 300.8 & 14.85 & 0.031 & 13.86 & 0.02 & 13.36 & 0.020 & 0.14 & 6.98 & HMS & NTT	  \\
134 & 16:39:57.70 & -48:45:56.0 & 0.967 & 357.5 & 13.74 & 0.019 & 12.74 & 0.011 & 12.30 & 0.012 & 0.26 & 3.14 & Disk & NTT	  \\
146 & 16:39:51.40 & -48:46:45.0 & 0.889 & 317.1 & 11.70 & 0.007 & 11.13 & 0.005 & 10.85 & 0.006 & 0.10 & 0.1 & M star & NTT	  \\
201 & 16:40:17.60 & -48:47:00.0 & 0.449 & 348.9 & 14.27 & 0.024 & 13.22 & 0.014 & 12.54 & 0.014 & -0.12 & 1.77 & -- & NTT	  \\
202 & 16:40:16.40 & -48:48:11.0 & 0.580 & 283.2 & 14.51 & 0.027 & 13.60 & 0.017 & 13.21 & 0.019 & 0.26 & 4.36 & HMS & NTT	  \\
204 & 16:40:15.50 & -48:48:31.0 & 0.905 & 262.9 & 16.71 & 0.079 & 15.35 & 0.042 & 14.67 & 0.042 & 0.20 & 9.3 & HMS & NTT	  \\
206 & 16:40:14.70 & -48:46:20.0 & 1.053 & 368.6 & 14.29 & 0.024 & 13.06 & 0.014 & 12.52 & 0.014 & 0.31 & 5.53 & Disk & NTT	  \\
211 & 16:39:51.00 & -48:47:01.0 & 1.207 & 301.8 & 13.78 & 0.019 & 13.34 & 0.015 & 13.21 & 0.019 & 0.21 & -- & -- & NTT		  \\
258 & 16:40:16.30 & -48:45:45.0 & 1.312 & 407.1 & 14.82 & 0.031 & 13.96 & 0.021 & 13.65 & 0.024 & 0.34 & 2.26 & -- & NTT	  \\
262 & 16:40:10.44 & -48:43:53.6 & 0.734 & 494.4 & 12.67 & 0.0289 & 11.61 & 0.0296 & 11.22 & 0.023 & 0.39 & 4.3 & Disk & AAA	  \\
266 & 16:40:07.22 & -48:44:36.2 & 1.854 & 446 & 16.81 & -- & 14.92 & 0.0827 & 14.15 & 0.067 & 0.58 & -- & -- & UAA	  \\
268 & 16:40:04.94 & -48:45:18.1 & 0.491 & 400.8 & 15.35 & -- & 14.79 & 0.1087 & 14.44 & 0.103 & -0.03 & -- & -- & UAA	  \\
270 & 16:40:00.79 & -48:42:59.6 & 3.147 & 535 & 15.50 & 0.148 & 13.95 & 0.121 & 13.39 & 0.107 & 0.59 & 9.66 & Disk & BBA	  \\
271 & 16:39:54.71 & -48:44:56.9 & 0.273 & 419.1 & 12.59 & -- & 12.03 & 0.0348 & 11.71 & -- & 0.00 & -- & -- & UAU  \\
273 & 16:39:50.22 & -48:43:48.7 & 2.526 & 492.6 & 15.68 & 0.0766 & 15.00 & 0.0921 & 14.44 & -- & -0.28 & -- & -- & AAU\\
276 & 16:39:45.84 & -48:44:50.5 & 0.539 & 442.3 & 12.66 & 0.0227 & 12.19 & 0.0214 & 12.08 & 0.029 & 0.28 & -- & Disk & AAA	  \\
277 & 16:39:44.63 & -48:44:30.2 & 1.039 & 465.1 & 13.96 & 0.0505 & 12.73 & 0.0604 & 11.88 & 0.042 & -0.23 & 2.92 & -- & AAA  \\
278 & 16:39:44.63 & -48:40:44.6 & 1.348 & 683.8 & 14.56 & 0.09 & 13.75 & 0.1417 & 10.98 & -- & -3.89 & -- & -- & ABU  \\
312 & 16:40:01.67 & -48:43:55.8 & 0.706 & 479.3 & 15.23 & 0.0798 & 14.07 & 0.0602 & 13.28 & 0.078 & -0.17 & 2.65 & -- & AAA  \\
316 & 16:39:57.87 & -48:43:01.1 & 3.446 & 533.1 & 15.77 & 0.1243 & 14.40 & 0.0858 & 13.81 & 0.079 & 0.38 & 7.12 & -- & BAA	  \\
319 & 16:39:50.06 & -48:44:00.8 & 1.104 & 480.9 & 14.02 & 0.0214 & 12.75 & 0.0219 & 12.13 & 0.021 & 0.24 & 7.97 & HMS & AAA	  \\
339 & 16:39:53.60 & -48:42:34.0 & 2.515 & 562.5 & 12.57 & 0.0272 & 12.15 & 0.0268 & 12.10 & 0.030 & 0.34 & -- & -- & AAA	  \\
419 & 16:40:06.10 &  -48:47:28.0 & 0.791 & 276.0 & 17.13 & 0.09 & 15.17 & 0.04 & 14.45 & 0.035 &  0.74 & 14.15 & -- &NTT\\
432 & 16:39:54.40 &  -48:48:33.0 & 0.888 & 205.2 & 16.56 & 0.07 & 15.74 & 0.05 & 15.25 & 0.054 & -0.01 & 0.22 & -- &NTT\\
456 & 16:40:06.80 &  -48:47:09.0 & 1.819 & 295.2 & 16.92 & 0.09 & 15.76 & 0.05 & 15.43 & 0.058 &  0.60 & 6.21 & -- &NTT\\
\tableline											  
RCW~108--IR &  &  &  &  &  &  &  &  &  &  &  &  &  & 										  \\
 42 & 16:40:18.80 & -48:49:43.0 & 2.458 & 239.3 & 18.53 & 0.212 & 17.05 & 0.107 & 16.80 & 0.140 & 1.05 & -- & -- & NTT	  \\
 44 & 16:40:18.00 & -48:49:10.0 & 0.728 & 251.1 & 16.52 & 0.069 & 15.19 & 0.038 & 14.50 & 0.037 & 0.17 & 5.81 & Disk & NTT	  \\
 47 & 16:40:15.90 & -48:53:33.0 & 0.926 & 195.8 & 12.56 & 0.01 & 12.33 & 0.009 & 12.24 & 0.012 & 0.07 & -- & Disk & NTT		  \\
 48 & 16:40:15.50 & -48:54:17.0 & 0.824 & 218.8 & 14.76 & 0.03 & 13.67 & 0.018 & 13.13 & 0.018 & 0.17 & 3.54 & -- & NTT	  \\
 50 & 16:40:14.40 & -48:52:53.0 & 1.206 & 165.2 & 14.83 & 0.031 & 13.58 & 0.017 & 12.82 & 0.016 & -0.04 & 6.67 & M star & NTT	  \\
 51 & 16:40:14.30 & -48:50:17.0 & 0.913 & 182.5 & 16.80 & 0.078 & 15.98 & 0.056 & -- & -- & -- & -- & -- & NTT	  \\
 52 & 16:40:14.30 & -48:51:02.0 & 0.839 & 162.2 & 15.43 & 0.041 & 13.20 & 0.014 & 11.73 & 0.009 & -0.27 & 11.87 & Disk & NTT	  \\
 56 & 16:40:13.20 & -48:53:05.0 & 0.297 & 159.4 & 16.09 & 0.056 & 14.87 & 0.034 & 14.36 & 0.036 & 0.36 & 5.67 & Disk & NTT	  \\
 57 & 16:40:12.80 & -48:51:13.0 & 0.810 & 144.9 & 19.46 & 0.322 & 16.44 & 0.073 & 14.90 & 0.046 & 0.41 & -- & -- & NTT	  \\
 58 & 16:40:12.60 & -48:52:33.0 & 0.749 & 142.7 & 17.24 & 0.098 & 15.92 & 0.059 & 15.12 & 0.054 & -0.03 & 12.74 & HMS & NTT	  \\
 62 & 16:40:12.00 & -48:48:59.0 & 0.829 & 218.3 & 14.49 & 0.027 & 12.17 & 0.009 & 10.72 & 0.006 & -0.14 & 13.24 & Disk & NTT	  \\
 63 & 16:40:11.60 & -48:51:34.0 & 0.151 & 129 & 18.33 & 0.163 & 15.93 & 0.055 & 14.69 & 0.041 & 0.30 & 16.13 & Disk & NTT	  \\
 65 & 16:40:10.80 & -48:52:32.0 & 0.525 & 125.1 & 16.28 & 0.061 & 14.71 & 0.029 & 14.00 & 0.027 & 0.37 & 8.93 & -- & NTT	  \\
 66 & 16:40:10.90 & -48:50:49.0 & 1.219 & 135.7 & 14.11 & 0.022 & 13.54 & 0.017 & 13.34 & 0.020 & 0.23 & 1.76 & HMS & NTT	  \\
 67 & 16:40:10.80 & -48:54:26.0 & 1.207 & 192.6 & 15.44 & 0.042 & 14.41 & 0.027 & 13.98 & 0.032 & 0.32 & 3.71 & Disk & NTT	  \\
 68 & 16:40:10.70 & -48:52:39.0 & 0.695 & 126 & 16.00 & 0.054 & 14.42 & 0.027 & 13.68 & 0.025 & 0.32 & 8.75 & Disk & NTT	  \\
 69 & 16:40:10.60 & -48:53:03.0 & 0.311 & 136.4 & 16.11 & 0.056 & 13.99 & 0.02 & 12.76 & 0.015 & 0.04 & 18.8 & HMS & NTT	  \\
 70 & 16:40:10.53 & -48:51:24.5 & 0.174 & 120.5 & 15.77 & 0.0755 & 13.77 & 0.0397 & 12.98 & 0.046 & 0.67 & 14.18 & Disk & AAA \\
 71 & 16:40:10.60 & -48:53:40.0 & 0.904 & 157.5 & 15.77 & 0.048 & 14.37 & 0.025 & 13.78 & 0.026 & 0.40 & 7.47 & -- & NTT	  \\
 73 & 16:40:10.40 & -48:52:50.0 & 0.326 & 128.1 & 16.96 & 0.084 & 15.04 & 0.034 & 14.09 & 0.029 & 0.30 & 11.69 & Disk & NTT	  \\
 74 & 16:40:10.20 & -48:54:25.0 & 1.570 & 188.3 & 15.05 & 0.034 & 14.04 & 0.022 & 13.57 & 0.024 & 0.23 & 5.71 & HMS & NTT	  \\
 76 & 16:40:08.90 & -48:51:47.0 & 0.598 & 100.5 & 18.56 & 0.176 & 14.95 & 0.032 & 12.88 & 0.016 & 0.08 & 26.01 & Disk & NTT	  \\
 78 & 16:40:08.70 & -48:51:08.0 & 0.398 & 108.8 & 16.11 & 0.056 & 14.26 & 0.023 & 13.44 & 0.021 & 0.46 & 11.85 & Disk & NTT	  \\
 80 & 16:40:08.30 & -48:51:28.0 & 0.430 & 98.7 & 16.69 & 0.073 & 16.17 & 0.059 & 15.93 & 0.075 & 0.12 & 3.12 & HMS & NTT	  \\
 81 & 16:40:07.90 & -48:50:36.0 & 0.--  & 119.7 & 17.38 & 0.102 & 15.23 & 0.038 & 14.23 & 0.031 & 0.45 & 14.51 & -- & NTT	  \\
 82 & 16:40:07.60 & -48:50:57.0 & 0.846 & 104 & 18.73 & 0.191 & 15.81 & 0.049 & 14.24 & 0.031 & 0.24 & 20.57 & Disk & NTT	  \\
 83 & 16:40:07.50 & -48:51:04.0 & 0.563 & 99.8 & 18.59 & 0.179 & 15.68 & 0.046 & 13.88 & 0.026 & -0.15 & 18.65 & Disk & NTT	  \\
 84 & 16:40:07.50 & -48:50:24.0 & 0.186 & 125.1 & 16.84 & 0.079 & 14.57 & 0.027 & 13.17 & 0.018 & -0.12 & 16.04 & M star & NTT	  \\
 85 & 16:40:07.20 & -48:50:55.0 & 0.579 & 102.3 & 18.60 & 0.179 & 15.46 & 0.041 & 13.11 & 0.018 & -0.86 & 17.32 & Disk & NTT	  \\
 86 & 16:40:07.10 & -48:50:38.0 & 0.306 & 112.6 & 17.24 & 0.097 & 14.89 & 0.032 & 13.72 & 0.024 & 0.36 & 15.9 & Disk & NTT	  \\
 89 & 16:40:06.44 & -48:50:43.5 & 0.986 & 104.1 & 15.24 & -- & 14.37 & -- & 14.23 & 0.086 & 0.62 & -- & -- & UUA	  \\
 90 & 16:40:06.40 & -48:54:31.0 & 0.879 & 174.5 & 14.07 & 0.022 & 13.47 & 0.016 & 13.20 & 0.019 & 0.14 & 0.26 & -- & NTT	  \\
 91 & 16:40:06.40 & -48:51:40.0 & 0.735 & 77 & 18.42 & 0.166 & 15.72 & 0.048 & 14.42 & 0.035 & 0.50 & 19.75 & Disk & NTT	  \\
 92 & 16:40:06.30 & -48:51:12.0 & 0.199 & 86 & 12.87 & 0.012 & 11.21 & 0.005 & 10.27 & 0.004 & 0.07 & 10.07 & M star & NTT	  \\
 93 & 16:40:06.10 & -48:51:44.0 & 0.692 & 73.1 & 16.40 & 0.064 & 14.20 & 0.023 & 13.10 & 0.018 & 0.34 & 14.5 & Disk & NTT	  \\
 95 & 16:40:06.00 & -48:51:11.0 & 0.823 & 83.2 & 17.18 & 0.093 & 14.86 & 0.031 & 13.66 & 0.024 & 0.28 & 15.27 & -- & NTT	  \\
 96 & 16:40:05.70 & -48:52:13.7 & 0.525 & 71.9 & 17.32 & -- & 14.20 & 0.0456 & 11.50 & 0.026 & -1.45 & -- & -- & UAA	  \\
 98 & 16:40:05.50 & -48:53:50.0 & 0.895 & 133.2 & -- & -- & -- & -- & 16.30 & 0.105 & -- & -- & -- & NTT		  \\
100 & 16:40:04.50 & -48:51:45.0 & 0.418 & 57.8 & 13.65 & 0.018 & 11.95 & 0.008 & 11.13 & 0.007 & 0.31 & 9.81 & Disk & NTT	  \\
101 & 16:40:03.90 & -48:52:54.0 & 0.879 & 79.4 & 15.62 & 0.044 & 14.65 & 0.028 & 14.25 & 0.031 & 0.30 & 3.03 & Disk & NTT	  \\
103 & 16:40:03.50 & -48:51:25.0 & 1.129 & 54.7 & 19.52 & 0.277 & 16.29 & 0.063 & 14.47 & 0.035 & 0.13 & -- & -- & NTT	  \\
105 & 16:40:01.90 & -48:51:53.0 & 0.606 & 32.0  & ---   & --    & 16.86 & 0.021 & 14.86 & 0.013 & --   & -- & - & VLT \\
107 & 16:40:01.80 & -48:51:37.0 & 0.478 & 35.4 & 18.80 & 0.028 & 14.95 & 0.032 & 13.05 & 0.009 &  0.62   & -- & - & VLT \\
%109  16:40:01.7    -48:51:52                     14.909 0.009   13.105 0.027   12.252 0.007  &  0.33   & -- & - & VLT \\
109 & 16:40:01.70 & -48:51:53.0 & 0.516 & 29.4 & 15.02 & 0.035 & 13.24 & 0.018 & 12.45 & 0.023 & 0.42 & 10.96 & Disk & NTT	  \\
111 & 16:40:01.30 & -48:51:45.0 & 0.526 & 26.9 & 15.47 & 0.048 & 12.86 & 0.013 & 11.53 & 0.011 & 0.36 & 18.34 & Disk & NTT	  \\
112 & 16:40:01.20 & -48:51:52.0 & 0.385 & 24.5 & 11.58 & 0.007 & 10.26 & 0.003 & 9.07 & 0.002 & -0.69 & 1.59 & Disk & NTT	  \\
113 & 16:40:01.10 & -48:50:51.0 & 0.879 & 66.7 & 14.08 & 0.022 & 13.00 & 0.013 & 12.56 & 0.014 & 0.34 & 4.27 & M star & NTT	  \\
%114& 16:40:00.82 & -48:51:38.5 & 0.935 & 26.2 & 12.41 & -- & 11.95 & 0.169 & 10.23 & 0.104 & -2.47 & -- & -- & NTT	  \\
114 & 16:40:00.82 & -48:51:38.5 & 0.935 & 26.2 & 12.41 & -- & 11.95 & 0.169 & 10.23 & 0.104 & -2.47 & -- & -- & NTT	  \\
116 & 16:40:00.40 & -48:51:43.0 & 0.601 & 19.7 & 13.07 & 0.018 & 11.15 & 0.01 & 10.28 & 0.012 & 0.44 & 12.39 & Disk & NTT	  \\
117 & 16:40:00.40 & -48:51:07.0 & 0.991 & 49.2 & -- & -- & -- & -- & 15.89 & 0.071 & -- & -- & -- & NTT		  \\
118$^a$ & 16:40:00.20 & -48:51:40.0 & 0.511 & 20.3 & 10.87 & 0.005 & 9.20 & 0.002 & 8.36 & 0.002 & 0.24 & 11.46 & HMS & NTT	  \\
120 & 16:40:00.00 & -48:51:42.0 & 0.611 & 17.4  & 14.48 & 0.018 & 12.23 & 0.010 & 10.662& 0.006 & -0.42 & -- & -- & VLT	  \\
121$^a$ & 16:40:00.00 & -48:51:53.0 & 0.797 & 12.2 & 13.04 & 0.016 & 11.90 & 0.01 & 11.23 & 0.010 & -0.01 & 5.52 & M star & NTT	  \\
122 & 16:40:00.00 & -48:51:07.0 & 0.713 & 48.5 & -- & -- & -- & -- & 16.02 & 0.078 & -- & -- & -- & NTT		  \\
123 & 16:39:59.80 & -48:54:41.0 & 0.973 & 167.9 & 14.18 & 0.023 & 13.70 & 0.018 & 13.47 & 0.022 & 0.08 & -- & -- & NTT	  \\
124 & 16:39:59.80 & -48:52:00.0 & 0.475 & 11.9 & 15.79 & 0.06 & 13.42 & 0.02 & 12.24 & 0.021 & 0.37 & 16.15 & Disk & NTT	  \\
125$^a$ & 16:39:59.50 & -48:51:37.3 & 0.245 & 18.7 & 12.39 & -- & 12.13 & 0.237 & 10.16 & 0.113 & -3.07 & -- & -- & UEE	  \\
126 & 16:39:59.50 & -48:51:00.0 & 0.594 & 54.8 & 15.21 & 0.037 & 13.35 & 0.015 & 12.47 & 0.013 & 0.37 & 11.49 & Disk & NTT	  \\
127 & 16:39:59.30 & -48:51:28.0 & 0.421 & 27.1 & --    & --    & --    &       & 18.97 & 0.093 & --   & -- & - & VLT \\
128 & 16:39:59.00 & -48:50:50.0 & 0.668 & 64.9 & -- & --       & 22.09 & 4.024 & 16.53 & 0.099 & -- & -- & -- & NTT	  \\
130 & 16:39:58.50 & -48:52:37.0 & 0.055 & 42.8 & 15.04 & 0.034 & 13.91 & 0.02 & 13.20 & 0.019 & -0.08 & 5.63 & M star & NTT	  \\
131 & 16:39:58.60 & -48:52:05.0 & 0.693 & 10.9 & 13.95 & 0.02 & 11.79 & 0.007 & 10.57 & 0.005 & 0.09 & 12.96 & Disk & NTT	  \\
132 & 16:39:58.50 & -48:51:54.0 & 0.287 &  1.7  & --    & --    & 20.88 & 0.289 & 16.98 & 0.037 & --   & -- & - & VLT \\
135 & 16:39:57.30 & -48:52:14.0 & 0.508 & 24.4 & 16.92 & 0.082 & 14.27 & 0.023 & 12.99 & 0.017 & 0.47 & 19.14 & Disk & NTT	  \\
136 & 16:39:56.00 & -48:51:48.0 & 0.405 & 27.1 & 11.67 & 0.007 & 10.54 & 0.004 & 9.79 & 0.003 & -0.15 & 2.42 & Disk & NTT	  \\
137 & 16:39:54.60 & -48:53:21.0 & 0.199 & 95.9 & 16.12 & 0.056 & 15.41 & 0.04 & 15.09 & 0.047 & 0.15 & 1.15 & -- & NTT	  \\
138 & 16:39:54.50 & -48:52:02.0 & 0.116 & 42.2 & 14.14 & 0.022 & 12.92 & 0.012 & 12.31 & 0.012 & 0.17 & 4.75 & Disk & NTT	  \\
140 & 16:39:53.80 & -48:51:46.0 & 0.861 & 49.7 & 12.83 & 0.012 & 11.39 & 0.006 & 10.40 & 0.005 & -0.25 & 4.7 & Disk & NTT	  \\
141 & 16:39:53.74 & -48:51:36.9 & 0.482 & 51.8 & 17.09 & -- & 15.31 & -- & 13.96 & 0.104 & -0.53 & -- & -- & UUA	  \\
142 & 16:39:53.40 & -48:51:48.0 & 0.922 & 53.3 & 15.03 & 0.034 & 13.20 & 0.014 & 12.20 & 0.011 & 0.14 & 10.17 & Disk & NTT	  \\
143 & 16:39:53.30 & -48:52:40.0 & 0.783 & 70.7 & 12.99 & 0.013 & 11.95 & 0.008 & 11.38 & 0.008 & 0.05 & 4.43 & M star & NTT	  \\
144 & 16:39:53.00 & -48:51:30.0 & 0.193 & 60.9 & 17.88 & 0.128 & 14.62 & 0.028 & 12.79 & 0.015 & 0.15 & 27.35 & HMS & NTT	  \\
145 & 16:39:51.90 & -48:51:42.0 & 0.768 & 68.9 & 13.80 & 0.019 & 12.42 & 0.01 & 11.34 & 0.008 & -0.44 & 3.32 & -- & NTT	  \\
147 & 16:39:49.70 & -48:50:23.0 & 0.870 & 126.7 & -- & -- & 16.70 & 0.077 & 15.55 & 0.060 & -- & -- & -- & NTT	  \\
148 & 16:39:49.50 & -48:52:25.0 & 0.846 & 96.6 & 17.68 & 0.118 & 15.28 & 0.04 & 14.14 & 0.031 & 0.47 & 16.97 & -- & NTT	  \\
149 & 16:39:48.50 & -48:49:00.0 & 0.624 & 200.9 & 14.96 & 0.033 & 13.83 & 0.02 & 13.38 & 0.021 & 0.37 & 4.83 & Disk & NTT	  \\
150 & 16:39:46.90 & -48:51:46.0 & 1.033 & 117.3 & 16.47 & 0.066 & 14.21 & 0.023 & 13.20 & 0.019 & 0.55 & 15.99 & -- & NTT	  \\
152 & 16:39:45.50 & -48:51:35.0 & 0.737 & 132 & 16.59 & 0.071 & 14.95 & 0.034 & 14.29 & 0.033 & 0.52 & 10.24 & Disk & NTT	  \\
153 & 16:39:45.50 & -48:51:01.0 & 1.106 & 141.1 & 15.13 & 0.036 & 13.74 & 0.018 & 13.18 & 0.019 & 0.43 & 7.44 & Disk & NTT	  \\
155 & 16:39:41.10 & -48:50:04.9 & 1.259 & 205.1 & 14.32 & -- & 15.02 & 0.0666 & 14.27 & 0.080 & -1.97 & -- & -- & UAA	  \\
210 & 16:39:51.10 & -48:51:53.0 & 0.333 & 74.6 & 14.74 & 0.029 & 13.60 & 0.017 & 12.93 & 0.016 & -0.01 & 3.08 & -- & NTT	  \\
412 & 16:40:18.9 &  -48:53:17.5 & 0.382 & 215.5 & 15.38 & 0.06 & 14.50 & 0.07 & 14.14 & 0.0718 & 0.27 &2.10 & -- & AAA\\
413 & 16:40:15.2 &  -48:51:41.6 & 0.219 & 163.3 & 17.42 & --      & 14.95 & --      & 13.69 & 0.0566 & -- & -- &-- & UUA\\
414 & 16:40:13.4 &  -48:48:53.0 & 0.839 & 231.6 & --  & --  & -- & -- & 20.10 & 2.332          & -- & -- &--&    NTT\\
421 & 16:40:05.1 &  -48:51:53.5 & 0.458 &  62.9 & 15.64 & --      & 13.73 & --      & 12.69 & 0.0696 & -- & -- &--& UUA\\
423 & 16:40:04.7 &  -48:53:38.0 & 0.899 & 119.4 & 15.99 & 0.05 & 14.38 & 0.03 & 13.57 & 0.028        &0.23 &8.58 & --& NTT\\
425 & 16:40:02.7 &  -48:50:03.5 & 0.521 & 174.8 & 17.56 & --      &15.35 &  --     & 14.39 & 0.0718  & -- & -- &--& UUA\\
426 & 16:40:02.2 &  -48:52:02.0 &       &  35.4 & --    & -- &   --      &  --   &   18.60 & 0.114   &  -- & -- &--& VLT\\
430 & 16:39:56.6 &  -48:50:05.0 & 0.822 & 111.6 & 18.50 & 0.17 & 16.30 & 0.07 & 15.28 & 0.065        &0.47 &15.06 & --& NTT\\
433 & 16:39:53.2 &  -48:55:57.4 & 1.586 & 249.0 & 14.32 & 0.02 & 11.42 & 0.02 & 9.99 & 0.0212        & -- & -- &--& AAA\\
434 & 16:39:50.8 &  -48:50:00.0 & 0.756 & 138.6 & 18.91 & 0.23 & 16.88 & 0.09 & 15.86 & 0.081        & -- & -- &--& NTT\\
435 & 16:39:50.1 &  -48:50:22.3 & 0.704 & 124.3 & 16.02 & 0.05 & 15.06 & 0.03 & 14.56 & 0.036        &0.11 &2.08 & --& NTT\\
449 & 16:40:24.6 &  -48:52:57.9 & 1.251 & 263.2 & 15.76 & 0.05 & 14.91 & 0.03 & 14.58 & 0.036        & -- & -- &--& NTT\\
450 & 16:40:18.8 &  -48:52:06.0 & 1.234 & 199.8 & 17.08 & 0.10 & 15.70 & 0.06 & 15.09 & 0.056        &0.34 &7.01 & --& NTT\\
451 & 16:40:18.3 &  -48:53:50.0 & 1.523 & 225.6 & 17.17 & 0.10 & 16.08 & 0.06 & 15.72 & 0.076        &0.48 &5.00 & --& NTT\\
454 & 16:40:09.7 &  -48:52:41.6 & 0.117 & 118.7 & 15.31 & 0.04 & 14.52 & 0.03 & 14.25 & 0.031        &0.33 &1.57 & --& NTT\\
457 & 16:40:01.4 &  -48:51:11.0 & 0.693 & 49.8 & 16.95 & 0.08 & 16.42 & 0.07 & 16.14 & 0.078         &0.05 &0.00 & --& NTT\\
458 & 16:39:59.8 &  -48:53:30.0 & 0.493 & 97.2 & -- & -- & -- & -- & 17.97 & 0.243       & -- & -- &--& NTT\\
460 & 16:39:55.8 &  -48:52:37.3 & 0.497 & 51.6 & 14.77 & 0.03 & 13.82 & 0.02 & 13.19 & 0.018         &-0.12&0.90& --& NTT\\
463 & 16:39:45.0 &  -48:55:11.0 & 1.209 & 237.6 & -- & -- & 17.78 & 0.17 & -- & --          & -- & -- &--& NTT\\
465 & 16:39:29.0 &  -48:52:12.0 & 0.607 & 303.3 & 10.13 & 0.00 & 9.44 & 0.00 & 8.93 & 0.002          & -- & -- &--& NTT\\
466 & 16:40:34.2 &  -48:51:53.2 & 0.747 & 350.8 & 15.13 & 0.04 & 14.39 & 0.03 & 14.13 & 0.033        & -- & -- &--& NTT\\
\tableline	      
South &  &  &  &  &  &  &  &  &  &  &  &  &  &                                                                            \\
 43 & 16:40:18.30 & -48:56:38.0 & 0.692 & 343 & 13.49 & 0.016 & 12.60 & 0.011 & 12.04 & 0.011 & -0.05 & 3.39 & M star & NTT	  \\
 45 & 16:40:16.60 & -48:55:28.0 & 1.111 & 276.8 & 14.02 & 0.021 & 13.16 & 0.014 & 12.88 & 0.016 & 0.38 & 2.46 & Disk & NTT	  \\
 49 & 16:40:15.50 & -48:55:04.0 & 0.616 & 251.6 & 13.21 & 0.014 & 12.57 & 0.01 & 12.34 & 0.012 & 0.26 & 1.8 & HMS & NTT	  \\
 53 & 16:40:14.40 & -48:55:42.0 & 2.037 & 273.6 & 16.97 & 0.088 & 15.81 & 0.053 & 15.23 & 0.053 & 0.18 & 7.9 & HMS & NTT	  \\
 54 & 16:40:14.10 & -48:57:06.0 & 1.320 & 346.7 & 11.71 & 0.007 & 10.94 & 0.005 & 10.65 & 0.005 & 0.29 & 1.46 & M star & NTT	  \\
 55 & 16:40:13.50 & -48:56:14.0 & 0.468 & 298.1 & 14.93 & 0.033 & 14.16 & 0.023 & 13.80 & 0.025 & 0.16 & 1.74 & M star & NTT	  \\
 64 & 16:40:11.20 & -48:54:51.0 & 1.588 & 215.7 & 11.86 & 0.007 & 10.89 & 0.005 & 10.52 & 0.005 & 0.34 & 3.3 & Disk & NTT	  \\
 75 & 16:40:09.40 & -48:55:38.0 & 1.112 & 247.6 & 11.83 & 0.007 & 11.43 & 0.006 & 11.24 & 0.007 & 0.08 & -- & -- & NTT		  \\
 79 & 16:40:08.70 & -48:56:30.0 & 0.794 & 292.7 & 14.56 & 0.027 & 13.67 & 0.018 & 13.32 & 0.020 & 0.29 & 2.3 & Disk & NTT	  \\
 88 & 16:40:06.60 & -48:57:03.0 & 0.887 & 318.5 & 15.68 & 0.047 & 14.86 & 0.035 & 14.49 & 0.039 & 0.20 & 2.1 & M star & NTT	  \\
 94 & 16:40:06.20 & -48:56:31.0 & 2.820 & 284.5 & 16.62 & 0.074 & 16.07 & 0.068 & 15.82 & 0.086 & 0.13 & 3.23 & HMS & NTT	  \\
 97 & 16:40:05.40 & -48:55:39.0 & 2.116 & 234.1 & 14.99 & 0.033 & 14.09 & 0.022 & 13.60 & 0.022 & 0.06 & 7.52 & HMS & NTT	  \\
104 & 16:40:02.30 & -48:56:35.0 & 1.495 & 283.1 & 14.75 & 0.03 & 12.41 & 0.01 & 11.17 & 0.007 & 0.24 & 15.32 & Disk & NTT	  \\
139 & 16:39:54.40 & -48:55:13.0 & 1.783 & 204.7 & 14.58 & 0.027 & 13.80 & 0.019 & 13.53 & 0.022 & 0.31 & 1.36 & -- & NTT	  \\
151 & 16:39:46.50 & -48:56:34.0 & 1.496 & 305.8 & 14.08 & 0.022 & 12.94 & 0.012 & 12.39 & 0.013 & 0.21 & 4.19 & Disk & NTT	  \\
200 & 16:40:18.50 & -48:56:16.0 & 0.513 & 326.4 & 15.59 & 0.044 & 14.68 & 0.029 & 14.35 & 0.032 & 0.35 & 2.76 & -- & NTT	  \\
203 & 16:40:16.30 & -48:56:27.0 & 1.038 & 323.2 & 14.42 & 0.026 & 13.63 & 0.019 & 13.29 & 0.021 & 0.21 & 3.93 & HMS & NTT	  \\
205 & 16:40:15.40 & -48:56:11.0 & 1.350 & 305.4 & 15.02 & 0.034 & 14.19 & 0.023 & 13.88 & 0.026 & 0.30 & 1.78 & -- & NTT	  \\
207 & 16:39:59.50 & -48:56:42.0 & 1.029 & 288.8 & 15.85 & 0.05 & 15.02 & 0.036 & 14.79 & 0.045 & 0.43 & 2.38 & -- & NTT	  \\
208 & 16:39:57.60 & -48:56:56.0 & 1.466 & 302.5 & 17.08 & 0.091 & 15.28 & 0.04 & 14.27 & 0.033 & 0.08 & 9.61 & -- & NTT	  \\
212 & 16:39:49.30 & -48:56:55.0 & 1.320 & 315.8 & 15.26 & 0.038 & 14.09 & 0.022 & 13.36 & 0.021 & -0.06 & 3.25 & Disk & NTT	  \\
222 & 16:40:10.60 & -48:57:40.0 & 1.850 & 363.7 & 12.91 & 0.012 & 11.86 & 0.007 & 11.40 & 0.008 & 0.28 & 5.16 & HMS & NTT	  \\
223 & 16:39:52.90 & -48:57:57.0 & 1.729 & 366.1 & 17.70 & 0.132 & 17.25 & 0.158 & 17.36 & 0.317 & 0.64 & -- & -- & NTT	  \\
259 & 16:40:16.07 & -48:58:16.3 & 0.740 & 418.8 & 8.88 & 0.0227 & 8.39 & 0.0343 & 8.17 & 0.018 & 0.13 & 2.74 & HMS & AAA	  \\
260 & 16:40:13.50 & -49:00:01.0 & 1.405 & 508.3 & 14.49 & 0.0375 & 13.65 & 0.0443 & 13.37 & 0.030 & 0.36 & 2.18 & Disk & AAA	  \\
263 & 16:40:09.32 & -48:58:54.6 & 0.606 & 433.3 & 12.72 & 0.0272 & 11.67 & 0.0262 & 10.94 & 0.025 & -0.20 & 5.22 & M star & AAA  \\
264 & 16:40:07.98 & -48:59:06.2 & 1.845 & 441.6 & 13.61 & 0.06 & 12.77 & 0.078 & 12.31 & 0.050 & 0.08 & 0.87 & -- & EEE	  \\
265 & 16:40:07.74 & -48:58:52.7 & 0.282 & 428 & 13.97 & 0.0479 & 12.85 & 0.0458 & 12.12 & 0.030 & -0.12 & 2.43 & -- & AAA	  \\
267 & 16:40:05.90 & -48:59:08.6 & 0.281 & 440.2 & 9.01 & 0.0255 & 8.48 & 0.0417 & 8.32 & 0.023 & 0.26 & -- & Disk & AAA	  \\
269 & 16:40:03.95 & -49:00:24.3 & 0.880 & 512.8 & 11.29 & 0.0239 & 10.22 & 0.0262 & 9.84 & 0.025 & 0.43 & 4.59 & Disk & AAA	  \\
272 & 16:39:50.66 & -48:59:03.9 & 1.216 & 437 & 13.98 & 0.0597 & 13.23 & 0.0678 & 12.87 & 0.050 & 0.13 & 0.20 & -- & EEA	  \\
274 & 16:39:49.17 & -49:00:59.1 & 0.370 & 552.9 & 14.56 & 0.0334 & 13.52 & 0.0214 & 13.09 & 0.034 & 0.30 & 3.68 & Disk & AAA	  \\
275 & 16:39:48.95 & -48:58:25.4 & 0.827 & 402.8 & 14.70 & 0.0776 & 13.82 & 0.0955 & 13.52 & 0.070 & 0.36 & 2.49 & -- & AAA  \\
309 & 16:40:18.67 & -48:58:57.7 & 0.903 & 467.1 & 13.99 & 0.0362 & 13.49 & 0.0415 & 13.23 & 0.035 & 0.04 & -- & -- & AAA	  \\
310 & 16:40:10.78 & -49:00:51.3 & 3.424 & 550.2 & 15.39 & -- & 14.64 & -- & 14.59 & 0.088 & 0.66 & -- & -- & UUA	  \\
311 & 16:40:07.40 & -48:58:29.4 & 0.472 & 404.5 & 13.80 & -- & 13.93 & 0.0899 & 13.54 & 0.069 & -0.79 & -- & -- & UAA	  \\
314 & 16:39:59.69 & -49:00:23.8 & 0.539 & 509.8 & 15.00 & 0.071 & 14.19 & 0.0591 & 13.99 & 0.068 & 0.45 & 2.27 & -- & AAA	  \\
315 & 16:39:58.56 & -49:01:12.4 & 1.144 & 558.3 & 14.73 & 0.0304 & 13.77 & 0.0214 & 13.50 & 0.030 & 0.49 & 3.86 & -- & AAA	  \\
318 & 16:39:53.46 & -48:59:40.1 & 2.317 & 468.8 & 12.63 & 0.0362 & 11.67 & 0.0384 & 11.23 & 0.030 & 0.22 & 5.42 & HMS & AAA	  \\
338 & 16:39:57.90 & -49:02:17.7 & 4.237 & 623.6 & 13.90 & 0.0609 & 13.18 & 0.0853 & 12.92 & 0.033 & 0.28 & 0.67 & -- & AAA	  \\
417 & 16:40:06.80&  -48:55:24.9 & 0.499 & 225.9 & 15.54 & 0.04 & 13.78 & 0.02 & 12.91 & 0.0328 & 0.28 & 10.18& -- & NTT\\
431 & 16:39:54.20&  -48:57:16.0 & 1.571 & 324.6 & 9.34 & 0.00 & -- & -- & 8.52 & 0.002 & -- & -- &--& NTT\\
438 & 16:39:41.90&  -48:56:57.0 & 0.92  &345.0  & 16.84 & 0.08 & 15.24 & 0.04 & 14.36 & 0.034 &        0.10 & 7.88 & -- &NTT\\
448 & 16:40:27.50&  -48:55:22.2 & 0.784 & 352.8 & 15.27 & 0.04 & 13.43 & 0.02 & 12.04 & 0.011 & -- & -- &--& NTT\\
455 & 16:40:09.10&  -48:55:54.1 & 0.703 & 260.8 & 15.07 & 0.07 & 14.32 & 0.08 & 14.13 & 0.0793  & 0.43 & 1.66 & -- & AAA\\
461 & 16:39:50.90&  -48:57:23.0 & 0.996 & 338.4 & 16.93 & 0.09 & 15.99 & 0.07 & 15.73 & 0.094      & 0.50 & 3.73 & -- & NTT\\
467 & 16:40:30.40&  -48:54:58.3 & 2.435 & 365.4 & 14.32 & 0.02 & 13.27 & 0.02 & 12.95 & 0.017 & -- & -- &--& NTT\\
468 & 16:40:16.20&  -48:57:06.7 & 0.819 & 358.0 & 14.66 & 0.03 & 13.70 & 0.02 & 13.17 & 0.019   &0.06 & 1.84 & --  & NTT\\
469 & 16:40:15.80&  -48:55:56.0 & 0.902 & 294 & 20.07 & 0.74 & 18.76 & 0.30 & -- & -- & -- & -- &--& NTT\\
470 & 16:40:03.70&  -48:57:15.0 & 1.119 & 325.2 & 17.46 & 0.12 & 16.46 & 0.10 & 16.64 & 0.194 & -- & -- &--& NTT\\
472 & 16:39:57.70&  -48:57:29.0 & 0.77  & 334.2 & 15.65 & 0.05 & 14.94 & 0.03 & 14.53 & 0.038     &0.01 & 0.00 & -- & NTT\\

\tableline	      										  
West &  &  &  &  &  &  &  &  &  &  &  &  &  &     										  \\
156 & 16:39:39.70 & -48:54:55.0 & 1.566 & 261.9 & 14.82 & 0.031 & 13.88 & 0.02 & 13.46 & 0.022 & 0.23 & 2.47 & -- & NTT	  \\
157 & 16:39:39.60 & -48:53:48.0 & 0.742 & 220.4 & 16.57 & 0.07 & 15.31 & 0.039 & 14.67 & 0.038 & 0.19 & 5.26 & Disk & NTT	  \\
158 & 16:39:39.60 & -48:47:30.0 & 0.992 & 323.9 & 13.00 & 0.013 & 12.50 & 0.01 & 12.44 & 0.013 & 0.39 & -- & Disk & NTT		  \\
159 & 16:39:39.40 & -48:53:56.0 & 1.093 & 227 & 14.62 & 0.028 & 13.71 & 0.018 & 13.39 & 0.021 & 0.36 & 2.74 & -- & NTT	  \\
160 & 16:39:39.30 & -48:53:19.0 & 1.524 & 210.7 & 15.54 & 0.043 & 14.21 & 0.023 & 13.64 & 0.023 & 0.36 & 6.65 & Disk & NTT	  \\
161 & 16:39:39.20 & -48:52:25.0 & 1.226 & 195.7 & 15.54 & 0.043 & 14.86 & 0.031 & 14.68 & 0.039 & 0.37 & 0.73 & Disk & NTT	  \\
162 & 16:39:39.10 & -48:46:19.0 & 1.861 & 387.4 & 9.77 & 0.003 & 8.85 & 0.001 & 8.39 & 0.002 & 0.14 & 6.42 & HMS & NTT	  \\
163 & 16:39:38.80 & -48:53:48.0 & 0.526 & 227.3 & 16.74 & 0.076 & 15.95 & 0.057 & 15.78 & 0.079 & 0.49 & 2.32 & -- & NTT	  \\
164 & 16:39:38.70 & -48:54:54.0 & 0.759 & 267.5 & 13.44 & 0.016 & 12.71 & 0.011 & 12.44 & 0.013 & 0.27 & 2.46 & HMS & NTT	  \\
165 & 16:39:38.20 & -48:56:55.0 & 1.227 & 363.3 & 13.15 & 0.014 & 12.31 & 0.009 & 11.95 & 0.010 & 0.24 & 1.68 & -- & NTT	  \\
166 & 16:39:38.20 & -48:46:57.0 & 1.039 & 358.6 & 14.73 & 0.029 & 13.17 & 0.014 & 11.97 & 0.010 & -0.49 & 4.73 & Disk & NTT	  \\
167 & 16:39:37.20 & -48:56:43.0 & 1.025 & 359.2 & 14.49 & 0.026 & 12.91 & 0.012 & 12.15 & 0.011 & 0.27 & 8.44 & Disk & NTT	  \\
168 & 16:39:37.30 & -48:46:51.0 & 0.988 & 369.4 & 13.15 & 0.014 & 12.11 & 0.008 & 11.75 & 0.009 & 0.44 & 4.38 & Disk & NTT	  \\
169 & 16:39:37.00 & -48:51:59.0 & 1.258 & 214.6 & -- & -- & -- & -- & 16.46 & 0.091 & -- & -- & -- & NTT		  \\
170 & 16:39:35.20 & -48:54:04.0 & 0.682 & 266.1 & 14.81 & 0.031 & 13.70 & 0.018 & 13.27 & 0.019 & 0.40 & 4.89 & Disk & NTT	  \\
171 & 16:39:34.70 & -48:53:31.0 & 2.353 & 258 & 9.63 & 0.002 & 9.11 & 0.002 & 8.81 & 0.002 & 0.02 & -- & Disk & NTT		  \\
172 & 16:39:34.40 & -48:55:06.0 & 1.126 & 308 & 12.77 & 0.012 & 11.30 & 0.006 & 10.33 & 0.005 & -0.19 & 5.21 & Disk & NTT	  \\
173 & 16:39:33.60 & -48:54:58.0 & 1.181 & 309.4 & 14.36 & 0.025 & 13.11 & 0.013 & 12.56 & 0.014 & 0.31 & 5.69 & Disk & NTT	  \\
174 & 16:39:30.69 & -48:51:02.8 & 0.235 & 281.1 & 8.59 & 0.0286 & 8.56 & 0.0493 & 8.52 & 0.021 & -0.04 & -- & -- & AAA	  \\
175 & 16:39:30.80 & -48:50:31.0 & 1.161 & 288.7 & 14.21 & 0.023 & 12.88 & 0.012 & 12.24 & 0.012 & 0.25 & 6.61 & M star & NTT	  \\
176 & 16:39:28.80 & -48:50:19.0 & 0.797 & 309.8 & 15.59 & 0.045 & 15.00 & 0.036 & 14.64 & 0.045 & -0.02 & -- & -- & NTT	  \\
215 & 16:39:36.50 & -48:47:55.0 & 1.143 & 324.8 & 11.23 & 0.005 & 10.89 & 0.005 & 10.80 & 0.006 & 0.18 & -- & Disk & NTT	  \\
216 & 16:39:35.00 & -48:55:30.0 & 1.579 & 319.6 & 19.13 & 0.269 & 17.75 & 0.148 & 17.34 & 0.169 & 0.68 & -- & -- & NTT	  \\
217 & 16:39:26.20 & -48:51:47.0 & 0.891 & 321.5 & 10.41 & 0.004 & 10.17 & 0.003 & 10.04 & 0.004 & 0.03 & -- & Disk & NTT	  \\
218 & 16:39:25.50 & -48:50:06.0 & 1.149 & 344.9 & 15.51 & 0.047 & 14.48 & 0.031 & 13.96 & 0.032 & 0.14 & 4.16 & M star & NTT	  \\
219 & 16:39:23.40 & -48:49:58.0 & 1.515 & 368.1 & 14.23 & 0.023 & 13.22 & 0.014 & 12.73 & 0.015 & 0.15 & 2.67 & -- & NTT	  \\
224 & 16:39:30.90 & -48:47:23.0 & 1.709 & 385.8 & 15.14 & 0.036 & 14.52 & 0.027 & 14.25 & 0.031 & 0.18 & 3.08 & HMS & NTT	  \\
225 & 16:39:20.51 & -48:51:42.1 & 1.528 & 376.9 & 14.61 & 0.0396 & 13.75 & 0.0654 & 13.38 & 0.055 & 0.23 & 1.75 & -- & AAA	  \\
282 & 16:39:37.67 & -48:44:46.6 & 0.129 & 475.3 & 14.37 & 0.0409 & 13.49 & 0.054 & 13.10 & 0.045 & 0.23 & 4.49 & HMS & AAA	  \\
283 & 16:39:30.95 & -48:46:42.6 & 0.431 & 414.9 & 14.08 & 0.0317 & 13.09 & 0.0335 & 12.78 & 0.039 & 0.47 & 4.02 & Disk & AAA  \\
284 & 16:39:29.40 & -48:46:20.0 & 2.043 & 442.6 & -- & -- & 18.24 & 0.511 & 18.72 & 1.573 & -- & -- & -- & NTT	  \\
285 & 16:39:26.80 & -48:46:11.0 & 1.117 & 465.3 & 14.39 & 0.025 & 13.56 & 0.017 & 13.31 & 0.021 & 0.41 & 2.33 & -- & NTT	  \\
286 & 16:39:26.00 & -48:45:31.0 & 1.831 & 501.9 & 8.91 & 0.002 & 8.69 & 0.001 & 8.25 & 0.001 & -0.53 & -- & -- & NTT		  \\
287 & 16:39:24.00 & -48:46:39.0 & 1.363 & 466.2 & 14.62 & 0.028 & 13.68 & 0.019 & 13.30 & 0.022 & 0.28 & 2.95 & M star & NTT	  \\
288 & 16:39:22.70 & -48:57:30.0 & 0.873 & 488 & 16.73 & 0.079 & 15.84 & 0.064 & 15.39 & 0.078 & 0.12 & 1.48 & Disk & NTT	  \\
289 & 16:39:18.10 & -48:50:46.8 & 2.585 & 406.2 & 13.01 & 0.042 & 11.87 & 0.063 & 11.22 & 0.039 & 0.05 & 3.46 & -- & EEE	  \\
290 & 16:39:17.70 & -48:55:00.3 & 1.625 & 445.1 & 13.29 & 0.0227 & 12.81 & 0.0214 & 12.61 & 0.021 & 0.14 & -- & -- & AAA	  \\
292 & 16:39:16.32 & -48:54:54.0 & 1.654 & 454.9 & 14.86 & -- & 14.62 & 0.075 & 13.48 & -- & -1.71 & -- & -- & UAU	  \\
293 & 16:39:16.32 & -48:52:30.6 & 0.845 & 419.7 & 14.14 & 0.0516 & 12.79 & -- & 12.40 & -- & 0.68 & -- & -- & AUU  \\
294 & 16:39:12.40 & -48:49:45.9 & 0.931 & 474.6 & 13.13 & 0.0505 & 12.45 & 0.0604 & 12.20 & 0.050 & 0.26 & 2.2 & HMS & AAA	  \\
295 & 16:39:11.58 & -48:51:03.4 & 0.459 & 467.7 & 14.80 & 0.0663 & 13.90 & 0.0761 & 13.66 & 0.069 & 0.50 & 3.4 & Disk & AAA	  \\
296 & 16:39:08.79 & -48:52:30.3 & 3.276 & 493.7 & 13.67 & 0.0274 & 11.96 & 0.0214 & 11.23 & 0.023 & 0.47 & 10.55 & Disk & AAA	  \\
297 & 16:39:03.13 & -48:49:39.6 & 0.896 & 564.7 & 12.42 & 0.0348 & 11.77 & 0.0399 & 11.52 & 0.035 & 0.21 & -- & -- & AEA	  \\
320 & 16:39:37.05 & -48:43:47.5 & 1.410 & 531.6 & 14.89 & 0.0586 & 13.90 & 0.0629 & 13.74 & 0.083 & 0.71 & 5.16 & Disk & AEA	  \\
322 & 16:39:25.50 & -48:57:11.0 & 2.508 & 457.6 & 15.53 & 0.043 & 14.35 & 0.026 & 13.81 & 0.028 & 0.25 & 4.7 & -- & NTT	  \\
323 & 16:39:24.60 & -48:47:27.0 & 1.927 & 430.7 & 14.49 & 0.027 & 13.58 & 0.018 & 13.20 & 0.021 & 0.27 & 2.41 & -- & NTT	  \\
324 & 16:39:24.00 & -48:47:41.0 & 1.420 & 426.5 & 14.30 & 0.024 & 13.38 & 0.015 & 12.99 & 0.017 & 0.26 & 2.88 & M star & NTT	  \\
325 & 16:39:21.80 & -48:57:52.0 & 1.694 & 511.7 & 16.20 & 0.061 & 15.20 & 0.042 & 14.64 & 0.049 & 0.06 & 8.48 & HMS & NTT	  \\
326 & 16:39:21.00 & -48:57:32.0 & 2.999 & 498.9 & 15.24 & 0.04 & 13.77 & 0.023 & 13.03 & 0.021 & 0.20 & 7.15 & Disk & NTT	  \\
327 & 16:39:11.24 & -48:55:24.2 & 1.157 & 512.9 & 13.98 & -- & 13.76 & 0.069 & 13.28 & 0.053 & -0.60 & -- & -- & UAA	  \\
329 & 16:39:09.35 & -48:48:31.7 & 1.285 & 527.6 & 14.48 & 0.0481 & 13.65 & 0.0499 & 13.37 & 0.048 & 0.35 & 2.02 & Disk & AAA	  \\
330 & 16:39:08.10 & -48:50:24.0 & 1.696 & 507.4 & 14.86 & 0.0707 & 13.98 & 0.0726 & 13.68 & 0.063 & 0.37 & 2.55 & Disk & AAA	  \\
331 & 16:39:06.60 & -48:56:36.9 & 0.854 & 586.3 & 13.16 & 0.0303 & 12.18 & 0.0309 & 11.90 & 0.032 & 0.50 & 4.11 & -- & AAA	  \\
332 & 16:39:05.69 & -48:51:36.3 & 0.475 & 523.3 & 15.13 & 0.0685 & 14.29 & 0.0702 & 14.07 & 0.092 & 0.46 & 2.64 & -- & AAA	  \\
333 & 16:39:05.43 & -48:55:57.7 & 1.782 & 578.8 & 12.58 & 0.0289 & 11.85 & 0.0352 & 11.48 & 0.032 & 0.09 & 1.55 & M star & AAA	  \\
334 & 16:39:05.61 & -48:48:52.8 & 0.848 & 554.5 & 13.65 & 0.043 & 12.73 & 0.065 & 12.12 & 0.039 & -0.11 & 0.69 & -- & EEE	  \\
340 & 16:39:07.39 & -48:51:45.1 & 2.278 & 506.3 & 15.23 & 0.063 & 14.35 & 0.0876 & 12.47 & -- & -2.32 & -- & -- & AAU  \\
341 & 16:38:46.62 & -48:53:47.3 & 4.348 & 719.9 & 15.76 & -- & 14.23 & 0.0604 & 13.42 & 0.042 & 0.17 & -- & -- & UAA	  \\
441 & 16:39:38.50 &  -48:51:23.1 & 0.339 & 201.0 & 15.55 & 0.04 & 14.81 & 0.03 & 14.45 & 0.034 &  0.13 & 1.72 & -- &NTT\\
442 & 16:39:35.00 &  -48:49:23.0 & 0.736 & 278.9 & 16.81 &   --    & 15.09 & 0.08 & 15.64 &  --  & -- & -- &--& UAU\\
443 & 16:39:34.80 &  -48:54:51.0 & 1.299 & 295.2 & 21.12 & 0.98 & -- & -- & -- & -- & -- & -- &--&        NTT\\
444 & 16:39:33.40 &  -48:53:43.0 & 1.604 & 273.0 &-- & -- & 19.21 & 0.35 & -- & -- & -- & -- &--& NTT\\
445 & 16:39:30.40 &  -48:48:10.1 & 2.099 & 359.4 & 18.07 & 0.16 & 16.92 & 0.11 & 16.79 & 0.151 & -- & -- &--& NTT\\
446 & 16:39:29.60 &  -48:51:01.0 & 0.551 & 292.2 & -- & -- & 19.40 & 0.94 & 16.28 & 0.115 & -- & -- &--& NTT\\
478 & 16:39:01.70 &  -48:56:37.3 & 0.705 & 462.4 & 15.97 & 0.05 & 14.50 & 0.03 & 13.85 & 0.028 & 0.37 & 0.00 &--& NTT\\
483 & 16:39:08.10 &  -48:49:28.9 & 2.170 & 398.5 & 14.30 & 0.04 & 13.01 & 0.05 & 12.45 & 0.0428 & 0.34 & 6.16 &--&AAA\\
484 & 16:39:13.30 &  -48:53:44.7 & 0.447 & 460.8 & 14.50 & 0.03 & 13.51 & 0.03 & 12.97 & 0.0315 & 0.07 & 2.17 &--&AAA\\
\enddata
\tablenotetext{a}{VLT adaptive optics data indicate this source is a double.}
\tablenotetext{~}{FLAGS:
VLT = data are from the Very Large Telescope, reduction
discussed in Comer{\'o}n \& Schneider (2007).
 NTT = data are from New Technology Telescope, reduction
discussed in Comer{\'o}n \e 2005.
  AAA, UAB, UAU, AAU, etc. = data are taken from 2MASS with these
  listed photometry codes for the JHK channels respectively: 
A-- error $<$10.9\%, B -- error $<$15.6\%, 
E -- This category includes detections where the goodness-of-fit
quality of the profile-fit photometry was very poor,  
U -- upper limit.}
\end{deluxetable}


==> table_11.tex <==
\begin{deluxetable}{lccrrrrrrrrc}
%\tabletypesize{\normal}
\tablecaption{IRAC detections of X-ray sources in the RCW 108 Field \label{XIRAC}}
\tablewidth{0pt}
\tablehead{
\colhead{SRC \#} &\colhead{Offset} &\colhead{Offaxis}  &\colhead{Ch1}   & \colhead{Ch2}   &
\colhead{Ch3} &  \colhead{Ch4} &\colhead{Ch1e}   & \colhead{Ch2e}   &
\colhead{Ch3e} &  \colhead{Ch4e} & \colhead{IR Class}\\
\colhead{} &\colhead{[arcsec.]} &\colhead{[arcsec.]}}
\startdata
%XID & OFFSET & OFAXIS & CH1 & CH2 & Ch3 & Ch4 & Ch1e & CH2e & CH3e & CH4e & Class  
East &  &  &  &  &  &  &  &  &  &  & \\ 
1 & 0.481 & 375.2 & 10.51 & 10.13 & 9.88 & 9.42 & 0.01 & 0.01 & 0.02 & 0.05 &II   \\ 
2 & 0.447 & 369.5 & 11.06 & 10.75 & 10.40 & 9.90 & 0.02 & 0.02 & 0.03 & 0.03 &II  \\
3 & 0.421 & 363.2 & 12.50 & 12.53 & 12.72 & -- & 0.03 & 0.03 & 0.12 & -- & --      \\
4 & 0.373 & 353.6 & 12.14 & 12.10 & -- & -- & 0.04 & 0.05 & -- & -- & --           \\  
6 & 0.441 & 365.2 & 11.46 & 11.05 & 10.60 & 9.79 & 0.01 & 0.01 & 0.03 & 0.03 &II  \\
7 & 0.364 & 336.7 & 12.88 & -- & -- & -- & 0.02 & -- & -- & -- & --                \\
8 & 0.233 & 332.3 & 11.41 & 11.05 & 10.72 & 9.84 & 0.01 & 0.01 & 0.03 & 0.05 &II  \\
10 & 0.063 & 324.2 & 13.20 & 13.18 & 13.61 & -- & 0.04 & 0.04 & 0.27 & -- & --     \\
11 & 0.261 & 346.1 & -- & 12.26 & -- & -- & -- & 0.03 & -- & -- & --               \\
12 & 0.382 & 316.3 & 10.99 & 10.62 & 10.06 & 8.46 & 0.01 & 0.01 & 0.02 & 0.03 &II \\
16 & 0.476 & 307.2 & 11.32 & 11.31 & 11.26 & 11.35 & 0.01 & 0.01 & 0.05 & 0.10 & III \\
17 & 0.322 & 298.2 & 13.30 & 13.17 & -- & -- & 0.04 & 0.06 & -- & -- & --          \\
18 & 0.425 & 313.4 & 12.85 & 12.84 & -- & -- & 0.03 & 0.04 & -- & -- & --	   \\
19 & 0.524 & 298.2 & 12.39 & 12.39 & 12.51 & -- & 0.02 & 0.03 & 0.11 & -- & --	   \\
20 & 0.331 & 281.5 & 12.61 & 12.58 & 12.73 & -- & 0.04 & 0.05 & 0.13 & -- & --	   \\
22 & 0.19 & 276.9 & 12.97 & 12.98 & 12.81 & -- & 0.05 & 0.07 & 0.16 & -- & --	   \\
23 & 0.179 & 279.1 & 13.36 & 13.47 & 13.66 & -- & 0.07 & 0.10 & 0.29 & -- & --	   \\
24 & 0.7 & 256.9 & 12.83 & 12.86 & -- & -- & 0.06 & 0.08 & -- & -- & --		   \\
28 & 0.288 & 245 & 12.57 & 12.53 & 12.40 & -- & 0.03 & 0.03 & 0.12 & -- & --	   \\
29 & 1.81 & 250.2 & 9.23 & 9.41 & 9.17 & 9.16 & 0.00 & 0.01 & 0.01 & 0.01 & III	   \\
30 & 0.326 & 301.4 & 11.52 & 11.44 & 11.46 & 11.52 & 0.01 & 0.02 & 0.06 & 0.10 & III \\
31 & 0.524 & 316.4 & 13.82 & 13.75 & -- & -- & 0.08 & 0.11 & -- & -- & --	   \\
32 & 0.296 & 230.1 & 10.37 & -- & 9.72 & 9.07 & 0.01 & 0.01 & 0.02 & 0.03 &II     \\
33 & 0.485 & 222.3 & 13.20 & 13.09 & -- & -- & 0.09 & 0.11 & -- & -- & --	   \\
36 & 0.081 & 217.1 & 11.85 & 11.47 & 10.95 & 10.02 & 0.02 & 0.02 & 0.05 & 0.06 &II\\
37 & 0.174 & 231.5 & 10.29 & 9.99 & 9.58 & 8.93 & 0.01 & 0.01 & 0.02 & 0.04 & II	   \\
38 & 0.243 & 248.4 & 12.56 & 12.29 & 11.86 & -- & 0.04 & 0.03 & 0.18 & -- & II	   \\
39 & 0.344 & 213 & 11.74 & 11.69 & 11.61 & -- & 0.02 & 0.02 & 0.14 & -- & --	   \\
40 & 0.099 & 226.2 & 8.93 & 8.46 & 7.98 & 7.16 & 0.00 & 0.00 & 0.01 & 0.02 & II	   \\
41 & 0.096 & 206.5 & 13.15 & 13.18 & -- & -- & 0.08 & 0.08 & -- & -- & --	   \\
177 & 0.511 & 388.5 & 13.21 & 12.74 & 12.91 & 11.39 & 0.04 & 0.04 & 0.20 & 0.14 & gal\\
178 & 0.676 & 375.3 & 13.24 & 12.90 & 12.39 & -- & 0.05 & 0.04 & 0.17 & -- & II	   \\
179 & 2.224 & 379.9 & 14.46 & 14.39 & -- & -- & 0.11 & 0.12 & -- & -- & --	   \\
180 & 0.343 & 350 & 13.18 & 12.98 & -- & -- & 0.05 & 0.06 & -- & -- & --            \\
181 & 1.011 & 357.5 & 13.84 & 13.61 & -- & -- & 0.06 & 0.08 & -- & -- & --	    \\
183 & 0.842 & 338.7 & 12.69 & 12.23 & 11.67 & 10.37 & 0.03 & 0.03 & 0.05 & 0.08 &II\\
184 & 1.887 & 355.2 & 13.55 & 13.49 & -- & -- & 0.06 & 0.06 & -- & -- & --	    \\
185 & 0.815 & 302.6 & 11.06 & 11.02 & 11.04 & 11.02 & 0.01 & 0.01 & 0.04 & 0.06 & III \\
187 & 0.383 & 323.6 & 13.58 & 13.44 & -- & 12.60 & 0.06 & 0.06 & -- & 0.15 & --	    \\
188 & 0.546 & 331.6 & 12.36 & 12.44 & 12.40 & 12.43 & 0.02 & 0.03 & 0.11 & 0.20 & --\\
189 & 1.106 & 264.9 & 11.72 & 11.41 & 11.14 & 10.59 & 0.02 & 0.02 & 0.04 & 0.05 &II\\
191 & 0.508 & 303 & 11.22 & 10.63 & 10.15 & 9.25 & 0.01 & 0.01 & 0.02 & 0.02 &II   \\
192 & 0.978 & 374.1 & 13.21 & 12.84 & 12.44 & 11.79 & 0.05 & 0.05 & 0.11 & 0.10 &II\\
194 & 0.752 & 366.2 & 11.57 & 11.06 & 10.68 & 9.83 & 0.01 & 0.01 & 0.03 & 0.03 &II \\
195 & 0.665 & 241.7 & 11.90 & 11.30 & 10.78 & 9.62 & 0.02 & 0.01 & 0.03 & 0.02 &II \\
196 & 0.749 & 385.7 & 12.45 & 12.47 & 12.35 & -- & 0.02 & 0.03 & 0.12 & -- & --	    \\
197 & 1.07 & 259.9 & 13.28 & 13.29 & -- & -- & 0.05 & 0.06 & -- & -- & --	    \\
198 & 0.514 & 321 & 10.84 & 10.65 & 10.25 & 9.25 & 0.01 & 0.01 & 0.03 & 0.02 &II   \\
228 & 1.201 & 550 & 13.48 & 13.11 & -- & -- & 0.05 & 0.05 & -- & -- & II		    \\
229 & 0.927 & 533.1 & 12.18 & 11.87 & 11.48 & 10.67 & 0.02 & 0.03 & 0.05 & 0.03 &II\\
230 & 0.241 & 538.2 & 12.56 & 12.53 & -- & -- & 0.03 & 0.03 & -- & -- & --	    \\
231 & 0.531 & 532.4 & 12.31 & 12.31 & 12.22 & -- & 0.02 & 0.03 & 0.11 & -- & --	    \\
232 & 0.775 & 504.8 & 14.10 & 14.38 & -- & -- & 0.08 & 0.16 & -- & -- & --	    \\
233 & 0.946 & 514.5 & 11.62 & 11.57 & 11.64 & 11.54 & 0.02 & 0.02 & 0.06 & 0.07 & III \\
234 & 0.244 & 541.8 & 11.19 & 10.73 & 10.45 & 9.54 & 0.01 & 0.01 & 0.03 & 0.02 &II \\
235 & 1.091 & 493.5 & 12.69 & 12.64 & -- & -- & 0.03 & 0.03 & -- & -- & --           \\
237 & 1.12 & 463.5 & 13.03 & 13.13 & -- & -- & 0.03 & 0.07 & -- & -- & --	     \\
238 & 0.484 & 458.5 & 13.41 & 13.20 & -- & -- & 0.04 & 0.04 & -- & -- & --	     \\
239 & 0.409 & 452.8 & 12.89 & 12.96 & 13.30 & -- & 0.03 & 0.04 & 0.19 & -- & --	     \\
240 & 0.72 & 453.9 & 12.42 & 12.47 & -- & -- & 0.04 & 0.04 & -- & -- & --	     \\
241 & 0.341 & 521.4 & 11.74 & 11.70 & 11.59 & 11.41 & 0.02 & 0.02 & 0.06 & 0.07 & III  \\
243 & 0.279 & 479.5 & 8.78 & 8.83 & 8.77 & 8.71 & 0.00 & 0.00 & 0.01 & 0.01 & III	     \\
244 & 0.467 & 449.7 & 12.68 & 12.37 & 11.97 & 10.74 & 0.03 & 0.04 & 0.10 & 0.08 &II \\
245 & 0.338 & 419.8 & 9.38 & 9.43 & 9.36 & 9.35 & 0.01 & 0.01 & 0.01 & 0.03 & III	     \\
246 & 0.934 & 440.7 & 10.94 & 11.04 & 10.99 & 10.86 & 0.01 & 0.01 & 0.04 & 0.06 & III  \\
247 & 0.294 & 422.6 & 10.68 & 10.40 & 10.22 & 9.79 & 0.01 & 0.01 & 0.03 & 0.06 &II  \\
248 & 0.43 & 416.9 & 11.33 & 11.27 & 11.31 & 11.14 & 0.01 & 0.02 & 0.07 & 0.10 & III   \\
250 & 0.657 & 426.4 & 13.09 & 12.71 & 12.14 & 11.67 & 0.04 & 0.04 & 0.07 & 0.13 &II \\
251 & 1.285 & 439.4 & 11.13 & 11.03 & -- & -- & 0.01 & 0.01 & -- & -- & --	     \\
252 & 0.583 & 428.9 & 13.22 & 13.24 & 12.47 & -- & 0.04 & 0.06 & 0.12 & -- & --	     \\
253 & 0.316 & 432.7 & 11.31 & 11.04 & 10.75 & 9.73 & 0.01 & 0.01 & 0.03 & 0.02 &II  \\
254 & 0.378 & 439.6 & 12.05 & 11.96 & 11.82 & 11.29 & 0.02 & 0.03 & 0.07 & 0.06 & III  \\
255 & 0.188 & 419.1 & 11.39 & 11.41 & 11.35 & 11.32 & 0.02 & 0.02 & 0.05 & 0.07 & III  \\
257 & 0.306 & 423.3 & 10.57 & 10.30 & 10.01 & 9.29 & 0.01 & 0.01 & 0.02 & 0.02 &II  \\
299 & 0.583 & 770.6 & 11.50 & 11.41 & 11.46 & -- & 0.02 & 0.02 & 0.10 & -- & --	     \\
300 & 0.585 & 594.5 & 12.24 & 12.18 & 11.74 & -- & 0.02 & 0.02 & 0.10 & -- & --	     \\
302 & 2.11 & 783.4 & 12.35 & 12.34 & -- & 11.35 & 0.03 & 0.04 & -- & 0.34 & --	     \\
305 & 0.921 & 497.7 & 12.37 & 12.08 & 11.94 & 10.92 & 0.03 & 0.03 & 0.09 & 0.07 &II \\
306 & 0.895 & 441.2 & 10.80 & 10.88 & 10.75 & 10.61 & 0.01 & 0.01 & 0.03 & 0.08 & III  \\
308 & 2.435 & 420.7 & 12.48 & 12.45 & -- & -- & 0.06 & 0.05 & -- & -- & --	     \\
337 & 2.368 & 487.6 & 11.97 & 11.61 & 11.22 & 10.70 & 0.02 & 0.02 & 0.04 & 0.04 &II \\
366 & 2.374 & 1113.4 & 12.21 & -- & -- & -- & 0.02 & -- & -- & -- & --		     \\
401 & 1.908 & 313.2 & 13.25 & 13.11 & -- & -- & 0.04 & 0.05 & -- & -- & --	     \\
448 & 0.588 & 352.8 & 10.48 & 9.90 & 9.38 & 8.35 & 0.01 & 0.01 & 0.01 & 0.01 &II    \\
449 & 1.243 & 263.4 & 14.42 & 14.18 & -- & -- & 0.12 & 0.14 & -- & -- & --	     \\
474 & 0.715 & 462.6 & 12.06 & 12.10 & 11.89 & 11.80 & 0.02 & 0.03 & 0.08 & 0.11 & III  \\
\hline
North &  &  &  &  &  &  &  &  &  &  & 						     \\
46 & 0.13 & 333 & 12.77 & 12.73 & -- & -- & 0.09 & 0.08 & -- & -- & --               \\
59 & 1.265 & 344 & -- & 12.85 & -- & -- & -- & 0.11 & -- & -- & --		     \\
60 & 0.355 & 241.6 & 9.04 & 7.82 & 7.02 & 6.21 & 0.00 & 0.00 & 0.01 & 0.01 & I	     \\
61 & 0.224 & 253.6 & 9.29 & 8.68 & 8.03 & 6.79 & 0.00 & 0.00 & 0.02 & 0.04 & II	     \\
133 & 0.663 & 300.8 & 13.11 & 13.18 & -- & -- & 0.13 & 0.25 & -- & -- & --	     \\
134 & 0.061 & 357.5 & -- & 11.78 & 11.67 & -- & -- & 0.03 & 0.15 & -- & --	     \\
146 & 0.104 & 317.1 & 10.82 & 10.81 & 10.86 & 11.02 & 0.01 & 0.01 & 0.04 & 0.14 & III  \\
201 & 0.855 & 348.9 & 11.82 & 11.47 & 11.21 & 10.40 & 0.02 & 0.02 & 0.07 & 0.15 &II \\
202 & 0.427 & 283.2 & 13.07 & 13.09 & -- & -- & 0.07 & 0.07 & -- & -- & --	     \\
211 & 1.167 & 301.8 & 13.05 & 13.04 & -- & -- & 0.04 & 0.07 & -- & -- & --	     \\
258 & 0.539 & 407.1 & 13.66 & 13.67 & -- & -- & 0.09 & 0.11 & -- & -- & --	     \\
262 & 0.653 & 494.4 & 11.02 & 10.98 & 10.81 & 10.26 & 0.01 & 0.01 & 0.04 & 0.10 & III  \\
266 & 1.725 & 446 & 13.58 & 13.37 & -- & -- & 0.07 & 0.06 & -- & -- & --	     \\
268 & 0.635 & 400.8 & -- & 14.04 & -- & -- & -- & 0.13 & -- & -- & --		     \\
271 & 0.355 & 419.1 & 11.64 & 11.65 & 11.57 & 11.10 & 0.02 & 0.02 & 0.09 & 0.26 & -- \\
276 & 0.512 & 442.3 & 11.95 & 11.99 & 12.05 & -- & 0.02 & 0.03 & 0.12 & -- & --	     \\
277 & 1.056 & 465.1 & 10.74 & 10.21 & 9.77 & 9.15 & 0.01 & 0.01 & 0.02 & 0.04 &II   \\
312 & 0.766 & 479.3 & 12.47 & 12.09 & 12.00 & 11.08 & 0.03 & 0.03 & 0.13 & 0.25 &II \\
319 & 1.274 & 480.9 & 11.19 & 10.83 & 10.50 & 9.95 & 0.01 & 0.01 & 0.03 & 0.05 &II  \\
339 & 2.446 & 562.5 & 12.08 & 12.15 & 12.23 & -- & 0.02 & 0.03 & 0.13 & -- & --	     \\
\hline
RCW~108--IR &  &  &  &  &  &  &  &  &  &  & 						     \\
47 & 0.291 & 195.8 & 12.20 & 12.21 & -- & -- & 0.04 & 0.06 & -- & -- & --	     \\
48 & 0.161 & 218.8 & 12.38 & 11.97 & 11.50 & 10.76 & 0.03 & 0.02 & 0.10 & 0.14 &II  \\
50 & 0.178 & 165.2 & 12.15 & 11.73 & 11.59 & 11.17 & 0.02 & 0.02 & 0.13 & 0.23 &II  \\
52 & 0.133 & 162.2 & 10.11 & 9.11 & 8.27 & 7.19 & 0.01 & 0.01 & 0.02 & 0.07 & I	     \\
62 & 0.188 & 218.3 & 9.05 & 8.26 & 7.59 & 6.77 & 0.00 & 0.00 & 0.01 & 0.02 & II	     \\
65 & 0.553 & 125.1 & 13.51 & 13.28 & -- & -- & 0.09 & 0.07 & -- & -- & --	     \\
66 & 0.376 & 135.7 & 13.25 & 13.29 & -- & -- & 0.10 & 0.13 & -- & -- & --	     \\
67 & 0.417 & 192.6 & -- & 13.70 & -- & -- & -- & 0.11 & -- & -- & --		     \\
69 & 0.561 & 136.4 & 11.52 & 10.99 & 10.60 & 9.87 & 0.02 & 0.02 & 0.06 & 0.09 &II   \\
70 & 0.116 & 120.5 & 12.41 & 12.22 & -- & -- & 0.06 & 0.07 & -- & -- & --	     \\
71 & 0.755 & 157.5 & 13.33 & -- & -- & -- & 0.06 & -- & -- & -- & --		     \\
73 & 0.138 & 128.1 & 13.82 & 13.28 & -- & -- & 0.21 & 0.12 & -- & -- & --	     \\
74 & 0.426 & 188.3 & 13.27 & 13.30 & -- & -- & 0.08 & 0.08 & -- & -- & --            \\
76 & 0.002 & 100.5 & 11.20 & 10.61 & 10.05 & -- & 0.06 & 0.04 & 0.43 & -- & --	     \\
78 & 0.06 & 108.8 & 12.40 & -- & -- & -- & 0.06 & -- & -- & -- & --		     \\
83 & 0.285 & 99.8 & 12.32 & 11.70 & 10.93 & 9.82 & 0.03 & 0.04 & 0.13 & 0.24 & --    \\
84 & 0.273 & 125.1 & 11.73 & 11.20 & 9.77 & -- & 0.05 & 0.04 & 0.13 & -- & II	     \\
85 & 0.035 & 102.3 & 10.55 & 9.92 & 9.24 & 8.31 & 0.01 & 0.01 & 0.03 & 0.06 & II	     \\
89 & 0.686 & 104.1 & 13.23 & 12.98 & -- & -- & 0.13 & 0.15 & -- & -- & --	     \\
90 & 0.293 & 174.5 & 12.61 & -- & -- & -- & 0.05 & -- & -- & -- & --		     \\
92 & 0.32 & 86 & 9.64 & 9.41 & 9.46 & -- & 0.01 & 0.01 & 0.08 & -- & --		     \\
96 & 0.516 & 71.9 & 8.97 & 8.04 & 7.26 & 6.39 & 0.01 & 0.01 & 0.05 & 0.10 & I	     \\
100 & 0.41 & 57.8 & 10.66 & 10.56 & -- & -- & 0.08 & 0.13 & -- & -- & --	     \\
101 & 0.544 & 79.4 & 14.09 & 14.04 & -- & -- & 0.19 & 0.20 & -- & -- & --            \\
112 & 0.378 & 24.5 & 6.91 & 5.93 & 4.69 & -- & 0.01 & 0.01 & 0.02 & -- & I	     \\
113 & 0.124 & 66.7 & 12.31 & 12.27 & 12.25 & -- & 0.02 & 0.03 & 0.43 & -- & --	     \\
118 & 0.379 & 20.3 & 7.28 & 6.73 & 5.60 & -- & 0.05 & 0.07 & 0.11 & -- & II	     \\
123 & 0.702 & 167.9 & 13.53 & 13.69 & -- & -- & 0.12 & 0.15 & -- & -- & --	     \\
125 & 0.117 & 18.7 & 8.35 & 7.40 & -- & -- & 0.21 & 0.20 & -- & -- & --		     \\
126 & 0.229 & 54.8 & 11.80 & 11.55 & 11.30 & -- & 0.02 & 0.03 & 0.35 & -- & --	     \\
130 & 0.117 & 42.8 & 12.15 & 11.60 & -- & -- & 0.11 & 0.07 & -- & -- & II	     \\
131 & 0.207 & 10.9 & 8.63 & 7.94 & 6.50 & 5.04 & 0.02 & 0.01 & 0.07 & 0.10 & I	     \\
135 & 0.154 & 24.4 & 12.05 & 11.87 & -- & -- & 0.07 & 0.09 & -- & -- & --	     \\
136 & 0.173 & 27.1 & 9.26 & 8.77 & 8.17 & 6.63 & 0.01 & 0.01 & 0.03 & 0.04 & II	     \\
140 & 0.469 & 49.7 & 8.90 & 8.35 & 7.81 & 7.02 & 0.00 & 0.00 & 0.01 & 0.01 &II      \\
141 & 0.295 & 51.8 & 11.59 & 10.74 & 10.21 & 9.58 & 0.03 & 0.02 & 0.07 & 0.14 &II   \\
142 & 0.22 & 53.3 & 10.62 & 9.98 & 9.43 & 8.44 & 0.02 & 0.02 & 0.04 & 0.04 & II	     \\
143 & 0.26 & 70.7 & 10.64 & 10.07 & 9.60 & 8.98 & 0.01 & 0.01 & 0.02 & 0.03 & II	     \\
144 & 0.322 & 60.9 & 11.28 & 11.00 & 10.86 & -- & 0.01 & 0.02 & 0.08 & -- & --	     \\
145 & 0.132 & 68.9 & 10.82 & 10.24 & 9.74 & 9.10 & 0.01 & 0.01 & 0.03 & 0.05 &II    \\
149 & 0.296 & 200.9 & -- & 13.02 & -- & -- & -- & 0.07 & -- & -- & --		     \\
150 & 0.217 & 117.3 & 12.74 & 12.61 & -- & -- & 0.03 & 0.03 & -- & -- & --	     \\
152 & 0.23 & 132 & 13.63 & -- & -- & -- & 0.07 & -- & -- & -- & --		     \\
153 & 0.224 & 141.1 & 12.88 & 12.77 & 12.40 & 10.42 & 0.02 & 0.04 & 0.18 & 0.08 & gal\\
210 & 0.258 & 74.6 & 11.71 & 11.33 & 10.79 & 10.19 & 0.01 & 0.02 & 0.05 & 0.08 &II  \\
412 & 0.438 & 215.4 & 14.04 & 13.94 & -- & -- & 0.09 & 0.11 & -- & -- & --           \\
413 & 0.138 & 163.2 & 12.21 & 11.60 & 10.50 & -- & 0.10 & 0.05 & 0.28 & -- & --	     \\
421 & 0.405 & 63 & 10.89 & 9.92 & -- & -- & 0.14 & 0.07 & -- & -- & --		     \\
425 & 0.36 & 174.6 & 13.44 & 13.37 & -- & -- & 0.08 & 0.10 & -- & -- & --	     \\
435 & 0.721 & 124.2 & 14.01 & 13.95 & -- & -- & 0.07 & 0.11 & -- & -- & --	     \\
460 & 0.38 & 51.6 & 12.42 & 11.90 & 11.83 & 11.04 & 0.02 & 0.02 & 0.12 & 0.23 &II   \\
\hline
south &  &  &  &  &  &  &  &  &  &  & 						     \\
43 & 0.497 & 343 & 11.44 & 11.10 & 10.71 & 9.99 & 0.01 & 0.01 & 0.04 & 0.03 & II	     \\
45 & 0.597 & 276.8 & 12.85 & 12.84 & -- & -- & 0.03 & 0.05 & -- & -- & --	     \\
49 & 0.189 & 251.6 & 12.37 & 12.22 & 12.03 & -- & 0.05 & 0.03 & 0.17 & -- & --	     \\
55 & 0.381 & 298.1 & 12.99 & -- & 13.18 & -- & 0.04 & -- & 0.34 & -- & --	     \\
64 & 0.248 & 215.7 & 10.38 & 10.35 & 10.27 & 10.11 & 0.01 & 0.01 & 0.04 & 0.10 & III \\
75 & 0.262 & 247.6 & 11.32 & 11.25 & 11.43 & -- & 0.02 & 0.02 & 0.06 & -- & --	     \\
79 & 0.378 & 292.7 & -- & 13.41 & -- & -- & -- & 0.16 & -- & -- & --		     \\
104 & 2.056 & 283.1 & 10.55 & 10.64 & 10.17 & 9.60 & 0.01 & 0.01 & 0.08 & 0.27 & --  \\
139 & 0.588 & 204.7 & 13.42 & -- & -- & -- & 0.04 & -- & -- & -- & --		     \\
151 & 0.184 & 305.8 & 12.31 & 12.22 & 11.47 & -- & 0.03 & 0.03 & 0.12 & -- & --	     \\
208 & 0.658 & 302.5 & 13.89 & 13.73 & -- & -- & 0.06 & 0.08 & -- & -- & --	     \\
212 & 0.543 & 315.8 & 12.66 & 12.23 & 11.75 & 11.16 & 0.03 & 0.03 & 0.10 & 0.21 &II \\
222 & 1.127 & 363.7 & 11.21 & 11.25 & 11.20 & 11.29 & 0.01 & 0.01 & 0.04 & 0.06 & III  \\
223 & 0.8 & 366.1 & 13.42 & 13.46 & -- & -- & 0.05 & 0.07 & -- & -- & --	     \\
259 & 0.617 & 418.8 & 8.24 & 8.27 & 8.22 & 8.12 & 0.00 & 0.00 & 0.01 & 0.01 & III	     \\
260 & 1.458 & 508.3 & 13.13 & 13.23 & -- & -- & 0.04 & 0.07 & -- & -- & --           \\
263 & 0.479 & 433.3 & 10.10 & 9.66 & 9.36 & 8.54 & 0.01 & 0.01 & 0.01 & 0.01 &II    \\
264 & 1.883 & 441.6 & 12.01 & 12.01 & -- & 11.75 & 0.02 & 0.04 & -- & 0.14 & --	     \\
265 & 0.245 & 428 & 11.28 & 10.90 & 10.59 & 9.75 & 0.01 & 0.01 & 0.03 & 0.02 &II    \\
267 & 0.295 & 440.2 & 8.30 & 8.43 & 8.27 & 8.24 & 0.00 & 0.00 & 0.01 & 0.02 & III	     \\
269 & 0.769 & 512.8 & 9.56 & 9.57 & 9.49 & 9.43 & 0.01 & 0.01 & 0.02 & 0.04 & III	     \\
272 & 1.206 & 437 & 12.45 & 12.33 & -- & -- & 0.02 & 0.03 & -- & -- & --	     \\
274 & 0.397 & 552.9 & 12.81 & 12.72 & 13.13 & -- & 0.02 & 0.04 & 0.28 & -- & --	     \\
275 & 0.921 & 402.8 & 13.06 & 12.97 & -- & -- & 0.04 & 0.08 & -- & -- & --	     \\
309 & 0.988 & 467.1 & 13.14 & 13.17 & -- & -- & 0.04 & 0.04 & -- & -- & --	     \\
315 & 1.049 & 558.3 & 13.11 & 13.08 & -- & -- & 0.04 & 0.05 & -- & -- & --	     \\
318 & 2.474 & 468.8 & 11.06 & 11.09 & 11.03 & 10.87 & 0.01 & 0.01 & 0.05 & 0.13 & III  \\
417 & 0.388 & 226.2 & 12.41 & 12.36 & -- & -- & 0.05 & 0.04 & -- & -- & --	     \\
433 & 1.732 & 249 & 9.04 & 8.98 & 8.62 & 8.49 & 0.00 & 0.00 & 0.01 & 0.02 & III	     \\
455 & 0.696 & 261 & 13.85 & -- & -- & -- & 0.09 & -- & -- & -- & --		     \\
468 & 0.73 & 358.2 & 12.52 & 12.23 & 12.07 & 11.47 & 0.03 & 0.03 & 0.07 & 0.07 &II  \\
476 & 1.344 & 423 & 12.10 & 12.14 & 11.87 & -- & 0.02 & 0.03 & 0.09 & -- & --	     \\
\hline
west &  &  &  &  &  &  &  &  &  &  & 						     \\
155 & 1.239 & 205.1 & 13.26 & 13.17 & -- & -- & 0.06 & 0.07 & -- & -- & --	     \\
156 & 2.386 & 261.9 & 11.77 & 11.73 & 11.63 & -- & 0.01 & 0.02 & 0.07 & -- & --	     \\
158 & 0.498 & 323.9 & 12.38 & 12.36 & 12.23 & -- & 0.03 & 0.04 & 0.12 & -- & --	     \\
159 & 0.039 & 227 & 13.13 & 13.01 & -- & -- & 0.06 & 0.07 & -- & -- & --	     \\
160 & 0.253 & 210.7 & 13.12 & 12.96 & -- & -- & 0.05 & 0.06 & -- & -- & --           \\
161 & 0.204 & 195.7 & 14.33 & -- & -- & -- & 0.10 & -- & -- & -- & --		     \\
162 & 0.438 & 387.4 & 8.01 & 8.06 & 7.94 & 7.94 & 0.00 & 0.00 & 0.01 & 0.02 & III	     \\
164 & 0.247 & 267.5 & 12.52 & 12.57 & 12.29 & -- & 0.02 & 0.03 & 0.09 & -- & --	     \\
165 & 0.318 & 363.3 & 11.88 & 11.82 & -- & 11.38 & 0.02 & 0.03 & -- & 0.17 & --	     \\
166 & 1.163 & 358.6 & 10.28 & 9.56 & 8.89 & 8.11 & 0.01 & 0.01 & 0.01 & 0.01 &II    \\
167 & 0.431 & 359.2 & 11.61 & 11.50 & 11.49 & 10.92 & 0.02 & 0.02 & 0.07 & 0.14 & III  \\
168 & 0.312 & 369.4 & 11.53 & 11.45 & -- & -- & 0.02 & 0.03 & -- & -- & --	     \\
170 & 0.435 & 266.1 & 13.12 & 13.08 & 13.30 & -- & 0.03 & 0.05 & 0.25 & -- & --	     \\
171 & 1.577 & 258 & -- & -- & -- & -- & -- & -- & -- & -- & --			     \\
172 & 0.345 & 308 & 9.50 & 9.03 & 8.70 & 8.08 & 0.01 & 0.01 & 0.01 & 0.01 & II	     \\
173 & 0.128 & 309.4 & 12.34 & 12.31 & 12.41 & -- & 0.02 & 0.03 & 0.11 & -- & --      \\
174 & 0.121 & 281.1 & 8.59 & 8.61 & 8.61 & 8.60 & 0.00 & 0.00 & 0.01 & 0.02 & III	     \\
175 & 0.154 & 288.7 & 12.09 & 12.06 & -- & -- & 0.02 & 0.03 & -- & -- & --	     \\
215 & 0.16 & 324.8 & 10.88 & 10.79 & 10.86 & 10.79 & 0.01 & 0.01 & 0.03 & 0.06 & III   \\
217 & 0.364 & 321.5 & 10.20 & 10.20 & 10.19 & 10.31 & 0.01 & 0.01 & 0.03 & 0.07 & III  \\
219 & 0.438 & 368.1 & -- & 11.88 & -- & -- & -- & 0.02 & -- & -- & --		     \\
224 & 1.123 & 385.8 & -- & -- & -- & -- & -- & -- & -- & -- & --		     \\
225 & 1.51 & 376.9 & 12.95 & 12.88 & -- & -- & 0.03 & 0.05 & -- & -- & --	     \\
282 & 0.249 & 475.3 & 12.79 & 12.77 & 12.82 & -- & 0.04 & 0.06 & 0.15 & -- & --	     \\
283 & 0.367 & 414.9 & 12.58 & 12.60 & 12.81 & -- & 0.04 & 0.05 & 0.14 & -- & --	     \\
286 & 0.567 & 501.9 & 8.09 & 8.19 & 8.12 & 7.97 & 0.00 & 0.00 & 0.01 & 0.01 & III	     \\
287 & 0.295 & 466.2 & 13.09 & 13.06 & -- & -- & 0.04 & 0.08 & -- & -- & --           \\
290 & 1.488 & 445.1 & 12.49 & 12.48 & 12.78 & -- & 0.03 & 0.05 & 0.16 & -- & --	     \\
293 & 0.892 & 419.7 & 12.36 & 12.34 & 12.29 & -- & 0.03 & 0.03 & 0.14 & -- & --	     \\
294 & 0.784 & 474.6 & 12.15 & 12.14 & 12.24 & 11.69 & 0.03 & 0.04 & 0.09 & 0.09 & III  \\
295 & 0.48 & 467.7 & 13.38 & 13.41 & -- & -- & 0.05 & 0.08 & -- & -- & --	     \\
297 & 0.835 & 564.7 & 11.30 & 11.27 & 11.14 & 11.16 & 0.01 & 0.01 & 0.05 & 0.16 & III  \\
320 & 1.491 & 531.6 & 13.10 & 13.10 & -- & -- & 0.06 & 0.08 & -- & -- & --	     \\
324 & 0.744 & 426.5 & 12.95 & 12.88 & -- & -- & 0.03 & 0.04 & -- & -- & --	     \\
329 & 1.392 & 527.6 & 13.09 & 13.19 & -- & -- & 0.03 & 0.07 & -- & -- & --	     \\
330 & 1.681 & 507.4 & 13.31 & 13.24 & -- & -- & 0.06 & 0.07 & -- & -- & --	     \\
331 & 0.932 & 586.3 & 11.77 & 11.74 & 11.73 & 11.31 & 0.02 & 0.02 & 0.10 & 0.29 & -- \\
332 & 0.545 & 523.3 & 13.74 & 13.80 & -- & -- & 0.06 & 0.12 & -- & -- & --           \\
333 & 1.832 & 578.8 & 11.22 & 11.16 & 10.91 & 10.42 & 0.01 & 0.01 & 0.04 & 0.08 & III  \\
334 & 0.731 & 554.5 & 11.75 & 11.73 & 11.51 & -- & 0.02 & 0.02 & 0.06 & -- & --	     \\
441 & 0.346 & 201 & -- & 14.16 & -- & -- & -- & 0.11 & -- & -- & --		     \\
442 & 0.771 & 279 & 14.20 & -- & -- & -- & 0.07 & -- & -- & -- & --		     \\
465 & 0.667 & 303 & 8.79 & 8.79 & 8.65 & 8.58 & 0.00 & 0.00 & 0.01 & 0.03 & III	     \\
478 & 0.719 & 462.6 & 13.46 & 13.28 & -- & -- & 0.06 & 0.09 & -- & -- & --	     \\
483 & 2.123 & 3 8.4 & 12.12 & 12.16 & 11.98 & -- & 0.03 & 0.04 & 0.08 & -- & --	     \\
484 & 0.319 & 460.8 & 12.35 & 11.97 & 11.63 & 10.95 & 0.02 & 0.02 & 0.07 & 0.12 &II \\
\enddata
%\tablenotetext{a}{Ratio of the unabsorbed flux of component 1 and
%component 2.}
%\tablenotetext{b}{Sources 39, 404 and 450 are not thought to be
%cluster members.} 
\end{deluxetable}

										     
										     


==> table_2.tex <==
\begin{deluxetable}{llllrrr}
%\tabletypesize{\normal}
\tablecaption{Faint X-ray sources detected in the RCW 108 Field \label{XSources_faint}}
\tablewidth{0pt}
\tablehead{
\colhead{SRC \#} &\colhead{CXOWSBJ} &\colhead{RA}  &\colhead{DEC}   & \colhead{Offaxis}   &
 \colhead{Src sig.} &\colhead{Counts} \\
\colhead{} &\colhead{} &\colhead{(J2000.0)}  &\colhead{(J2000.0)}   & \colhead{[arcsec.]}   &
\colhead{~} &  \colhead{[Net]}} 
\startdata
401&164028.1-484956.6&16:40:28.109&-48:49:56.59&313.2&3.1&8.1\\
402&164027.4-485040.1&16:40:27.481&-48:50:40.14&293.4&2.1&5.0\\
403&164027.3-485116.9&16:40:27.339&-48:51:16.89&285.0&1.9&4.2\\
404&164026.2-484749.1&16:40:26.210&-48:47:49.05&366.0&3.0&8.5\\
405&164022.5-485512.0&16:40:22.533&-48:55:11.96&307.2&2.2&5.0\\
406&164022.4-485231.4&16:40:22.425&-48:52:31.37&237.0&2.5&5.9\\
407&164022.3-485650.1&16:40:22.357&-48:56:50.06&376.8&3.0&9.4\\
408&164022.0-485025.4&16:40:22.038&-48:50:25.39&247.2&2.8&6.8\\
409&164021.0-485202.1&16:40:21.037&-48:52:02.06&220.8&2.1&5.0\\
410&164019.9-484945.7&16:40:19.991&-48:49:45.75&246.6&2.8&6.8\\
411&164019.6-485314.3&16:40:19.635&-48:53:14.30&221.4&3.1&7.1\\
412&164018.8-485317.6&16:40:18.827&-48:53:17.69&215.4&2.3&5.2\\
413&164015.1-485141.6&16:40:15.188&-48:51:41.64&163.2&3.3&8.4\\
414&164013.3-484853.1&16:40:13.316&-48:48:53.11&231.6&3.0&7.0\\
415&164010.9-484742.8&16:40:10.964&-48:47:42.86&279.0&2.2&4.6\\
416&164009.7-484743.2&16:40:09.777&-48:47:43.29&273.6&2.6&5.5\\
417&164006.8-485525.3&16:40:06.835&-48:55:25.35&226.2&3.2&7.8\\
418&164006.5-485214.1&16:40:06.514&-48:52:14.17& 79.8&1.7&4.0\\
419&164006.1-484728.2&16:40:06.178&-48:47:28.22&276.0&3.4&8.0\\
420&164005.6-484811.0&16:40:05.667&-48:48:11.03&233.4&2.0&4.4\\
421&164005.0-485153.9&16:40:05.062&-48:51:53.97& 63.0&2.3&5.7\\
422&164004.7-484630.4&16:40:04.726&-48:46:30.44&329.4&3.5&8.0\\
423&164004.6-485338.5&16:40:04.624&-48:53:38.54&119.4&3.2&7.7\\
424&164003.8-485500.3&16:40:03.819&-48:55:00.38&193.2&2.9&6.9\\
425&164002.7-484903.9&16:40:02.743&-48:49:03.96&174.6&2.7&6.1\\
426&164002.1-485203.0&16:40:02.181&-48:52:03.01& 35.4&3.4&9.5\\
427&164000.1-485214.8&16:40:00.134&-48:52:14.80& 25.2&3.3&7.8\\
428&163957.4-484802.6&16:39:57.470&-48:48:02.68&231.6&1.6&3.4\\
429&163957.3-485128.2&16:39:57.344&-48:51:28.25& 29.4&1.8&4.5\\
430&163956.5-485004.2&16:39:56.567&-48:50:04.25&111.6&3.4&7.9\\
431&163954.3-485715.7&16:39:54.355&-48:57:15.75&324.6&2.8&6.2\\
432&163954.3-484833.6&16:39:54.343&-48:48:33.67&205.2&3.4&8.0\\
433&163953.0-485556.8&16:39:53.057&-48:55:56.85&249.0&3.2&7.7\\
434&163950.8-484959.2&16:39:50.817&-48:49:59.26&138.6&2.4&5.3\\
435&163950.1-485022.9&16:39:50.127&-48:50:22.96&124.2&2.3&5.2\\
436&163946.4-485109.1&16:39:46.473&-48:51:09.10&129.0&1.9&4.2\\
437&163943.4-485059.8&16:39:43.475&-48:50:59.86&159.6&2.9&6.9\\
438&163941.9-485657.4&16:39:41.984&-48:56:57.40&345.0&1.8&4.1\\
439&163941.2-485139.4&16:39:41.237&-48:51:39.42&172.8&2.5&5.9\\
440&163939.4-485142.6&16:39:39.454&-48:51:42.66&190.2&2.4&5.3\\
441&163938.5-485123.1&16:39:38.569&-48:51:23.12&201.0&2.9&6.8\\
442&163934.9-484923.4&16:39:34.916&-48:49:23.42&279.0&3.0&6.4\\
443&163934.7-485452.2&16:39:34.787&-48:54:52.29&295.2&2.7&6.1\\
444&163933.2-485341.8&16:39:33.281&-48:53:41.88&273.0&2.0&4.4\\
445&163930.2-484810.0&16:39:30.212&-48:48:10.02&359.4&2.7&8.0\\
446&163929.5-485100.7&16:39:29.555&-48:51:00.71&292.2&2.4&5.3\\
447&163928.3-485246.6&16:39:28.375&-48:52:46.64&303.6&2.4&5.3\\
448&164027.6-485521.9&16:40:27.605&-48:55:21.93&352.8&3.2&7.2\\
449&164024.5-485259.1&16:40:24.544&-48:52:59.17&263.4&2.2&5.0\\
450&164018.9-485206.3&16:40:18.921&-48:52:06.32&199.8&3.1&7.6\\
451&164018.2-485351.2&16:40:18.217&-48:53:51.28&225.6&3.0&7.0\\
452&164015.2-485155.9&16:40:15.258&-48:51:55.92&163.2&3.2&7.7\\
453&164011.9-484838.7&16:40:11.909&-48:48:38.74&235.2&3.2&8.3\\
454&164009.7-485241.5&16:40:09.721&-48:52:41.52&118.8&2.1&4.9\\
455&164009.0-485554.3&16:40:09.020&-48:55:54.33&261.0&3.3&8.3\\
456&164006.9-484710.5&16:40:06.904&-48:47:10.51&295.2&2.8&6.8\\
457&164001.3-485111.6&16:40:01.374&-48:51:11.64& 49.8&2.9&8.7\\
458&163959.7-485330.4&16:39:59.788&-48:53:30.49& 97.2&3.4&8.5\\
459&163958.4-485708.5&16:39:58.471&-48:57:08.52&314.4&3.3&7.8\\
460&163955.8-485237.4&16:39:55.856&-48:52:37.48& 51.6&2.7&7.1\\
461&163950.8-485723.8&16:39:50.853&-48:57:23.88&338.4&3.4&8.4\\
462&163949.6-485706.0&16:39:49.650&-48:57:06.07&324.6&1.5&3.3\\
463&163945.0-485510.1&16:39:45.083&-48:55:10.12&237.6&2.9&7.4\\
464&163934.3-485236.2&16:39:34.378&-48:52:36.23&243.6&3.1&7.7\\
465&163928.9-485312.2&16:39:28.985&-48:53:12.29&303.0&3.4&8.0\\
466&164034.2-485153.1&16:40:34.232&-48:51:53.14&351.0&2.9&7.4\\
467&164030.6-485459.1&16:40:30.640&-48:54:59.10&365.4&3.3&12.3\\
468&164016.2-485707.2&16:40:16.297&-48:57:07.24&358.2&2.1&5.0\\
469&164015.7-485555.1&16:40:15.757&-48:55:55.19&294.0&3.0&7.5\\
470&164003.8-485715.4&16:40:03.805&-48:57:15.40&325.2&3.1&7.7\\
471&164001.8-485811.3&16:40:01.835&-48:58:11.31&378.6&2.9&9.5\\
472&163957.6-485728.2&16:39:57.676&-48:57:28.28&334.2&1.9&4.2\\
473&163943.5-485339.8&16:39:43.529&-48:53:39.83&183.0&1.6&3.8\\
474&164039.1-484801.3&16:40:39.166&-48:48:01.36&462.6&2.1&6.7\\
475&164026.7-485742.1&16:40:26.716&-48:57:42.15&444.6&2.3&7.2\\
476&164001.8-485856.1&16:40:01.806&-48:58:56.13&423.0&2.6&6.9\\
477&163950.8-485823.7&16:39:50.879&-48:58:23.71&397.2&3.5&11.0\\
478&163921.6-485637.8&16:39:21.649&-48:56:37.85&462.6&2.6&7.8\\
479&163911.6-485210.9&16:39:11.680&-48:52:10.97&464.4&3.0&10.6\\
480&164048.5-485116.8&16:40:48.503&-48:51:16.84&493.2&2.9&10.4\\
481&164038.6-484641.0&16:40:38.668&-48:46:41.00&504.0&2.5&10.9\\
482&164008.1-485945.2&16:40:08.110&-48:59:45.26&480.0&3.1&9.9\\
483&163921.0-484928.8&16:39:21.098&-48:49:28.80&398.4&3.2&11.8\\
484&163913.3-485345.0&16:39:13.346&-48:53:45.09&460.8&3.2&10.6\\
485&164039.7-485238.1&16:40:39.731&-48:52:38.14&407.4&3.2&13.4\\
486&164033.1-485610.6&16:40:33.133&-48:56:10.63&425.4&2.8&9.7\\
487&164024.8-485941.8&16:40:24.835&-48:59:41.87&534.0&0.4&0.9\\
\enddata
\end{deluxetable}


==> table_5.tex <==
%Src,Q25,Q25_ERR,Q50,Q50_ERR,Q75,Q75_ERR,log(m/1-m),3*Q25/Q75
%,keV,keV,keV,keV,keV,keV,,
\begin{deluxetable}{lcccccccc}
%\begin{deluxetable}{123456789}
%\tabletypesize{\normal}
\tablecaption{Quartile Values of X-ray sources \label{quantin}}
\tablewidth{0pt}
\tablehead{
\colhead{SRC\#} &\colhead{Q25} &\colhead{Q25$_{err}$} &\colhead{M}&
\colhead{M$_{err}$}  & \colhead{Q75}   &\colhead{Q75$_{err}$} &
 \colhead{log(m/(1-m))} &\colhead{3*Q25/Q75} }
\startdata
East &  &  &  &  &  &  &  & \\
1 & 0.147 & 0.012 & 0.228 & 0.019 & 0.399 & 0.031 & -0.530 & 1.105    \\
2 & 0.100 & 0.005 & 0.145 & 0.011 & 0.208 & 0.017 & -0.771 & 1.442    \\
3 & 0.086 & 0.009 & 0.131 & 0.010 & 0.188 & 0.027 & -0.822 & 1.372    \\
4 & 0.108 & 0.003 & 0.153 & 0.003 & 0.224 & 0.012 & -0.743 & 1.446    \\
5 & 0.100 & 0.014 & 0.141 & 0.015 & 0.176 & 0.048 & -0.785 & 1.705    \\
6 & 0.106 & 0.006 & 0.133 & 0.012 & 0.177 & 0.019 & -0.814 & 1.797    \\
7 & 0.102 & 0.009 & 0.146 & 0.008 & 0.213 & 0.021 & -0.767 & 1.437    \\
8 & 0.124 & 0.008 & 0.180 & 0.010 & 0.254 & 0.035 & -0.659 & 1.465    \\
9 & 0.095 & 0.007 & 0.130 & 0.014 & 0.199 & 0.025 & -0.826 & 1.432    \\
10 & 0.095 & 0.015 & 0.146 & 0.011 & 0.249 & 0.060 & -0.767 & 1.145   \\
11 & 0.080 & 0.007 & 0.101 & 0.008 & 0.137 & 0.071 & -0.949 & 1.752   \\
12 & 0.111 & 0.003 & 0.168 & 0.005 & 0.294 & 0.015 & -0.695 & 1.133   \\
13 & 0.111 & 0.012 & 0.144 & 0.023 & 0.273 & 0.118 & -0.774 & 1.220   \\
14 & 0.089 & 0.014 & 0.154 & 0.019 & 0.226 & 0.109 & -0.740 & 1.181   \\
15 & 0.029 & 0.012 & 0.068 & 0.048 & 0.240 & 0.134 & -1.137 & 0.363   \\
16 & 0.099 & 0.005 & 0.138 & 0.006 & 0.213 & 0.016 & -0.796 & 1.394   \\
17 & 0.100 & 0.007 & 0.149 & 0.018 & 0.227 & 0.036 & -0.757 & 1.322   \\
18 & 0.132 & 0.014 & 0.164 & 0.017 & 0.235 & 0.037 & -0.707 & 1.685   \\
19 & 0.097 & 0.011 & 0.124 & 0.012 & 0.215 & 0.046 & -0.849 & 1.353   \\
20 & 0.083 & 0.006 & 0.119 & 0.018 & 0.169 & 0.012 & -0.869 & 1.473   \\
21 & 0.097 & 0.009 & 0.136 & 0.009 & 0.181 & 0.022 & -0.803 & 1.608   \\
22 & 0.089 & 0.005 & 0.128 & 0.012 & 0.200 & 0.030 & -0.833 & 1.335   \\
23 & 0.095 & 0.007 & 0.137 & 0.009 & 0.195 & 0.032 & -0.799 & 1.462   \\
24 & 0.105 & 0.010 & 0.147 & 0.010 & 0.205 & 0.039 & -0.764 & 1.537   \\
25 & 0.099 & 0.005 & 0.136 & 0.014 & 0.206 & 0.019 & -0.803 & 1.442   \\
26 & 0.099 & 0.004 & 0.130 & 0.013 & 0.199 & 0.012 & -0.826 & 1.492   \\
27 & 0.096 & 0.008 & 0.167 & 0.025 & 0.250 & 0.044 & -0.698 & 1.152   \\
28 & 0.085 & 0.004 & 0.110 & 0.007 & 0.150 & 0.014 & -0.908 & 1.700   \\
29 & 0.102 & 0.005 & 0.135 & 0.009 & 0.195 & 0.029 & -0.807 & 1.569   \\
30 & 0.090 & 0.004 & 0.138 & 0.006 & 0.201 & 0.012 & -0.796 & 1.343   \\
31 & 0.089 & 0.009 & 0.111 & 0.014 & 0.167 & 0.074 & -0.904 & 1.599   \\
32 & 0.123 & 0.011 & 0.178 & 0.020 & 0.311 & 0.043 & -0.664 & 1.186   \\
33 & 0.110 & 0.018 & 0.148 & 0.020 & 0.200 & 0.065 & -0.760 & 1.650   \\
34 & 0.082 & 0.006 & 0.109 & 0.012 & 0.137 & 0.016 & -0.912 & 1.796   \\
35 & 0.133 & 0.018 & 0.155 & 0.009 & 0.197 & 0.027 & -0.737 & 2.025   \\
36 & 0.097 & 0.017 & 0.142 & 0.016 & 0.192 & 0.030 & -0.781 & 1.516   \\
37 & 0.095 & 0.002 & 0.131 & 0.005 & 0.194 & 0.008 & -0.822 & 1.469   \\
38 & 0.092 & 0.009 & 0.134 & 0.023 & 0.226 & 0.039 & -0.810 & 1.221   \\
39 & 0.124 & 0.012 & 0.168 & 0.011 & 0.221 & 0.042 & -0.695 & 1.683   \\
40 & 0.117 & 0.005 & 0.169 & 0.010 & 0.282 & 0.026 & -0.692 & 1.245   \\
41 & 0.142 & 0.016 & 0.175 & 0.030 & 0.259 & 0.041 & -0.673 & 1.645   \\
177 & 0.116 & 0.006 & 0.158 & 0.020 & 0.328 & 0.076 & -0.727 & 1.061  \\
178 & 0.096 & 0.016 & 0.203 & 0.045 & 0.454 & 0.140 & -0.594 & 0.634  \\
179 & 0.178 & 0.027 & 0.326 & 0.035 & 0.473 & 0.056 & -0.315 & 1.129  \\
180 & 0.085 & 0.008 & 0.110 & 0.014 & 0.155 & 0.047 & -0.908 & 1.645  \\
181 & 0.098 & 0.023 & 0.159 & 0.024 & 0.245 & 0.098 & -0.723 & 1.200  \\
182 & 0.172 & 0.031 & 0.334 & 0.058 & 0.631 & 0.139 & -0.300 & 0.818  \\
183 & 0.105 & 0.021 & 0.175 & 0.040 & 0.341 & 0.056 & -0.673 & 0.924  \\
184 & 0.122 & 0.012 & 0.158 & 0.061 & 0.353 & 0.167 & -0.727 & 1.037  \\
185 & 0.102 & 0.016 & 0.167 & 0.057 & 0.374 & 0.088 & -0.698 & 0.818  \\
186 & 0.250 & 0.052 & 0.348 & 0.074 & 0.523 & 0.075 & -0.273 & 1.434  \\
187 & 0.098 & 0.016 & 0.131 & 0.032 & 0.217 & 0.069 & -0.822 & 1.355  \\
188 & 0.091 & 0.006 & 0.135 & 0.021 & 0.181 & 0.030 & -0.807 & 1.508  \\
189 & 0.075 & 0.015 & 0.156 & 0.030 & 0.255 & 0.041 & -0.733 & 0.882  \\
190 & 0.094 & 0.018 & 0.137 & 0.023 & 0.215 & 0.122 & -0.799 & 1.312  \\
191 & 0.150 & 0.026 & 0.214 & 0.034 & 0.401 & 0.110 & -0.565 & 1.122  \\
192 & 0.108 & 0.008 & 0.151 & 0.015 & 0.274 & 0.063 & -0.750 & 1.182  \\
193 & 0.107 & 0.016 & 0.156 & 0.019 & 0.220 & 0.093 & -0.733 & 1.459  \\
194 & 0.085 & 0.006 & 0.140 & 0.028 & 0.394 & 0.107 & -0.788 & 0.647  \\
195 & 0.098 & 0.017 & 0.160 & 0.031 & 0.335 & 0.098 & -0.720 & 0.878  \\
196 & 0.085 & 0.009 & 0.115 & 0.013 & 0.215 & 0.061 & -0.886 & 1.186  \\
197 & 0.139 & 0.017 & 0.185 & 0.030 & 0.292 & 0.229 & -0.644 & 1.428  \\
198 & 0.120 & 0.039 & 0.179 & 0.079 & 0.358 & 0.070 & -0.661 & 1.006  \\
199 & 0.108 & 0.026 & 0.211 & 0.081 & 0.377 & 0.098 & -0.573 & 0.859  \\
226 & 0.103 & 0.008 & 0.149 & 0.016 & 0.280 & 0.033 & -0.757 & 1.104  \\
227 & 0.107 & 0.007 & 0.168 & 0.011 & 0.251 & 0.033 & -0.695 & 1.279  \\
228 & 0.109 & 0.008 & 0.174 & 0.012 & 0.291 & 0.038 & -0.676 & 1.124  \\
229 & 0.120 & 0.014 & 0.185 & 0.016 & 0.328 & 0.060 & -0.644 & 1.098  \\
230 & 0.095 & 0.002 & 0.133 & 0.005 & 0.195 & 0.008 & -0.814 & 1.462  \\
231 & 0.095 & 0.002 & 0.135 & 0.005 & 0.194 & 0.009 & -0.807 & 1.469  \\
232 & 0.098 & 0.010 & 0.165 & 0.021 & 0.331 & 0.043 & -0.704 & 0.888  \\
233 & 0.093 & 0.003 & 0.127 & 0.007 & 0.191 & 0.012 & -0.837 & 1.461  \\
234 & 0.093 & 0.003 & 0.144 & 0.010 & 0.216 & 0.038 & -0.774 & 1.292  \\
235 & 0.106 & 0.008 & 0.153 & 0.011 & 0.371 & 0.087 & -0.743 & 0.857  \\
236 & 0.108 & 0.005 & 0.164 & 0.011 & 0.305 & 0.033 & -0.707 & 1.062  \\
237 & 0.088 & 0.004 & 0.125 & 0.010 & 0.184 & 0.020 & -0.845 & 1.435  \\
238 & 0.116 & 0.008 & 0.170 & 0.011 & 0.272 & 0.025 & -0.689 & 1.279  \\
239 & 0.091 & 0.004 & 0.130 & 0.013 & 0.208 & 0.029 & -0.826 & 1.313  \\
240 & 0.103 & 0.003 & 0.160 & 0.011 & 0.256 & 0.021 & -0.720 & 1.207  \\
241 & 0.094 & 0.004 & 0.139 & 0.008 & 0.237 & 0.031 & -0.792 & 1.190  \\
242 & 0.104 & 0.014 & 0.205 & 0.044 & 0.503 & 0.150 & -0.589 & 0.620  \\
243 & 0.066 & 0.004 & 0.085 & 0.005 & 0.133 & 0.010 & -1.032 & 1.489  \\
244 & 0.122 & 0.016 & 0.187 & 0.029 & 0.333 & 0.047 & -0.638 & 1.099  \\
245 & 0.105 & 0.002 & 0.152 & 0.002 & 0.224 & 0.006 & -0.747 & 1.406  \\
246 & 0.069 & 0.003 & 0.091 & 0.007 & 0.157 & 0.013 & -1.000 & 1.318  \\
247 & 0.094 & 0.004 & 0.136 & 0.007 & 0.197 & 0.016 & -0.803 & 1.431  \\
248 & 0.092 & 0.004 & 0.136 & 0.007 & 0.196 & 0.011 & -0.803 & 1.408  \\
249 & 0.138 & 0.020 & 0.214 & 0.039 & 0.443 & 0.113 & -0.565 & 0.935  \\
250 & 0.125 & 0.015 & 0.198 & 0.022 & 0.349 & 0.050 & -0.608 & 1.074  \\
251 & 0.087 & 0.008 & 0.149 & 0.019 & 0.191 & 0.033 & -0.757 & 1.366  \\
252 & 0.108 & 0.005 & 0.148 & 0.014 & 0.216 & 0.028 & -0.760 & 1.500  \\
253 & 0.098 & 0.005 & 0.142 & 0.010 & 0.193 & 0.012 & -0.781 & 1.523  \\
254 & 0.094 & 0.003 & 0.129 & 0.007 & 0.183 & 0.012 & -0.829 & 1.541  \\
255 & 0.096 & 0.003 & 0.145 & 0.005 & 0.214 & 0.012 & -0.771 & 1.346  \\
256 & 0.115 & 0.009 & 0.186 & 0.021 & 0.318 & 0.075 & -0.641 & 1.085  \\
257 & 0.101 & 0.003 & 0.141 & 0.004 & 0.201 & 0.008 & -0.785 & 1.507  \\
298 & 0.102 & 0.006 & 0.155 & 0.014 & 0.307 & 0.041 & -0.737 & 0.997  \\
300 & 0.225 & 0.035 & 0.372 & 0.025 & 0.588 & 0.085 & -0.227 & 1.148  \\
301 & 0.100 & 0.010 & 0.164 & 0.016 & 0.239 & 0.034 & -0.707 & 1.255  \\
303 & 0.088 & 0.013 & 0.157 & 0.035 & 0.519 & 0.111 & -0.730 & 0.509  \\
304 & 0.097 & 0.014 & 0.162 & 0.024 & 0.343 & 0.140 & -0.714 & 0.848  \\
305 & 0.085 & 0.006 & 0.112 & 0.016 & 0.192 & 0.055 & -0.899 & 1.328  \\
306 & 0.089 & 0.008 & 0.129 & 0.042 & 0.397 & 0.075 & -0.829 & 0.673  \\
307 & 0.251 & 0.047 & 0.420 & 0.107 & 0.683 & 0.057 & -0.140 & 1.102  \\
308 & 0.109 & 0.012 & 0.169 & 0.023 & 0.255 & 0.147 & -0.692 & 1.282  \\
337 & 0.096 & 0.009 & 0.158 & 0.047 & 0.533 & 0.103 & -0.727 & 0.540\\
\tableline
North &  &  &  &  &  &  &  & 					      \\
46 & 0.093 & 0.004 & 0.124 & 0.009 & 0.183 & 0.016 & -0.849 & 1.525   \\
59 & 0.112 & 0.009 & 0.150 & 0.014 & 0.226 & 0.054 & -0.753 & 1.487   \\
60 & 0.291 & 0.028 & 0.421 & 0.056 & 0.589 & 0.072 & -0.138 & 1.482   \\
61 & 0.151 & 0.003 & 0.209 & 0.006 & 0.365 & 0.012 & -0.578 & 1.241   \\
115 & 0.070 & 0.040 & 0.220 & 0.162 & 0.675 & 0.135 & -0.550 & 0.311  \\
133 & 0.133 & 0.012 & 0.188 & 0.025 & 0.280 & 0.038 & -0.635 & 1.425  \\
134 & 0.135 & 0.010 & 0.189 & 0.009 & 0.314 & 0.024 & -0.633 & 1.290  \\
146 & 0.126 & 0.008 & 0.170 & 0.010 & 0.270 & 0.025 & -0.689 & 1.400  \\
201 & 0.109 & 0.009 & 0.138 & 0.007 & 0.221 & 0.062 & -0.796 & 1.480  \\
202 & 0.109 & 0.024 & 0.205 & 0.043 & 0.279 & 0.068 & -0.589 & 1.172  \\
204 & 0.222 & 0.059 & 0.346 & 0.091 & 0.490 & 0.179 & -0.277 & 1.359  \\
206 & 0.133 & 0.008 & 0.193 & 0.023 & 0.335 & 0.036 & -0.621 & 1.191  \\
211 & 0.040 & 0.017 & 0.100 & 0.034 & 0.162 & 0.206 & -0.954 & 0.741  \\
258 & 0.094 & 0.006 & 0.137 & 0.010 & 0.183 & 0.021 & -0.799 & 1.541  \\
261 & 0.183 & 0.021 & 0.332 & 0.026 & 0.493 & 0.034 & -0.304 & 1.114  \\
262 & 0.111 & 0.004 & 0.159 & 0.007 & 0.241 & 0.016 & -0.723 & 1.382  \\
266 & 0.259 & 0.030 & 0.413 & 0.020 & 0.561 & 0.027 & -0.153 & 1.385  \\
268 & 0.247 & 0.022 & 0.386 & 0.039 & 0.572 & 0.026 & -0.202 & 1.295  \\
270 & 0.145 & 0.018 & 0.265 & 0.044 & 0.469 & 0.047 & -0.443 & 0.928  \\
271 & 0.084 & 0.006 & 0.129 & 0.012 & 0.192 & 0.015 & -0.829 & 1.313  \\
273 & 0.108 & 0.043 & 0.216 & 0.090 & 0.677 & 0.119 & -0.560 & 0.479  \\
276 & 0.079 & 0.005 & 0.098 & 0.009 & 0.154 & 0.065 & -0.964 & 1.539  \\
277 & 0.109 & 0.012 & 0.163 & 0.013 & 0.275 & 0.044 & -0.711 & 1.189  \\
278 & 0.127 & 0.007 & 0.185 & 0.013 & 0.364 & 0.030 & -0.644 & 1.047  \\
279 & 0.241 & 0.027 & 0.401 & 0.038 & 0.603 & 0.037 & -0.174 & 1.199  \\
312 & 0.129 & 0.022 & 0.271 & 0.084 & 0.479 & 0.098 & -0.430 & 0.808  \\
313 & 0.221 & 0.044 & 0.384 & 0.044 & 0.620 & 0.110 & -0.205 & 1.069  \\
316 & 0.117 & 0.012 & 0.165 & 0.031 & 0.275 & 0.160 & -0.704 & 1.276  \\
317 & 0.192 & 0.041 & 0.318 & 0.082 & 0.632 & 0.100 & -0.331 & 0.911  \\
319 & 0.154 & 0.016 & 0.240 & 0.050 & 0.560 & 0.072 & -0.501 & 0.825  \\
339 & 0.100 & 0.018 & 0.173 & 0.033 & 0.437 & 0.101 & -0.679 & 0.686  \\
\tableline
Inner &  &  &  &  &  &  &  & 					      \\
42 & 0.273 & 0.049 & 0.380 & 0.079 & 0.551 & 0.055 & -0.213 & 1.486   \\
44 & 0.145 & 0.024 & 0.190 & 0.031 & 0.277 & 0.043 & -0.630 & 1.570   \\
47 & 0.075 & 0.007 & 0.096 & 0.016 & 0.146 & 0.018 & -0.974 & 1.541   \\
48 & 0.137 & 0.033 & 0.211 & 0.030 & 0.234 & 0.168 & -0.573 & 1.756   \\
50 & 0.143 & 0.020 & 0.181 & 0.015 & 0.249 & 0.041 & -0.656 & 1.723   \\
51 & 0.261 & 0.057 & 0.413 & 0.048 & 0.520 & 0.086 & -0.153 & 1.506   \\
52 & 0.267 & 0.074 & 0.516 & 0.119 & 0.706 & 0.069 & 0.028 & 1.135    \\
56 & 0.160 & 0.017 & 0.229 & 0.029 & 0.391 & 0.077 & -0.527 & 1.228   \\
57 & 0.231 & 0.056 & 0.366 & 0.079 & 0.498 & 0.155 & -0.239 & 1.392   \\
58 & 0.179 & 0.021 & 0.199 & 0.050 & 0.388 & 0.070 & -0.605 & 1.384   \\
62 & 0.159 & 0.013 & 0.208 & 0.030 & 0.412 & 0.062 & -0.581 & 1.158   \\
63 & 0.143 & 0.039 & 0.243 & 0.041 & 0.282 & 0.077 & -0.493 & 1.521   \\
65 & 0.115 & 0.031 & 0.167 & 0.036 & 0.311 & 0.131 & -0.698 & 1.109   \\
66 & 0.065 & 0.009 & 0.079 & 0.007 & 0.093 & 0.093 & -1.067 & 2.097   \\
67 & 0.144 & 0.012 & 0.183 & 0.024 & 0.319 & 0.059 & -0.650 & 1.354   \\
68 & 0.148 & 0.011 & 0.203 & 0.057 & 0.403 & 0.054 & -0.594 & 1.102   \\
69 & 0.217 & 0.043 & 0.321 & 0.036 & 0.422 & 0.088 & -0.325 & 1.543   \\
70 & 0.180 & 0.008 & 0.286 & 0.015 & 0.426 & 0.015 & -0.397 & 1.268   \\
71 & 0.130 & 0.039 & 0.288 & 0.099 & 0.389 & 0.053 & -0.393 & 1.003   \\
72 & 0.467 & 0.030 & 0.578 & 0.028 & 0.701 & 0.052 & 0.137 & 1.999    \\
73 & 0.188 & 0.028 & 0.234 & 0.027 & 0.314 & 0.038 & -0.515 & 1.796   \\
74 & 0.147 & 0.015 & 0.211 & 0.030 & 0.297 & 0.049 & -0.573 & 1.485   \\
76 & 0.176 & 0.066 & 0.379 & 0.126 & 0.602 & 0.106 & -0.214 & 0.877   \\
77 & 0.205 & 0.058 & 0.314 & 0.060 & 0.522 & 0.095 & -0.339 & 1.178   \\
78 & 0.180 & 0.029 & 0.264 & 0.032 & 0.370 & 0.066 & -0.445 & 1.459   \\
80 & 0.046 & 0.018 & 0.088 & 0.018 & 0.123 & 0.019 & -1.016 & 1.122   \\
81 & 0.178 & 0.070 & 0.262 & 0.048 & 0.386 & 0.096 & -0.450 & 1.383   \\
82 & 0.191 & 0.040 & 0.336 & 0.046 & 0.511 & 0.063 & -0.296 & 1.121   \\
83 & 0.193 & 0.023 & 0.234 & 0.066 & 0.399 & 0.152 & -0.515 & 1.451   \\
84 & 0.306 & 0.008 & 0.411 & 0.009 & 0.581 & 0.019 & -0.156 & 1.580   \\
85 & 0.244 & 0.034 & 0.353 & 0.038 & 0.402 & 0.076 & -0.263 & 1.821   \\
86 & 0.210 & 0.027 & 0.359 & 0.038 & 0.459 & 0.037 & -0.252 & 1.373   \\
87 & 0.142 & 0.107 & 0.375 & 0.082 & 0.469 & 0.065 & -0.222 & 0.908   \\
89 & 0.222 & 0.030 & 0.344 & 0.039 & 0.408 & 0.046 & -0.280 & 1.632   \\
90 & 0.069 & 0.006 & 0.092 & 0.009 & 0.137 & 0.030 & -0.994 & 1.511   \\
91 & 0.180 & 0.052 & 0.379 & 0.067 & 0.416 & 0.051 & -0.214 & 1.298   \\
92 & 0.190 & 0.009 & 0.313 & 0.017 & 0.439 & 0.018 & -0.341 & 1.298   \\
93 & 0.178 & 0.010 & 0.229 & 0.026 & 0.379 & 0.044 & -0.527 & 1.409   \\
95 & 0.145 & 0.034 & 0.243 & 0.045 & 0.315 & 0.114 & -0.493 & 1.381   \\
96 & 0.402 & 0.095 & 0.521 & 0.043 & 0.663 & 0.050 & 0.037 & 1.819    \\
98 & 0.288 & 0.038 & 0.367 & 0.028 & 0.509 & 0.055 & -0.237 & 1.697   \\
99 & 0.211 & 0.035 & 0.338 & 0.069 & 0.433 & 0.167 & -0.292 & 1.462   \\
100 & 0.193 & 0.023 & 0.291 & 0.041 & 0.468 & 0.032 & -0.387 & 1.237  \\
101 & 0.082 & 0.017 & 0.141 & 0.025 & 0.158 & 0.054 & -0.785 & 1.557  \\
102 & 0.320 & 0.033 & 0.416 & 0.032 & 0.528 & 0.042 & -0.147 & 1.818  \\
103 & 0.319 & 0.036 & 0.405 & 0.026 & 0.475 & 0.030 & -0.167 & 2.015  \\
105 & 0.264 & 0.039 & 0.369 & 0.027 & 0.538 & 0.074 & -0.233 & 1.472  \\
106 & 0.058 & 0.011 & 0.084 & 0.011 & 0.118 & 0.045 & -1.038 & 1.475  \\
107 & 0.264 & 0.032 & 0.351 & 0.022 & 0.460 & 0.022 & -0.267 & 1.722  \\
108 & 0.351 & 0.055 & 0.463 & 0.041 & 0.572 & 0.033 & -0.064 & 1.841  \\
109 & 0.161 & 0.010 & 0.215 & 0.017 & 0.336 & 0.045 & -0.562 & 1.438  \\
110 & 0.449 & 0.046 & 0.547 & 0.022 & 0.647 & 0.066 & 0.082 & 2.082   \\
111 & 0.213 & 0.023 & 0.301 & 0.028 & 0.480 & 0.055 & -0.366 & 1.331  \\
112 & 0.189 & 0.026 & 0.231 & 0.056 & 0.378 & 0.073 & -0.522 & 1.500  \\
113 & 0.118 & 0.007 & 0.164 & 0.008 & 0.273 & 0.038 & -0.707 & 1.297  \\
114 & 0.257 & 0.023 & 0.320 & 0.020 & 0.436 & 0.035 & -0.327 & 1.768  \\
116 & 0.196 & 0.007 & 0.284 & 0.013 & 0.416 & 0.019 & -0.402 & 1.413  \\
117 & 0.289 & 0.031 & 0.373 & 0.030 & 0.487 & 0.045 & -0.226 & 1.780  \\
118 & 0.222 & 0.005 & 0.334 & 0.007 & 0.474 & 0.006 & -0.300 & 1.405  \\
119 & 0.546 & 0.020 & 0.670 & 0.029 & 0.796 & 0.021 & 0.308 & 2.058   \\
120 & 0.215 & 0.009 & 0.321 & 0.014 & 0.466 & 0.019 & -0.325 & 1.384  \\
121 & 0.164 & 0.013 & 0.257 & 0.029 & 0.365 & 0.067 & -0.461 & 1.348  \\
122 & 0.344 & 0.025 & 0.482 & 0.037 & 0.615 & 0.034 & -0.031 & 1.678  \\
123 & 0.067 & 0.024 & 0.108 & 0.030 & 0.134 & 0.058 & -0.917 & 1.500  \\
124 & 0.195 & 0.010 & 0.294 & 0.019 & 0.419 & 0.025 & -0.380 & 1.396  \\
125 & 0.269 & 0.021 & 0.361 & 0.023 & 0.542 & 0.032 & -0.248 & 1.489  \\
126 & 0.146 & 0.013 & 0.192 & 0.026 & 0.328 & 0.035 & -0.624 & 1.335  \\
127 & 0.374 & 0.078 & 0.484 & 0.041 & 0.539 & 0.035 & -0.028 & 2.082  \\
128 & 0.395 & 0.031 & 0.520 & 0.026 & 0.613 & 0.039 & 0.035 & 1.933   \\
129 & 0.488 & 0.091 & 0.591 & 0.035 & 0.720 & 0.058 & 0.160 & 2.033   \\
130 & 0.101 & 0.022 & 0.145 & 0.032 & 0.198 & 0.046 & -0.771 & 1.530  \\
131 & 0.228 & 0.008 & 0.367 & 0.010 & 0.498 & 0.011 & -0.237 & 1.373  \\
132 & 0.475 & 0.013 & 0.534 & 0.067 & 0.765 & 0.064 & 0.059 & 1.863   \\
135 & 0.295 & 0.064 & 0.344 & 0.058 & 0.483 & 0.166 & -0.280 & 1.832  \\
136 & 0.125 & 0.005 & 0.191 & 0.008 & 0.297 & 0.018 & -0.627 & 1.263  \\
137 & 0.083 & 0.012 & 0.096 & 0.020 & 0.122 & 0.103 & -0.974 & 2.041  \\
138 & 0.111 & 0.014 & 0.148 & 0.024 & 0.255 & 0.054 & -0.760 & 1.306  \\
140 & 0.177 & 0.013 & 0.264 & 0.062 & 0.426 & 0.075 & -0.445 & 1.246  \\
141 & 0.352 & 0.105 & 0.560 & 0.115 & 0.649 & 0.041 & 0.105 & 1.627   \\
142 & 0.172 & 0.019 & 0.225 & 0.060 & 0.408 & 0.069 & -0.537 & 1.265  \\
143 & 0.097 & 0.014 & 0.152 & 0.032 & 0.254 & 0.106 & -0.747 & 1.146  \\
144 & 0.258 & 0.041 & 0.318 & 0.058 & 0.446 & 0.041 & -0.331 & 1.735  \\
145 & 0.142 & 0.022 & 0.168 & 0.054 & 0.386 & 0.111 & -0.695 & 1.104  \\
147 & 0.020 & 0.007 & 0.035 & 0.026 & 0.105 & 0.115 & -1.440 & 0.571  \\
148 & 0.226 & 0.022 & 0.356 & 0.024 & 0.495 & 0.038 & -0.257 & 1.370  \\
149 & 0.134 & 0.033 & 0.163 & 0.047 & 0.231 & 0.163 & -0.711 & 1.740  \\
150 & 0.192 & 0.032 & 0.307 & 0.054 & 0.446 & 0.059 & -0.354 & 1.291  \\
152 & 0.174 & 0.018 & 0.217 & 0.063 & 0.382 & 0.083 & -0.557 & 1.366  \\
153 & 0.115 & 0.014 & 0.168 & 0.021 & 0.223 & 0.045 & -0.695 & 1.547  \\
154 & 0.312 & 0.034 & 0.383 & 0.074 & 0.565 & 0.131 & -0.207 & 1.657  \\
155 & 0.283 & 0.042 & 0.383 & 0.037 & 0.641 & 0.092 & -0.207 & 1.324  \\
209 & 0.400 & 0.086 & 0.604 & 0.176 & 0.828 & 0.083 & 0.183 & 1.449   \\
210 & 0.165 & 0.055 & 0.320 & 0.088 & 0.464 & 0.094 & -0.327 & 1.067  \\
214 & 0.011 & 0.007 & 0.018 & 0.029 & 0.072 & 0.074 & -1.737 & 0.458  \\
221 & 0.200 & 0.058 & 0.331 & 0.122 & 0.585 & 0.172 & -0.306 & 1.026  \\
\tableline
South &  &  &  &  &  &  &  & 					      \\
43 & 0.098 & 0.004 & 0.124 & 0.009 & 0.181 & 0.014 & -0.849 & 1.624   \\
45 & 0.111 & 0.011 & 0.142 & 0.015 & 0.208 & 0.068 & -0.781 & 1.601   \\
49 & 0.112 & 0.005 & 0.142 & 0.008 & 0.208 & 0.023 & -0.781 & 1.615   \\
53 & 0.201 & 0.013 & 0.362 & 0.022 & 0.534 & 0.027 & -0.246 & 1.129   \\
54 & 0.095 & 0.008 & 0.137 & 0.015 & 0.210 & 0.018 & -0.799 & 1.357   \\
55 & 0.108 & 0.007 & 0.150 & 0.012 & 0.199 & 0.015 & -0.753 & 1.628   \\
64 & 0.136 & 0.006 & 0.192 & 0.006 & 0.283 & 0.015 & -0.624 & 1.442   \\
75 & 0.103 & 0.007 & 0.132 & 0.012 & 0.181 & 0.023 & -0.818 & 1.707   \\
79 & 0.088 & 0.006 & 0.138 & 0.014 & 0.189 & 0.035 & -0.796 & 1.397   \\
88 & 0.136 & 0.016 & 0.181 & 0.016 & 0.272 & 0.082 & -0.656 & 1.500   \\
94 & 0.229 & 0.032 & 0.388 & 0.043 & 0.590 & 0.058 & -0.198 & 1.164   \\
97 & 0.224 & 0.043 & 0.348 & 0.061 & 0.569 & 0.087 & -0.273 & 1.181   \\
104 & 0.247 & 0.026 & 0.389 & 0.015 & 0.528 & 0.021 & -0.196 & 1.403  \\
139 & 0.082 & 0.007 & 0.095 & 0.015 & 0.141 & 0.048 & -0.979 & 1.745  \\
151 & 0.157 & 0.003 & 0.227 & 0.008 & 0.411 & 0.013 & -0.532 & 1.146  \\
200 & 0.104 & 0.013 & 0.148 & 0.031 & 0.221 & 0.184 & -0.760 & 1.412  \\
203 & 0.161 & 0.038 & 0.198 & 0.041 & 0.298 & 0.180 & -0.608 & 1.621  \\
205 & 0.091 & 0.006 & 0.106 & 0.014 & 0.147 & 0.076 & -0.926 & 1.857  \\
207 & 0.088 & 0.021 & 0.112 & 0.036 & 0.226 & 0.152 & -0.899 & 1.168  \\
208 & 0.149 & 0.032 & 0.236 & 0.054 & 0.432 & 0.198 & -0.510 & 1.035  \\
212 & 0.127 & 0.015 & 0.193 & 0.035 & 0.301 & 0.074 & -0.621 & 1.266  \\
213 & 0.195 & 0.061 & 0.445 & 0.105 & 0.654 & 0.124 & -0.096 & 0.894  \\
222 & 0.120 & 0.020 & 0.169 & 0.022 & 0.362 & 0.109 & -0.692 & 0.994  \\
223 & 0.124 & 0.027 & 0.202 & 0.049 & 0.422 & 0.151 & -0.597 & 0.882  \\
259 & 0.062 & 0.005 & 0.082 & 0.022 & 0.203 & 0.111 & -1.049 & 0.916  \\
260 & 0.100 & 0.004 & 0.143 & 0.005 & 0.194 & 0.017 & -0.778 & 1.546  \\
263 & 0.123 & 0.011 & 0.181 & 0.010 & 0.246 & 0.030 & -0.656 & 1.500  \\
264 & 0.096 & 0.005 & 0.136 & 0.016 & 0.216 & 0.079 & -0.803 & 1.333  \\
265 & 0.105 & 0.021 & 0.176 & 0.031 & 0.443 & 0.111 & -0.670 & 0.711  \\
267 & 0.069 & 0.004 & 0.095 & 0.004 & 0.141 & 0.014 & -0.979 & 1.468  \\
269 & 0.134 & 0.006 & 0.185 & 0.008 & 0.338 & 0.027 & -0.644 & 1.189  \\
272 & 0.104 & 0.023 & 0.199 & 0.047 & 0.446 & 0.091 & -0.605 & 0.700  \\
274 & 0.158 & 0.009 & 0.236 & 0.017 & 0.371 & 0.022 & -0.510 & 1.278  \\
275 & 0.099 & 0.007 & 0.140 & 0.018 & 0.276 & 0.040 & -0.788 & 1.076  \\
309 & 0.096 & 0.013 & 0.149 & 0.031 & 0.225 & 0.045 & -0.757 & 1.280  \\
310 & 0.165 & 0.016 & 0.281 & 0.045 & 0.469 & 0.043 & -0.408 & 1.055  \\
311 & 0.088 & 0.009 & 0.138 & 0.027 & 0.225 & 0.089 & -0.796 & 1.173  \\
314 & 0.093 & 0.006 & 0.144 & 0.026 & 0.340 & 0.100 & -0.774 & 0.821  \\
315 & 0.129 & 0.027 & 0.197 & 0.025 & 0.463 & 0.084 & -0.610 & 0.836  \\
318 & 0.136 & 0.020 & 0.188 & 0.058 & 0.440 & 0.202 & -0.635 & 0.927  \\
338 & 0.110 & 0.022 & 0.189 & 0.048 & 0.682 & 0.140 & -0.633 & 0.484  \\
\tableline
West &  &  &  &  &  &  &  & 					      \\
156 & 0.092 & 0.010 & 0.124 & 0.020 & 0.204 & 0.114 & -0.849 & 1.353  \\
157 & 0.161 & 0.013 & 0.246 & 0.022 & 0.381 & 0.040 & -0.486 & 1.268  \\
158 & 0.081 & 0.004 & 0.110 & 0.009 & 0.162 & 0.016 & -0.908 & 1.500  \\
159 & 0.076 & 0.022 & 0.112 & 0.026 & 0.172 & 0.029 & -0.899 & 1.326  \\
160 & 0.141 & 0.008 & 0.181 & 0.016 & 0.309 & 0.052 & -0.656 & 1.369  \\
161 & 0.089 & 0.004 & 0.104 & 0.011 & 0.136 & 0.044 & -0.935 & 1.963  \\
162 & 0.106 & 0.010 & 0.141 & 0.020 & 0.264 & 0.224 & -0.785 & 1.205  \\
163 & 0.090 & 0.011 & 0.116 & 0.034 & 0.261 & 0.066 & -0.882 & 1.034  \\
164 & 0.092 & 0.003 & 0.122 & 0.006 & 0.180 & 0.011 & -0.857 & 1.533  \\
165 & 0.104 & 0.005 & 0.157 & 0.006 & 0.269 & 0.019 & -0.730 & 1.160  \\
166 & 0.463 & 0.016 & 0.534 & 0.034 & 0.679 & 0.039 & 0.059 & 2.046   \\
167 & 0.174 & 0.005 & 0.266 & 0.015 & 0.425 & 0.020 & -0.441 & 1.228  \\
168 & 0.107 & 0.005 & 0.150 & 0.007 & 0.208 & 0.027 & -0.753 & 1.543  \\
169 & 0.188 & 0.020 & 0.228 & 0.071 & 0.441 & 0.107 & -0.530 & 1.279  \\
170 & 0.143 & 0.008 & 0.199 & 0.012 & 0.343 & 0.027 & -0.605 & 1.251  \\
171 & 0.054 & 0.006 & 0.074 & 0.005 & 0.095 & 0.039 & -1.097 & 1.705  \\
172 & 0.145 & 0.006 & 0.207 & 0.013 & 0.328 & 0.022 & -0.583 & 1.326  \\
173 & 0.139 & 0.012 & 0.214 & 0.016 & 0.347 & 0.036 & -0.565 & 1.202  \\
174 & 0.096 & 0.006 & 0.142 & 0.010 & 0.248 & 0.029 & -0.781 & 1.161  \\
175 & 0.179 & 0.015 & 0.253 & 0.046 & 0.429 & 0.083 & -0.470 & 1.252  \\
176 & 0.075 & 0.008 & 0.111 & 0.034 & 0.366 & 0.086 & -0.904 & 0.615  \\
215 & 0.053 & 0.005 & 0.075 & 0.007 & 0.101 & 0.014 & -1.091 & 1.574  \\
216 & 0.208 & 0.038 & 0.343 & 0.077 & 0.547 & 0.064 & -0.282 & 1.141  \\
217 & 0.089 & 0.015 & 0.123 & 0.013 & 0.177 & 0.064 & -0.853 & 1.508  \\
218 & 0.098 & 0.018 & 0.184 & 0.052 & 0.309 & 0.115 & -0.647 & 0.951  \\
219 & 0.102 & 0.017 & 0.156 & 0.021 & 0.271 & 0.041 & -0.733 & 1.129  \\
220 & 0.290 & 0.031 & 0.416 & 0.025 & 0.515 & 0.048 & -0.147 & 1.689  \\
224 & 0.071 & 0.019 & 0.154 & 0.093 & 0.636 & 0.185 & -0.740 & 0.335  \\
225 & 0.087 & 0.013 & 0.143 & 0.040 & 0.367 & 0.206 & -0.778 & 0.711  \\
280 & 0.258 & 0.020 & 0.387 & 0.026 & 0.512 & 0.017 & -0.200 & 1.512  \\
281 & 0.198 & 0.014 & 0.362 & 0.029 & 0.561 & 0.032 & -0.246 & 1.059  \\
282 & 0.110 & 0.008 & 0.175 & 0.015 & 0.310 & 0.038 & -0.673 & 1.065  \\
283 & 0.123 & 0.010 & 0.177 & 0.012 & 0.241 & 0.055 & -0.667 & 1.531  \\
284 & 0.356 & 0.024 & 0.530 & 0.020 & 0.631 & 0.022 & 0.052 & 1.693   \\
285 & 0.093 & 0.009 & 0.148 & 0.012 & 0.274 & 0.045 & -0.760 & 1.018  \\
286 & 0.083 & 0.003 & 0.112 & 0.012 & 0.180 & 0.027 & -0.899 & 1.383  \\
287 & 0.112 & 0.009 & 0.180 & 0.011 & 0.324 & 0.060 & -0.659 & 1.037  \\
288 & 0.127 & 0.008 & 0.196 & 0.020 & 0.366 & 0.045 & -0.613 & 1.041  \\
289 & 0.101 & 0.012 & 0.160 & 0.018 & 0.300 & 0.047 & -0.720 & 1.010  \\
290 & 0.076 & 0.005 & 0.106 & 0.008 & 0.198 & 0.016 & -0.926 & 1.152  \\
291 & 0.099 & 0.031 & 0.158 & 0.020 & 0.206 & 0.052 & -0.727 & 1.442  \\
292 & 0.074 & 0.009 & 0.113 & 0.019 & 0.221 & 0.061 & -0.895 & 1.005  \\
293 & 0.123 & 0.010 & 0.171 & 0.009 & 0.271 & 0.039 & -0.686 & 1.362  \\
294 & 0.091 & 0.003 & 0.122 & 0.009 & 0.204 & 0.016 & -0.857 & 1.338  \\
295 & 0.088 & 0.005 & 0.133 & 0.025 & 0.258 & 0.041 & -0.814 & 1.023  \\
296 & 0.146 & 0.019 & 0.214 & 0.044 & 0.435 & 0.112 & -0.565 & 1.007  \\
297 & 0.097 & 0.006 & 0.151 & 0.006 & 0.255 & 0.039 & -0.750 & 1.141  \\
320 & 0.129 & 0.014 & 0.178 & 0.019 & 0.348 & 0.088 & -0.664 & 1.112  \\
321 & 0.212 & 0.035 & 0.358 & 0.042 & 0.631 & 0.076 & -0.254 & 1.008  \\
322 & 0.130 & 0.016 & 0.199 & 0.027 & 0.419 & 0.067 & -0.605 & 0.931  \\
323 & 0.087 & 0.007 & 0.132 & 0.015 & 0.289 & 0.108 & -0.818 & 0.903  \\
324 & 0.101 & 0.013 & 0.173 & 0.020 & 0.265 & 0.105 & -0.679 & 1.143  \\
325 & 0.179 & 0.018 & 0.236 & 0.046 & 0.491 & 0.100 & -0.510 & 1.094  \\
326 & 0.133 & 0.013 & 0.220 & 0.027 & 0.436 & 0.050 & -0.550 & 0.915  \\
327 & 0.095 & 0.006 & 0.181 & 0.037 & 0.370 & 0.075 & -0.656 & 0.770  \\
328 & 0.192 & 0.045 & 0.348 & 0.057 & 0.665 & 0.074 & -0.273 & 0.866  \\
329 & 0.127 & 0.019 & 0.184 & 0.019 & 0.384 & 0.077 & -0.647 & 0.992  \\
330 & 0.129 & 0.017 & 0.205 & 0.033 & 0.482 & 0.072 & -0.589 & 0.803  \\
331 & 0.130 & 0.017 & 0.223 & 0.025 & 0.444 & 0.057 & -0.542 & 0.878  \\
332 & 0.108 & 0.014 & 0.192 & 0.052 & 0.612 & 0.152 & -0.624 & 0.529  \\
333 & 0.138 & 0.008 & 0.203 & 0.032 & 0.419 & 0.031 & -0.594 & 0.988  \\
334 & 0.118 & 0.009 & 0.162 & 0.012 & 0.302 & 0.041 & -0.714 & 1.172  \\
340 & 0.101 & 0.010 & 0.183 & 0.032 & 0.368 & 0.086 & -0.650 & 0.823  \\
\enddata
\end{deluxetable}



















































































































































































































































































































































































==> table_7.tex <==
\begin{deluxetable}{lcccccccc}
\tabletypesize{\small}
\tablecaption{One Temperature Spectral Fits \label{1t}}
\tablewidth{0pt}
\tablehead{ 
\colhead{SRC\#} &\colhead{$\chi^2$ $^a$} & \colhead{\nh}
 & \colhead{\nh err }&\colhead{kT} &  \colhead{kT err} & 
\colhead{    Abs. Flux}& \colhead{    Unabs. Flux} & \colhead{Log L$_{x}$} \\ 
\colhead{}  & \colhead{per d.o.f.} & 
\colhead{10$^{22}~cm^{-2}$} & \colhead{10$^{22}~cm^{-2}$} &
\colhead{keV} & \colhead{keV} &\colhead{                         } &
\colhead{                         } &\colhead{ergs sec$^{-1}$}}
\startdata
East &     &      &      &      &      &        &        & \\
  1 & 0.62 & 0.55 & 0.15 & 5.51 & 1.87 & -13.73 & -13.53 & 30.77   \\
  2 & 0.58 & 0.44 & 0.08 & 1.10 & 0.08 & -13.90 & -13.40 & 30.91   \\
  3 & 0.53 & 0.79 & 0.09 & 0.61 & 0.07 & -14.29 & -13.28 & 31.03   \\
  4 & 0.47 & 0.17 & 0.03 & 2.65 & 0.31 & -13.14 & -12.95 & 31.36   \\
  5 & 0.29 & 1.03 & 0.18 & 0.56 & 0.11 & -14.87 & -13.63 & 30.67   \\
  6 & 0.51 & 0.34 & 0.12 & 1.14 & 0.13 & -14.42 & -13.99 & 30.31   \\
  7 & 0.37 & 0.09 & 0.06 & 2.34 & 0.54 & -13.87 & -13.72 & 30.58   \\
  8 & 0.38 & 0.40 & 0.10 & 2.52 & 0.54 & -13.80 & -13.52 & 30.79   \\
  9 & 0.39 & 0.58 & 0.12 & 0.95 & 0.15 & -14.42 & -13.78 & 30.53   \\
 10 & 0.35 & 0.04 & -- & 2.93 & 1.13 & -14.20 & -14.12 & 30.19 \\
 11 & 0.25 & 0.01 & -- & 1.02 & 0.18 & -14.57 & -14.48 & 29.83 \\
 12 & 0.56 & 0.20 & 0.04 & 4.01 & 0.54 & -13.05 & -12.89 & 31.41   \\
 13 & 0.39 & 0.73 & 0.16 & 0.82 & 0.15 & -14.67 & -13.86 & 30.45   \\
 14 & 0.37 & 0.01 & -- & 2.04 & 0.84 & -14.39 & -14.34 & 29.97 \\
 15 & 0.29 & 0.02 & -- & 0.09 & 0.01 & -13.80 & -13.11 & 31.20 \\
 16 & 0.39 & 0.14 & 0.06 & 2.13 & 0.42 & -13.73 & -13.53 & 30.77   \\
 17 & 0.30 & 0.31 & 0.13 & 1.38 & 0.26 & -14.39 & -14.02 & 30.28   \\
 18 & 0.38 & 0.98 & 0.20 & 1.09 & 0.21 & -14.50 & -13.77 & 30.53   \\
 19 & 0.39 & 0.68 & 0.13 & 0.76 & 0.17 & -14.64 & -13.82 & 30.48   \\
 20 & 0.31 & 0.17 & 0.10 & 1.00 & 0.13 & -14.46 & -14.13 & 30.17   \\
 21 & 0.37 & 0.81 & 0.12 & 0.83 & 0.10 & -14.29 & -13.44 & 30.87   \\
 22 & 0.31 & 0.28 & 0.11 & 1.02 & 0.15 & -14.44 & -14.02 & 30.29   \\
 23 & 0.35 & 0.01 & -- & 2.05 & 0.74 & -14.14 & -14.08 & 30.22 \\
 24 & 0.32 & 0.97 & 0.12 & 0.81 & 0.10 & -14.30 & -13.36 & 30.95   \\
 25 & 0.41 & 0.25 & 0.09 & 1.34 & 0.23 & -14.17 & -13.83 & 30.47   \\
 26 & 0.41 & 0.24 & 0.08 & 1.31 & 0.21 & -14.14 & -13.80 & 30.51   \\
 27 & 0.35 & 0.05 & -- & 2.67 & 1.11 & -14.28 & -14.18 & 30.13 \\
 28 & 0.33 & 0.04 & -- & 1.10 & 0.11 & -14.24 & -14.07 & 30.23 \\
 29 & 0.43 & 0.16 & 0.08 & 1.67 & 0.35 & -14.04 & -13.80 & 30.51   \\
 30 & 0.44 & 0.06 & 0.05 & 2.10 & 0.46 & -13.73 & -13.59 & 30.71   \\
 31 & 0.34 & 0.06 & -- & 1.09 & 0.21 & -14.67 & -14.48 & 29.83 \\
 32 & 0.28 & 0.19 & 0.11 & 5.21 & 2.04 & -13.97 & -13.83 & 30.47   \\
 33 & 0.18 & 1.05 & 0.23 & 0.85 & 0.19 & -14.86 & -13.92 & 30.38   \\
 34 & 0.19 & 0.08 & -- & 0.98 & 0.14 & -14.60 & -14.36 & 29.94 \\
 35 & 0.20 & 0.46 & 0.18 & 1.44 & 0.38 & -14.61 & -14.19 & 30.12   \\
 36 & 0.22 & 0.06 & -- & 2.09 & 0.72 & -14.44 & -14.30 & 30.00 \\
 37 & 0.29 & 0.40 & 0.05 & 1.09 & 0.06 & -13.69 & -13.21 & 31.10   \\
 38 & 0.36 & 0.89 & 0.15 & 0.75 & 0.12 & -14.63 & -13.66 & 30.64   \\
 39 & 0.23 & 0.38 & 0.14 & 2.27 & 0.66 & -14.23 & -13.94 & 30.37   \\
 40 & 0.31 & 0.29 & 0.09 & 2.93 & 0.65 & -13.81 & -13.59 & 30.72   \\
 41 & 0.16 & 1.63 & 0.34 & 0.90 & 0.19 & -14.84 & -13.77 & 30.53   \\
177 & 0.45 & 1.10 & 0.15 & 0.79 & 0.12 & -14.41 & -13.39 & 30.92   \\
178 & 0.52 & 0.20 & -- & 0.01 & -- & -27.93 & -18.37 & 25.94\\
179 & 0.49 & 0.88 & 0.34 & 5.96 & 2.72 & -14.05 & -13.83 & 30.47   \\
180 & 0.23 & 0.93 & 0.12 & 0.29 & 0.03 & -14.72 & -13.04 & 31.27   \\
181 & 0.29 & 1.10 & 0.20 & 0.44 & 0.08 & -14.98 & -13.54 & 30.77   \\
182 & 0.47 & 0.65 & 0.37 & 5.96 & 3.88 & -14.42 & -14.22 & 30.09   \\
183 & 0.31 & 0.16 & -- & 3.71 & 1.89 & -14.50 & -14.35 & 29.95 \\
184 & 0.33 & 0.66 & 0.29 & 1.27 & 0.41 & -14.91 & -14.37 & 29.94   \\
185 & 0.27 & 0.04 & -- & 3.39 & -- & -14.69 & -14.61 & 29.70\\
186 & 0.34 & 3.52 & 1.13 & 2.93 & 1.09 & -14.47 & -13.92 & 30.38   \\
187 & 0.35 & 0.99 & 0.23 & 0.71 & 0.14 & -14.96 & -13.91 & 30.40   \\
188 & 0.37 & 0.15 & 0.10 & 1.10 & 0.13 & -14.48 & -14.18 & 30.12   \\
189 & 0.27 & 0.01 & -- & 2.32 & -- & -14.53 & -14.48 & 29.83\\
190 & 0.33 & 0.01 & -- & 1.55 & 0.50 & -14.76 & -14.69 & 29.62 \\
191 & 0.31 & 1.18 & 0.39 & 1.62 & 0.59 & -14.63 & -14.06 & 30.25   \\
192 & 0.54 & 0.54 & 0.13 & 1.06 & 0.15 & -14.39 & -13.82 & 30.48   \\
193 & 0.36 & 0.96 & 0.21 & 0.79 & 0.24 & -14.86 & -13.90 & 30.41   \\
194 & 0.53 & 0.19 & 0.12 & 0.87 & 0.12 & -14.61 & -14.24 & 30.07   \\
195 & 0.35 & 0.23 & -- & 0.01 & -- & -28.65 & -18.53 & 25.78\\
196 & 0.53 & 0.01 & -- & 1.14 & 0.17 & -14.47 & -14.39 & 29.92 \\
197 & 0.32 & 0.78 & 0.31 & 1.44 & 0.44 & -14.79 & -14.26 & 30.04   \\
198 & 0.34 & 0.37 & -- & 0.01 & -- & -29.18 & -16.87 & 27.43\\
199 & 0.30 & 0.27 & -- & 3.35 & -- & -14.77 & -14.57 & 29.74\\
226 & 0.66 & 0.01 & -- & 3.08 & 0.94 & -13.67 & -13.63 & 30.67 \\
227 & 0.49 & 0.12 & 0.09 & 2.12 & 0.55 & -13.98 & -13.79 & 30.51   \\
228 & 0.39 & 0.13 & 0.09 & 2.63 & 0.81 & -13.93 & -13.76 & 30.54   \\
229 & 0.39 & 0.01 & -- & 8.44 & -- & -13.61 & -13.59 & 30.72\\
230 & 0.70 & 0.06 & 0.04 & 1.35 & 0.11 & -13.46 & -13.28 & 31.02   \\
231 & 0.72 & 0.08 & 0.04 & 1.34 & 0.11 & -13.49 & -13.29 & 31.01   \\
232 & 0.67 & 0.76 & 0.14 & 0.88 & 0.12 & -14.31 & -13.54 & 30.77   \\
233 & 0.67 & 0.01 & -- & 1.25 & 0.14 & -13.71 & -13.63 & 30.68 \\
234 & 0.64 & 0.01 & -- & 1.38 & 0.18 & -13.85 & -13.78 & 30.52 \\
235 & 0.57 & 0.06 & -- & 1.36 & 0.24 & -14.18 & -14.00 & 30.30 \\
236 & 0.62 & 0.10 & 0.07 & 2.41 & 0.67 & -13.79 & -13.63 & 30.68   \\
237 & 0.43 & 0.02 & -- & 1.07 & 0.12 & -14.12 & -14.00 & 30.30 \\
238 & 0.55 & 0.16 & 0.08 & 2.81 & 0.77 & -13.81 & -13.63 & 30.68   \\
239 & 0.50 & 0.14 & 0.10 & 1.11 & 0.14 & -14.36 & -14.06 & 30.24   \\
240 & 0.59 & 0.11 & 0.06 & 2.46 & 0.47 & -13.64 & -13.47 & 30.83   \\
241 & 0.64 & 0.09 & 0.06 & 1.30 & 0.21 & -13.83 & -13.62 & 30.69   \\
242 & 0.35 & 0.01 & -- & 1.19 & 0.27 & -14.68 & -14.60 & 29.71 \\
243 & 0.38 & 0.35 & 0.05 & 0.30 & 0.02 & -13.96 & -13.11 & 31.20   \\
244 & 0.51 & 0.73 & 0.23 & 1.69 & 0.45 & -14.38 & -13.92 & 30.39   \\
245 & 0.76 & 0.16 & 0.02 & 2.59 & 0.20 & -12.76 & -12.58 & 31.73   \\
246 & 0.44 & 0.48 & 0.06 & 0.42 & 0.03 & -14.13 & -13.25 & 31.05   \\
247 & 0.57 & 0.05 & -- & 1.48 & 0.27 & -13.78 & -13.63 & 30.68 \\
248 & 0.57 & 0.08 & 0.05 & 1.34 & 0.15 & -13.76 & -13.56 & 30.75   \\
249 & 0.51 & 1.58 & 0.34 & 0.82 & 0.22 & -14.74 & -13.58 & 30.72   \\
250 & 0.57 & 0.29 & 0.13 & 4.24 & 1.63 & -13.97 & -13.80 & 30.51   \\
251 & 0.49 & 0.52 & 0.12 & 0.78 & 0.14 & -14.56 & -13.87 & 30.44   \\
252 & 0.53 & 0.40 & 0.10 & 1.32 & 0.22 & -14.09 & -13.67 & 30.64   \\
253 & 0.53 & 0.53 & 0.09 & 1.03 & 0.10 & -14.03 & -13.46 & 30.85   \\
254 & 0.54 & 0.48 & 0.07 & 0.92 & 0.07 & -14.03 & -13.43 & 30.87   \\
255 & 0.62 & 0.06 & 0.03 & 2.24 & 0.29 & -13.33 & -13.19 & 31.11   \\
256 & 0.53 & 1.20 & 0.17 & 0.72 & 0.10 & -14.49 & -13.35 & 30.96   \\
257 & 0.69 & 0.15 & 0.04 & 1.91 & 0.28 & -13.31 & -13.09 & 31.22   \\
298 & 0.30 & 0.01 & -- & 4.31 & 1.43 & -13.52 & -13.49 & 30.82 \\
300 & 0.24 & 1.46 & 0.40 & $>$15 & -- & -13.59 & -13.44 & 30.86\\
301 & 0.17 & 0.01 & -- & 3.83 & 1.51 & -13.50 & -13.47 & 30.84 \\
303 & 0.51 & 0.75 & 0.14 & 0.29 & 0.04 & -14.78 & -13.32 & 30.98   \\
304 & 0.49 & 0.24 & 0.14 & 1.07 & 0.18 & -14.55 & -14.17 & 30.14   \\
305 & 0.53 & 0.79 & 0.09 & 0.32 & 0.03 & -14.44 & -13.01 & 31.29   \\
306 & 0.43 & 0.03 & -- & 1.06 & 0.21 & -14.64 & -14.50 & 29.80 \\
307 & 0.51 & 2.43 & 1.12 & $>$15 & -- & -14.18 & -13.99 & 30.31\\
308 & 0.55 & 1.05 & 0.16 & 0.56 & 0.09 & -14.71 & -13.46 & 30.85   \\
337 & 0.55 & 0.94 & 0.15 & 0.40 & 0.06 & -14.66 & -13.29 & 31.01   \\
\tableline
North &  &  &  &  &  &   &   &                         \\
46 & 0.34 & 0.06 & -- & 1.35 & 0.21 & -14.12 & -13.94 & 30.37  \\
59 & 0.28 & 0.24 & 0.14 & 2.20 & 0.76 & -14.38 & -14.14 & 30.17	   \\
60 & 0.35 & 8.31 & 1.71 & 1.56 & 0.28 & -14.31 & -13.18 & 31.13	   \\
61 & 0.62 & 0.81 & 0.05 & 3.65 & 0.30 & -12.82 & -12.53 & 31.77	   \\
115 & 0.33 & 0.01 & -- & 0.37 & 0.15 & -15.09 & -15.00 & 29.30 \\
133 & 0.36 & 1.18 & 0.26 & 1.24 & 0.26 & -14.52 & -13.82 & 30.49   \\
134 & 0.44 & 0.43 & 0.10 & 3.18 & 0.75 & -13.77 & -13.52 & 30.79   \\
146 & 0.39 & 0.37 & 0.10 & 2.39 & 0.59 & -13.93 & -13.65 & 30.66   \\
201 & 0.36 & 0.08 & -- & 2.24 & 0.82 & -14.31 & -14.16 & 30.14 \\
202 & 0.30 & 1.00 & 0.27 & 0.96 & 0.25 & -14.92 & -14.09 & 30.22   \\
204 & 0.31 & 3.34 & 1.27 & 2.12 & 0.87 & -14.84 & -14.16 & 30.15   \\
206 & 0.49 & 0.40 & 0.14 & 2.93 & 0.87 & -14.07 & -13.82 & 30.49   \\
211 & 0.30 & 0.01 & -- & 0.18 & 0.03 & -14.41 & -14.25 & 30.05 \\
258 & 0.49 & 0.18 & 0.10 & 1.22 & 0.19 & -14.28 & -13.97 & 30.34   \\
261 & 0.58 & 0.77 & 0.24 & 50.00 & 30.52 & -13.58 & -13.46 & 30.84 \\
262 & 0.67 & 0.26 & 0.06 & 2.02 & 0.34 & -13.49 & -13.22 & 31.09   \\
266 & 0.60 & 2.62 & 0.48 & $>$15 & -- & -13.42 & -13.19 & 31.11\\
268 & 0.57 & 2.60 & 0.48 & 11.68 & -- & -13.52 & -13.27 & 31.03\\
270 & 0.58 & 0.84 & 0.27 & 4.70 & 1.87 & -14.01 & -13.76 & 30.54   \\
271 & 0.50 & 0.75 & 0.09 & 0.62 & 0.08 & -14.27 & -13.30 & 31.01   \\
273 & 0.62 & 0.04 & 0.03 & 0.05 & 0.01 & -13.43 & -11.72 & 32.58   \\
276 & 0.44 & 0.99 & 0.09 & 0.14 & 0.01 & -14.58 & -11.51 & 32.79   \\
277 & 0.49 & 0.12 & -- & 2.12 & 0.65 & -14.22 & -14.04 & 30.27 \\
278 & 0.75 & 0.01 & -- & 6.35 & 2.55 & -13.57 & -13.54 & 30.76 \\
279 & 0.60 & 2.40 & 0.62 & 19.40 & -- & -13.65 & -13.43 & 30.87\\
312 & 0.40 & 0.24 & -- & 3.98 & -- & -14.65 & -14.48 & 29.82\\
313 & 0.48 & 1.77 & 0.62 & 9.03 & -- & -14.06 & -13.82 & 30.48 \\
316 & 0.55 & 0.01 & -- & 1.83 & -- & -14.42 & -14.36 & 29.94\\
317 & 0.46 & 1.98 & 0.86 & 3.76 & -- & -14.56 & -14.18 & 30.13 \\
319 & 0.64 & 2.75 & 0.40 & 0.31 & 0.04 & -14.85 & -12.29 & 32.02   \\
339 & 0.65 & 0.01 & -- & 2.01 & -- & -14.45 & -14.40 & 29.91\\
\tableline
RCW~108--IR &  &  &  &  &  &   &   &  			   \\
42 & 0.18 & 2.28 & 0.91 & $>$15 & -- & -14.22 & -14.00 & 30.30 \\
44 & 0.35 & 1.25 & 0.33 & 1.44 & 0.33 & -14.57 & -13.94 & 30.37	   \\
47 & 0.18 & 0.61 & 0.11 & 0.47 & 0.08 & -14.74 & -13.78 & 30.53	   \\
48 & 0.18 & 0.24 & -- & 7.54 & 5.12 & -14.51 & -14.39 & 29.92  \\
50 & 0.22 & 1.19 & 0.25 & 1.17 & 0.21 & -14.53 & -13.80 & 30.51	   \\
51 & 0.21 & 4.43 & 1.33 & 4.03 & 1.48 & -14.29 & -13.81 & 30.50	   \\
52 & 0.21 & 2.77 & 1.15 & $>$15 & -- & -14.21 & -14.02 & 30.29 \\
56 & 0.27 & 0.76 & 0.25 & 4.70 & 1.81 & -14.13 & -13.89 & 30.42	   \\
57 & 0.17 & 3.37 & 1.16 & 2.93 & 1.12 & -14.60 & -14.06 & 30.24	   \\
58 & 0.21 & 2.48 & 0.52 & 1.17 & 0.28 & -14.67 & -13.70 & 30.61	   \\
62 & 0.26 & 1.11 & 0.27 & 2.49 & 0.73 & -14.26 & -13.84 & 30.47	   \\
63 & 0.20 & 2.48 & 0.59 & 0.91 & 0.22 & -14.96 & -13.73 & 30.57	   \\
64 & 0.38 & 0.62 & 0.09 & 2.49 & 0.38 & -13.56 & -13.22 & 31.08	   \\
65 & 0.20 & 0.01 & -- & 6.88 & -- & -14.61 & -14.59 & 29.72\\
66 & 0.21 & 0.58 & 0.09 & 0.17 & 0.02 & -14.80 & -12.92 & 31.39	   \\
67 & 0.22 & 0.72 & 0.22 & 2.72 & 0.87 & -14.29 & -13.96 & 30.35	   \\
68 & 0.19 & 1.06 & 0.32 & 2.79 & 0.95 & -14.41 & -14.03 & 30.27	   \\
69 & 0.19 & 3.84 & 0.87 & 1.66 & 0.36 & -14.49 & -13.64 & 30.66	   \\
70 & 0.48 & 1.29 & 0.12 & 4.27 & 0.62 & -13.19 & -12.89 & 31.42	   \\
71 & 0.18 & 0.54 & 0.33 & 4.24 & -- & -14.52 & -14.29 & 30.01  \\
72 & 0.31 & 13.24 & 2.21 & 12.63 & -- & -13.43 & -12.98 & 31.32\\
73 & 0.17 & 3.02 & 0.55 & 0.81 & 0.14 & -14.74 & -13.29 & 31.02	   \\
74 & 0.21 & 1.47 & 0.32 & 1.14 & 0.22 & -14.66 & -13.84 & 30.47	   \\
76 & 0.19 & 2.24 & 0.94 & 5.96 & 3.18 & -14.55 & -14.24 & 30.06	   \\
77 & 0.20 & 5.32 & 1.20 & 1.32 & 0.26 & -14.59 & -13.46 & 30.85	   \\
78 & 0.23 & 2.18 & 0.52 & 1.63 & 0.38 & -14.49 & -13.78 & 30.53	   \\
80 & 0.16 & 0.73 & 0.10 & 0.12 & 0.01 & -14.92 & -12.12 & 32.19	   \\
81 & 0.17 & 0.01 & -- & $>$15  & -- & -14.54 & -14.52 & 29.78\\
82 & 0.19 & 1.11 & 0.45 & 40.43 & -- & -14.10 & -13.96 & 30.35 \\
83 & 0.14 & 3.96 & 0.84 & 0.73 & 0.16 & -14.97 & -13.23 & 31.08	   \\
84 & 0.41 & 4.15 & 0.33 & 5.16 & 0.68 & -13.00 & -12.59 & 31.72	   \\
85 & 0.16 & 5.07 & 0.95 & 1.24 & 0.21 & -14.48 & -13.30 & 31.00	   \\
86 & 0.15 & 3.38 & 0.63 & 2.25 & 0.46 & -14.14 & -13.49 & 30.82	   \\
87 & 0.16 & 0.01 & -- & $>$15 & -- & -14.64 & -14.62 & 29.68\\
89 & 0.17 & 6.12 & 0.90 & 0.91 & 0.12 & -14.45 & -12.79 & 31.52	   \\
90 & 0.20 & 0.05 & -- & 0.85 & 0.10 & -14.55 & -14.37 & 29.94  \\
91 & 0.20 & 1.61 & 0.61 & 3.71 & 1.56 & -14.55 & -14.18 & 30.12	   \\
92 & 0.36 & 2.22 & 0.25 & 3.22 & 0.49 & -13.52 & -13.08 & 31.23	   \\
93 & 0.27 & 2.07 & 0.32 & 1.66 & 0.26 & -14.14 & -13.45 & 30.85	   \\
95 & 0.18 & 0.51 & 0.31 & 5.17 & -- & -14.63 & -14.43 & 29.87  \\
96 & 0.26 & 9.80 & 3.41 & $>$15 & -- & -13.95 & -13.60 & 30.71 \\
98 & 0.21 & 9.86 & 1.56 & 1.02 & 0.11 & -14.35 & -12.63 & 31.67	   \\
99 & 0.19 & 3.32 & 1.02 & 2.05 & 0.72 & -14.70 & -14.00 & 30.30	   \\
100 & 0.29 & 1.77 & 0.34 & 3.43 & 0.85 & -13.98 & -13.58 & 30.72   \\
101 & 0.13 & 0.56 & 0.19 & 0.80 & 0.23 & -14.80 & -14.09 & 30.22   \\
102 & 0.23 & 6.15 & 1.08 & 2.01 & 0.33 & -14.10 & -13.24 & 31.06   \\
103 & 0.24 & 7.63 & 1.26 & 1.44 & 0.18 & -14.20 & -13.02 & 31.29   \\
105 & 0.27 & 3.18 & 0.72 & 3.84 & 1.14 & -14.08 & -13.64 & 30.67   \\
106 & 0.18 & 0.47 & 0.09 & 0.23 & 0.03 & -14.78 & -13.49 & 30.82   \\
107 & 0.29 & 4.81 & 0.52 & 1.52 & 0.15 & -13.85 & -12.87 & 31.43   \\
108 & 0.21 & 6.15 & 1.55 & 3.71 & 1.01 & -13.67 & -13.10 & 31.20   \\
109 & 0.29 & 2.00 & 0.26 & 1.41 & 0.19 & -14.08 & -13.31 & 31.00   \\
110 & 0.25 & 11.86 & 2.55 & 5.28 & 1.53 & -13.82 & -13.25 & 31.06  \\
111 & 0.20 & 2.23 & 0.42 & 3.34 & 0.78 & -13.95 & -13.52 & 30.79   \\
112 & 0.13 & 3.24 & 0.79 & 1.14 & 0.27 & -14.84 & -13.76 & 30.55   \\
113 & 0.32 & 0.40 & 0.10 & 2.40 & 0.52 & -13.94 & -13.65 & 30.66   \\
114 & 0.26 & 3.95 & 0.51 & 1.83 & 0.22 & -13.91 & -13.11 & 31.19   \\
116 & 0.37 & 2.34 & 0.18 & 2.19 & 0.20 & -13.32 & -12.74 & 31.57   \\
117 & 0.27 & 8.29 & 1.34 & 1.17 & 0.14 & -14.27 & -12.83 & 31.48   \\
118 & 0.44 & 3.10 & 0.11 & 2.51 & 0.11 & -12.62 & -12.03 & 32.27   \\
119 & 0.31 & 40.40 & 3.99 & 2.91 & 0.31 & -13.36 & -12.17 & 32.14  \\
120 & 0.35 & 2.40 & 0.19 & 3.05 & 0.30 & -13.22 & -12.75 & 31.56   \\
121 & 0.25 & 0.97 & 0.21 & 5.20 & 1.66 & -13.86 & -13.62 & 30.69   \\
122 & 0.29 & 7.81 & 1.40 & 4.00 & 0.86 & -13.76 & -13.18 & 31.12   \\
123 & 0.14 & 0.01 & -- & 0.97 & 0.30 & -15.07 & -14.97 & 29.34 \\
124 & 0.27 & 2.49 & 0.28 & 2.04 & 0.27 & -13.75 & -13.12 & 31.18   \\
125 & 0.31 & 3.48 & 0.50 & 3.29 & 0.60 & -13.71 & -13.20 & 31.10   \\
126 & 0.20 & 0.98 & 0.21 & 2.01 & 0.41 & -14.16 & -13.70 & 30.61   \\
127 & 0.15 & 19.02 & 3.54 & 0.95 & 0.12 & -14.52 & -12.31 & 31.99  \\
128 & 0.19 & 9.90 & 2.06 & 6.54 & 2.15 & -13.36 & -12.87 & 31.44   \\
129 & 0.24 & 31.05 & 6.22 & 2.15 & 0.38 & -14.11 & -12.79 & 31.52  \\
130 & 0.22 & 1.30 & 0.28 & 0.56 & 0.13 & -15.22 & -13.83 & 30.48   \\
131 & 0.43 & 2.27 & 0.18 & 6.15 & 0.96 & -12.60 & -12.30 & 32.01   \\
132 & 0.24 & 31.70 & 5.43 & 1.63 & 0.21 & -14.09 & -12.47 & 31.83      \\
135 & 0.16 & 4.56 & 1.43 & 1.56 & 0.42 & -14.59 & -13.65 & 30.66       \\
136 & 0.35 & 0.52 & 0.08 & 2.82 & 0.45 & -13.09 & -12.80 & 31.51       \\
137 & 0.17 & 0.24 & 0.17 & 0.82 & 0.21 & -15.17 & -14.75 & 29.56       \\
138 & 0.16 & 0.50 & 0.21 & 1.53 & 0.51 & -14.47 & -14.05 & 30.26       \\
140 & 0.15 & 0.94 & 0.37 & 9.38 & -- & -13.59 & -13.40 & 30.91     \\
141 & 0.12 & 7.96 & 3.47 & $>$15 & -- & -13.74 & -13.42 & 30.89    \\
142 & 0.12 & 1.71 & 0.49 & 2.11 & 0.63 & -14.15 & -13.61 & 30.70       \\
143 & 0.20 & 0.75 & 0.21 & 0.86 & 0.21 & -14.97 & -14.18 & 30.12       \\
144 & 0.12 & 5.78 & 1.33 & 1.14 & 0.21 & -14.32 & -13.00 & 31.31       \\
145 & 0.15 & 0.01 & -- & $>$15 & -- & -14.33 & -14.31 & 30.00  \\
147 & 0.18 & 0.06 & -- & 0.11 & 0.02 & -14.41 & -13.62 & 30.68     \\
148 & 0.31 & 1.88 & 0.40 & 12.51 & -- & -13.71 & -13.49 & 30.82    \\
149 & 0.17 & 0.31 & -- & 2.45 & -- & -15.04 & -14.78 & 29.53   \\
150 & 0.22 & 1.90 & 0.51 & 3.09 & 1.02 & -14.34 & -13.91 & 30.39       \\
152 & 0.20 & 1.11 & 0.42 & 2.93 & 1.19 & -14.58 & -14.21 & 30.10       \\
153 & 0.19 & 0.52 & 0.20 & 1.44 & 0.37 & -14.70 & -14.25 & 30.05       \\
154 & 0.21 & 10.88 & 2.52 & 1.03 & 0.19 & -14.74 & -12.98 & 31.33      \\
155 & 0.22 & 3.72 & 0.86 & 5.53 & 1.86 & -13.76 & -13.38 & 30.93       \\
209 & 0.18 & 10.73 & 4.17 & 3.71 & 1.40 & -14.24 & -13.57 & 30.73      \\
210 & 0.19 & 0.37 & -- & $>$15 & -- & -14.53 & -14.44 & 29.87  \\
214 & 0.12 & 0.05 & 0.03 & 0.05 & 0.00 & -13.32 & -11.51 & 32.79       \\
221 & 0.17 & 2.07 & 0.96 & 5.18 & -- & -14.69 & -14.37 & 29.94     \\
\tableline
South &  &  &  &  &  &   &   &  			       \\
43 & 0.37 & 1.00 & 0.10 & 0.69 & 0.08 & -14.24 & -13.17 & 31.14	       \\
45 & 0.36 & 1.37 & 0.21 & 0.57 & 0.09 & -14.77 & -13.36 & 30.94	       \\
49 & 0.40 & 0.36 & 0.10 & 1.49 & 0.25 & -14.01 & -13.64 & 30.67	       \\
53 & 0.50 & 1.38 & 0.23 & $>$15 & 18.46 & -13.22 & -13.06 & 31.25      \\
54 & 0.39 & 0.39 & 0.12 & 1.04 & 0.16 & -14.44 & -13.94 & 30.37	       \\
55 & 0.34 & 0.44 & 0.12 & 1.25 & 0.18 & -14.27 & -13.81 & 30.50	       \\
75 & 0.41 & 0.17 & 0.10 & 1.44 & 0.30 & -14.32 & -14.05 & 30.26	       \\
79 & 0.32 & 0.35 & 0.11 & 1.01 & 0.13 & -14.44 & -13.96 & 30.35	       \\
88 & 0.35 & 0.36 & 0.17 & 3.54 & 1.40 & -14.14 & -13.93 & 30.38	       \\
94 & 0.43 & 1.63 & 0.40 & $>$15 & -- & -13.55 & -13.40 & 30.91     \\
97 & 0.20 & 3.08 & 0.87 & 3.03 & 1.00 & -14.38 & -13.86 & 30.44	       \\
104 & 0.47 & 2.63 & 0.36 & 6.63 & 1.84 & -13.39 & -13.08 & 31.22       \\
139 & 0.14 & 0.28 & 0.14 & 0.82 & 0.18 & -14.91 & -14.44 & 29.86       \\
151 & 0.62 & 0.70 & 0.06 & 6.83 & 1.18 & -12.81 & -12.62 & 31.68       \\
200 & 0.29 & 0.05 & -- & 1.44 & 0.34 & -14.78 & -14.63 & 29.68     \\
203 & 0.27 & 3.16 & 0.65 & 0.56 & 0.11 & -15.03 & -13.08 & 31.23       \\
205 & 0.29 & 0.30 & 0.17 & 0.90 & 0.15 & -14.98 & -14.51 & 29.80       \\
207 & 0.26 & 0.01 & -- & 1.14 & 0.18 & -14.90 & -14.82 & 29.49     \\
208 & 0.32 & 0.01 & -- & $>$15 & -- & -14.53 & -14.51 & 29.79  \\
212 & 0.30 & 0.54 & 0.25 & 1.83 & 0.80 & -14.70 & -14.31 & 29.99       \\
213 & 0.32 & 1.73 & 0.94 & $>$15 & -- & -14.30 & -14.14 & 30.16    \\
222 & 0.54 & 0.98 & 0.15 & 0.60 & 0.10 & -14.61 & -13.46 & 30.84       \\
223 & 0.50 & 1.65 & 0.32 & 0.49 & 0.10 & -15.04 & -13.39 & 30.92       \\
259 & 0.47 & 0.66 & 0.10 & 0.17 & 0.02 & -14.71 & -12.68 & 31.63       \\
260 & 0.69 & 0.77 & 0.08 & 0.82 & 0.07 & -13.89 & -13.06 & 31.24       \\
263 & 0.49 & 1.19 & 0.15 & 0.95 & 0.13 & -14.18 & -13.28 & 31.03       \\
264 & 0.46 & 0.07 & -- & 1.27 & 0.22 & -14.39 & -14.20 & 30.11     \\
265 & 0.39 & 0.01 & -- & 2.93 & 1.60 & -14.45 & -14.41 & 29.89     \\
267 & 0.43 & 0.40 & 0.06 & 0.49 & 0.04 & -14.08 & -13.36 & 30.95       \\
269 & 0.75 & 0.21 & 0.07 & 4.35 & 1.03 & -13.41 & -13.26 & 31.05       \\
272 & 0.50 & 0.01 & -- & 4.20 & -- & -14.40 & -14.37 & 29.94   \\
274 & 0.66 & 0.83 & 0.14 & 3.74 & 0.76 & -13.46 & -13.17 & 31.13       \\
275 & 0.52 & 0.03 & -- & 2.20 & 0.77 & -14.23 & -14.14 & 30.17     \\
309 & 0.49 & 0.01 & -- & 1.44 & 0.41 & -14.64 & -14.57 & 29.73     \\
310 & 0.66 & 1.09 & 0.29 & 3.75 & 1.28 & -13.89 & -13.58 & 30.73       \\
311 & 0.49 & 0.01 & -- & 1.18 & 0.19 & -14.53 & -14.44 & 29.86     \\
314 & 0.54 & 0.01 & -- & 1.14 & 0.13 & -14.41 & -14.32 & 29.98     \\
315 & 0.60 & 0.25 & -- & 0.01 & -- & -28.64 & -18.07 & 26.23   \\
318 & 0.46 & 0.94 & 0.32 & 1.13 & 0.34 & -14.84 & -14.16 & 30.15       \\
338 & 0.59 & 0.01 & -- & 1.83 & -- & -14.32 & -14.26 & 30.04   \\
\tableline
West &  &  &  &  &  &   &   &  			       \\
156 & 0.28 & 0.27 & 0.15 & 1.01 & 0.21 & -14.79 & -14.37 & 29.93       \\
157 & 0.25 & 0.89 & 0.19 & 4.49 & 1.22 & -13.77 & -13.51 & 30.79       \\
158 & 0.39 & 0.22 & 0.07 & 0.89 & 0.06 & -14.17 & -13.77 & 30.54       \\
159 & 0.15 & 0.01 & -- & 1.40 & 0.45 & -14.96 & -14.89 & 29.42     \\
160 & 0.28 & 0.91 & 0.21 & 1.98 & 0.45 & -14.24 & -13.79 & 30.52       \\
161 & 0.18 & 0.32 & 0.14 & 0.90 & 0.11 & -14.82 & -14.33 & 29.98       \\
162 & 0.46 & 1.69 & 0.18 & 0.18 & 0.01 & -14.95 & -11.79 & 32.51       \\
163 & 0.15 & 0.35 & 0.18 & 1.05 & 0.25 & -14.93 & -14.46 & 29.85       \\
164 & 0.38 & 0.42 & 0.07 & 1.00 & 0.08 & -13.94 & -13.41 & 30.89       \\
165 & 0.63 & 0.09 & 0.05 & 3.30 & 0.74 & -13.52 & -13.39 & 30.91       \\
166 & 0.36 & 19.86 & 2.46 & 3.20 & 0.43 & -13.44 & -12.55 & 31.76      \\
167 & 0.50 & 1.10 & 0.11 & 5.24 & 0.87 & -13.08 & -12.82 & 31.49       \\
168 & 0.49 & 0.46 & 0.10 & 1.31 & 0.19 & -14.06 & -13.61 & 30.70       \\
169 & 0.21 & 2.04 & 0.63 & 2.13 & 0.74 & -14.61 & -14.03 & 30.27       \\
170 & 0.43 & 0.56 & 0.11 & 3.71 & 0.77 & -13.63 & -13.39 & 30.92       \\
171 & 0.32 & 0.29 & 0.06 & 0.21 & 0.02 & -14.48 & -13.46 & 30.85       \\
172 & 0.38 & 0.70 & 0.13 & 2.82 & 0.56 & -13.74 & -13.41 & 30.89       \\
173 & 0.38 & 0.60 & 0.13 & 3.41 & 0.80 & -13.77 & -13.50 & 30.80       \\
174 & 0.45 & 0.06 & 0.06 & 2.88 & 0.70 & -13.81 & -13.69 & 30.61       \\
175 & 0.36 & 1.35 & 0.35 & 2.71 & 0.90 & -14.28 & -13.86 & 30.45       \\
176 & 0.34 & 0.01 & -- & 4.20 & -- & -14.35 & -14.31 & 29.99   \\
215 & 0.33 & 0.22 & 0.06 & 0.25 & 0.02 & -14.40 & -13.66 & 30.64       \\
216 & 0.30 & 3.34 & 0.92 & 2.72 & 0.90 & -14.37 & -13.80 & 30.51       \\
217 & 0.32 & 0.75 & 0.15 & 0.61 & 0.13 & -14.86 & -13.88 & 30.42       \\
218 & 0.27 & 0.81 & 0.20 & 0.75 & 0.18 & -14.96 & -14.05 & 30.26       \\
219 & 0.57 & 0.15 & -- & 0.01 & -- & -26.86 & -18.29 & 26.02   \\
220 & 0.40 & 4.73 & 0.92 & 3.34 & 0.75 & -13.85 & -13.29 & 31.01       \\
224 & 0.51 & 0.41 & 0.10 & 0.17 & 0.02 & -14.87 & -13.35 & 30.96       \\
225 & 0.49 & 0.01 & -- & 1.04 & 0.23 & -14.80 & -14.71 & 29.60     \\
280 & 0.65 & 3.28 & 0.44 & 4.66 & 0.91 & -13.36 & -12.96 & 31.34       \\
281 & 0.82 & 1.37 & 0.30 & $>$15 & 28.28 & -13.32 & -13.17 & 31.14     \\
282 & 0.47 & 0.78 & 0.11 & 1.03 & 0.09 & -14.06 & -13.36 & 30.94       \\
283 & 0.46 & 1.09 & 0.17 & 0.99 & 0.15 & -14.38 & -13.54 & 30.76       \\
284 & 0.59 & 4.41 & 0.74 & $>$15 & -- & -13.18 & -12.95 & 31.36    \\
285 & 0.47 & 0.02 & -- & 2.22 & 0.82 & -14.09 & -14.01 & 30.30     \\
286 & 0.61 & 0.01 & -- & 0.94 & 0.07 & -14.03 & -13.93 & 30.38     \\
287 & 0.60 & 0.50 & 0.12 & 1.57 & 0.35 & -14.07 & -13.66 & 30.65       \\
288 & 0.68 & 0.25 & 0.11 & 3.28 & 1.06 & -13.91 & -13.72 & 30.59       \\
289 & 0.63 & 0.38 & -- & 0.01 & -- & -28.59 & -16.03 & 28.27   \\
290 & 0.50 & 0.01 & -- & 1.04 & 0.10 & -14.06 & -13.97 & 30.33     \\
291 & 0.48 & 0.01 & -- & 0.07 & 0.01 & -13.61 & -13.10 & 31.21     \\
292 & 0.45 & 0.01 & -- & 0.98 & 0.17 & -14.46 & -14.37 & 29.94     \\
293 & 0.57 & 0.48 & 0.11 & 1.91 & 0.36 & -13.94 & -13.58 & 30.73       \\
294 & 0.55 & 0.41 & 0.07 & 0.89 & 0.06 & -14.05 & -13.49 & 30.82       \\
295 & 0.53 & 0.22 & 0.10 & 1.03 & 0.13 & -14.37 & -14.00 & 30.31       \\
296 & 0.60 & 1.26 & 0.23 & 0.86 & 0.17 & -14.52 & -13.51 & 30.79       \\
297 & 0.58 & 0.01 & -- & 2.83 & 0.76 & -13.64 & -13.59 & 30.71     \\
320 & 0.59 & 1.25 & 0.17 & 0.71 & 0.10 & -14.47 & -13.30 & 31.01       \\
321 & 0.63 & 0.52 & 0.37 & $>$15 & -- & -14.11 & -14.01 & 30.30    \\
322 & 0.53 & 0.01 & -- & 12.88 & -- & -14.04 & -14.02 & 30.28  \\
323 & 0.52 & 0.01 & -- & 1.01 & 0.14 & -14.43 & -14.34 & 29.97     \\
324 & 0.50 & 0.67 & 0.16 & 0.84 & 0.19 & -14.63 & -13.87 & 30.43       \\
325 & 0.49 & 1.53 & 0.38 & 2.14 & 0.79 & -14.30 & -13.78 & 30.52       \\
326 & 0.67 & 0.28 & 0.14 & 4.86 & 2.08 & -13.98 & -13.82 & 30.49       \\
327 & 0.59 & 0.01 & -- & 1.08 & 0.18 & -14.48 & -14.38 & 29.92     \\
328 & 0.64 & 0.01 & -- & $>$15 & -- & -14.22 & -14.21 & 30.10  \\
329 & 0.62 & 0.70 & 0.20 & 1.30 & 0.28 & -14.37 & -13.82 & 30.49       \\
330 & 0.57 & 1.24 & 0.23 & 0.71 & 0.14 & -14.71 & -13.53 & 30.77       \\
331 & 0.51 & 0.06 & -- & $>$15 & -- & -13.61 & -13.58 & 30.73  \\
332 & 0.57 & 0.01 & -- & 1.43 & 0.36 & -14.55 & -14.48 & 29.82     \\
333 & 0.59 & 0.39 & 0.17 & 6.84 & 3.21 & -13.77 & -13.62 & 30.69       \\
334 & 0.51 & 0.15 & 0.09 & 3.38 & 1.16 & -13.73 & -13.58 & 30.73       \\
340 & 0.58 & 0.01 & -- & 1.91 & 0.73 & -14.21 & -14.16 & 30.15     \\
341 & 0.70 & 0.23 & 0.15 & $>$15 & 26.57 & -13.55 & -13.48 & 30.83     \\
\enddata
\tablenotetext{a}{$\chi^2$/d.o.f is included for completeness.  These
  models were calculated with C statistics,  it is
unclear how $\chi^2$/d.o.f  relates to  goodness of fit.  The formal
errors are unbiased however. --
see text.}
\end{deluxetable}










